Towards a Unified Framework of Clustering-based Anomaly Detection

Unsupervised Anomaly Detection (UAD) plays a crucial role in identifying abnormal patterns within data without labeled examples, holding significant practical implications across various domains. Although the individual contributions of representation learning and clustering to anomaly detection are well-established, their interdependencies remain under-explored due to the absence of a unified theoretical framework. Consequently, their collective potential to enhance anomaly detection performance remains largely untapped. To bridge this gap, in this paper, we propose a novel probabilistic mixture model for anomaly detection to establish a theoretical connection among representation learning, clustering, and anomaly detection. By maximizing a novel anomaly-aware data likelihood, representation learning and clustering can effectively reduce the adverse impact of anomalous data and collaboratively benefit anomaly detection. Meanwhile, a theoretically substantiated anomaly score is naturally derived from this framework. Lastly, drawing inspiration from gravitational analysis in physics, we have devised an improved anomaly score that more effectively harnesses the combined power of representation learning and clustering. Extensive experiments, involving 17 baseline methods across 30 diverse datasets, validate the effectiveness and generalization capability of the proposed method, surpassing state-of-the-art methods.

==> sections/preliminaries.tex <==
% \subsection{Notations and Definitions}

\input{tables/notations}

% \textbf{Unsupervised Anomaly Detection.}
Given a dataset $\mathbf{X} \in \mathbb{R}^{N \times D}$ comprising $N$ instances and $D$ features, \textbf{unsupervised anomaly detection} aims to learn an anomaly score $o_{i}$ for each instance $x_{i}$ in an unsupervised manner, so that the abnormal ones have higher scores than the normal ones.
In practice, the samples are usually attributed by high-dimensional features and it is challenging to detect anomalies from the raw features.
Therefore, modern anomaly detection methods often employ representation learning techniques to map each raw data instance $x_{i}$ into a low-dimensional vector $h_{i}$ and detect anomalies within this space.
The detailed notations are summarized in Table \ref{table:notations}.
\zs{The current section seems too short, shall we merge it into methogology section?}
% which can be formulated as:
% \begin{equation}
%      \mathbf{o} = \mathcal{S}(\mathbf{X})
%      % , \text{ where } \mathbf{Z} = \mathcal{F}(\mathbf{X}), 
% \end{equation}
% where $\mathcal{S}(\cdot)$ represents the anomaly scoring function,
% and $\mathcal{F}(\cdot)$ denotes the representation learning function.
% $\mathbf{Z} = \{\mathbf{z_i}\} \in \mathbb{R}^{N \times d}$ is the embedding matrix, while 
% $\mathbf{o} \in \mathbb{R}^{1 \times N}$ is the anomaly score with each element $\mathbf{o}_i$ denoting the anomaly score for instance $\mathbf{x}_i$.


==> tables/ablation.tex <==
% Table generated by Excel2LaTeX from sheet 'pivot_aucroc'
\begin{table}[t]
  \centering
  \caption{Ablation study on AUC-ROC scores.}
    \begin{tabular}{c|cccc}
    \toprule
    \textbf{Dataset} & \textbf{w/ Gauss.} & \textbf{w/o $J(\Theta,\Phi)$} & \textbf{w/o $\delta(\mathbf{x}_i)$} & \textbf{Ours} \\
    \midrule
    Hepatitis & 0.740 & 0.768  & 0.767  & \textbf{0.806 } \\
    Ionosphere & 0.886 & 0.882  & 0.893  & \textbf{0.904 } \\
    landsat & 0.551 & 0.549  & 0.551  & \textbf{0.574 } \\
    letter & 0.658 & 0.673  & 0.697  & \textbf{0.738 } \\
    mnist & 0.857 & 0.850  & 0.856  & \textbf{0.866 } \\
    satellite & 0.579 & 0.753  & 0.761  & \textbf{0.777 } \\
    Stamps & 0.914 & 0.903  & 0.919  & \textbf{0.942 } \\
    vertebral & 0.342 & 0.352  & 0.304  & \textbf{0.474 } \\
    % Wilt & 0.371  & 0.455  & \textbf{0.526 } \\
    wine & 0.814 & 0.818  & 0.917  & \textbf{0.952 } \\
    WPBC & 0.480 & 0.466  & 0.474  & \textbf{0.499 } \\
    \midrule
    \makecell{Avg. Rank \\ (w/ baselines)} & 6.7 & 6.5   & 5.0   & 4.2 $\uparrow$ \\
    \bottomrule
    \end{tabular}%
  \label{tab:abla_auc}%
\end{table}%


\begin{table}[t]
  \centering
  \caption{Ablation study on AUC-PR scores.}
    \begin{tabular}{c|cccc}
    \toprule
    \textbf{Dataset} & \textbf{w/ Gauss.} & \textbf{w/o $J(\Theta,\Phi)$} & \textbf{w/o $\delta(\mathbf{x}_i)$} & \textbf{Ours} \\
    \midrule
    Hepatitis & 0.318 & 0.364  & 0.390  & \textbf{0.434}  \\
    Ionosphere & 0.854 & 0.854  & 0.866  & \textbf{0.876}  \\
    landsat & 0.215 & 0.218  & 0.217  & \textbf{0.233}  \\
    letter & 0.105 & 0.111  & 0.126  & \textbf{0.143}  \\
    mnist & 0.411 & 0.407  & 0.409  & \textbf{0.419}  \\
    satellite & 0.710 & 0.705  & 0.728  & \textbf{0.751}  \\
    Stamps & 0.416 & 0.386  & 0.429  & \textbf{0.509}  \\
    vertebral & 0.101 & 0.101  & 0.096  & \textbf{0.130}  \\
    wine  & 0.226 & 0.220  & 0.379  & \textbf{0.496}  \\
    WPBC  & 0.228 & 0.218  & 0.224  & \textbf{0.249}  \\
    \midrule
    \makecell{Avg. Rank \\ (w/ baselines)} & 7.4 & 7.7   & 6.4   & 5.3 $\uparrow$ \\
    \bottomrule
    \end{tabular}%s
  \label{tab:abla_pr}%
\end{table}%


==> tables/aucpr.tex <==
% Table generated by Excel2LaTeX from sheet 'pivot_aucpr'
\begin{table*}[htbp]
  \centering
  \caption{AUCPR of 17 unsupervised algorithms on 47 tabular benchmark datasets. 
  In each dataset, the highest score is highlighted in \textbf{bold}, and the second-highest score is \underline{underlined}.
  The table includes three summary statistics for each algorithm: Avg. rank (average ranking across all datasets).}
  \begin{adjustbox}{max width=\linewidth}

\begin{tabular}{c|ccccccccccccccccc|c}
\toprule
    \textbf{Dataset} & \textbf{CBLOF} & \textbf{COF} & \textbf{COPOD} & \makecell{\textbf{DA} \\ \textbf{GMM}} & \textbf{DCFOD} & \makecell{\textbf{Deep} \\ \textbf{SVDD}} & \textbf{ECOD} & \textbf{GMM} & \textbf{HBOS} & \textbf{IForest} & \textbf{KMeans-$ $-} & \textbf{KNN} & \textbf{LODA} & \textbf{LOF} & \textbf{OCSVM} & \textbf{PCA} & \textbf{SOD} & \textbf{\model} \\
    \midrule
ALOI & 0.045 & \underline{0.068} & 0.036 & 0.043 & 0.041 & 0.037 & 0.039 & 0.048 & 0.037 & 0.039 & 0.047 & 0.060 & 0.045 & \textbf{0.081} & 0.050 & 0.042 & 0.060 & 0.040 \\
annthyroid & 0.137 & 0.144 & 0.166 & 0.096 & 0.100 & 0.218 & \underline{0.254} & 0.136 & 0.170 & \textbf{0.305} & 0.154 & 0.167 & 0.071 & 0.157 & 0.104 & 0.161 & 0.188 & 0.170 \\
backdoor & 0.070 & 0.238 & 0.077 & 0.055 & 0.068 & \underline{0.557} & 0.107 & \textbf{0.564} & 0.050 & 0.048 & 0.155 & 0.444 & 0.138 & 0.261 & 0.088 & 0.313 & 0.371 & 0.364 \\
breastw & 0.919 & 0.276 & \textbf{0.994} & N/A & 0.968 & 0.486 & \underline{0.985} & 0.914 & 0.977 & 0.960 & 0.922 & 0.922 & 0.970 & 0.285 & 0.827 & 0.951 & 0.849 & 0.959 \\
campaign & 0.209 & 0.130 & \textbf{0.386} & 0.145 & 0.196 & 0.168 & 0.367 & 0.294 & \underline{0.380} & 0.323 & 0.189 & 0.272 & 0.141 & 0.146 & 0.292 & 0.279 & 0.191 & 0.271 \\
cardio & 0.619 & 0.287 & 0.604 & 0.289 & 0.543 & 0.225 & 0.597 & 0.510 & 0.521 & 0.599 & 0.382 & 0.407 & 0.534 & 0.238 & \underline{0.629} & \textbf{0.661} & 0.285 & 0.563 \\
Cardiotocography & 0.454 & 0.282 & 0.405 & 0.306 & 0.477 & 0.349 & \underline{0.499} & 0.365 & 0.383 & 0.415 & 0.356 & 0.348 & 0.480 & 0.307 & \textbf{0.526} & 0.480 & 0.280 & 0.374 \\
celeba & 0.112 & 0.018 & 0.137 & 0.019 & \textbf{0.175} & 0.027 & 0.140 & 0.101 & 0.138 & 0.090 & 0.032 & 0.031 & 0.040 & 0.017 & 0.107 & \underline{0.159} & 0.024 & 0.147 \\
census & 0.075 & 0.049 & 0.099 & 0.090 & \textbf{0.109} & 0.084 & 0.095 & 0.097 & 0.087 & 0.078 & 0.081 & 0.090 & 0.050 & 0.055 & 0.068 & \underline{0.100} & 0.085 & 0.098 \\
cover & 0.045 & 0.040 & 0.114 & \textbf{0.276} & 0.015 & 0.033 & \underline{0.171} & 0.104 & 0.068 & 0.089 & 0.098 & 0.062 & 0.131 & 0.081 & 0.114 & 0.098 & 0.039 & 0.039 \\
donors & 0.180 & 0.089 & 0.216 & 0.107 & 0.184 & 0.177 & \textbf{0.270} & 0.147 & \underline{0.244} & 0.127 & N/A & 0.160 & 0.039 & 0.085 & 0.104 & 0.179 & 0.103 & 0.142 \\
fault & 0.468 & 0.416 & 0.305 & 0.335 & 0.338 & 0.355 & 0.319 & 0.430 & 0.365 & 0.411 & \underline{0.518} & \textbf{0.545} & 0.310 & 0.384 & 0.384 & 0.328 & 0.480 & 0.337 \\
fraud & 0.392 & 0.215 & \underline{0.428} & 0.157 & 0.035 & 0.215 & 0.374 & 0.118 & 0.280 & 0.217 & 0.395 & 0.376 & 0.396 & \textbf{0.466} & 0.403 & 0.229 & 0.175 & 0.423 \\
glass & 0.116 & 0.118 & 0.098 & \textbf{0.246} & 0.097 & 0.085 & 0.154 & 0.128 & 0.118 & 0.110 & 0.147 & \underline{0.203} & 0.134 & 0.201 & 0.080 & 0.100 & 0.187 & 0.153 \\
Hepatitis & 0.365 & 0.144 & \underline{0.415} & 0.229 & 0.195 & 0.300 & 0.328 & 0.332 & 0.377 & 0.263 & 0.251 & 0.220 & 0.309 & 0.137 & 0.294 & 0.366 & 0.247 & \textbf{0.434} \\
http & 0.475 & 0.096 & 0.352 & N/A & 0.440 & 0.134 & 0.166 & 0.554 & 0.448 & \textbf{0.908} & 0.451 & 0.007 & 0.007 & 0.038 & 0.469 & \underline{0.564} & 0.083 & 0.435 \\
InternetAds & \underline{0.544} & 0.387 & 0.510 & N/A & 0.327 & 0.319 & 0.511 & 0.384 & 0.540 & 0.486 & 0.501 & 0.432 & 0.239 & 0.401 & \textbf{0.547} & 0.325 & 0.269 & 0.242 \\
Ionosphere & 0.898 & 0.829 & 0.699 & 0.650 & 0.476 & 0.432 & 0.647 & \underline{0.906} & 0.418 & 0.804 & \textbf{0.914} & 0.904 & 0.730 & 0.881 & 0.745 & 0.739 & 0.859 & 0.876 \\
landsat & \underline{0.311} & 0.250 & 0.175 & 0.245 & 0.156 & \textbf{0.369} & 0.162 & 0.184 & 0.220 & 0.198 & 0.224 & 0.246 & 0.189 & 0.247 & 0.162 & 0.162 & 0.264 & 0.233 \\
letter & 0.139 & 0.214 & 0.068 & 0.117 & 0.063 & 0.088 & 0.076 & 0.183 & 0.084 & 0.085 & 0.153 & \underline{0.300} & 0.069 & \textbf{0.340} & 0.061 & 0.069 & 0.286 & 0.143 \\
Lymphography & 0.973 & 0.367 & 0.887 & 0.195 & 0.123 & 0.346 & 0.909 & 0.715 & 0.918 & \underline{0.973} & \textbf{1.000} & 0.387 & 0.445 & 0.231 & 0.936 & 0.970 & 0.220 & 0.967 \\
magic.gamma & \underline{0.688} & 0.541 & 0.592 & 0.469 & 0.598 & 0.487 & 0.537 & 0.667 & 0.624 & 0.647 & 0.683 & \textbf{0.756} & 0.585 & 0.548 & 0.514 & 0.593 & 0.679 & 0.650 \\
mammography & 0.111 & 0.111 & \underline{0.407} & N/A & 0.161 & 0.051 & \textbf{0.413} & 0.211 & 0.213 & 0.207 & N/A & 0.159 & 0.147 & 0.098 & 0.129 & 0.192 & 0.134 & 0.063 \\
mnist & 0.306 & 0.255 & 0.213 & 0.237 & 0.236 & 0.202 & 0.175 & 0.387 & 0.125 & 0.277 & 0.371 & 0.355 & 0.259 & 0.209 & 0.332 & \underline{0.399} & 0.192 & \textbf{0.419} \\
musk & 1.000 & 0.026 & 0.348 & 0.328 & 0.029 & 0.088 & 0.501 & 0.903 & \underline{1.000} & 0.996 & 0.375 & 0.097 & 0.476 & 0.028 & 0.106 & 0.999 & 0.076 & \textbf{1.000} \\
optdigits & \textbf{0.102} & 0.044 & 0.044 & 0.056 & 0.026 & 0.022 & 0.035 & 0.027 & \underline{0.100} & 0.051 & 0.095 & 0.031 & 0.040 & 0.061 & 0.029 & 0.028 & 0.044 & 0.028 \\
PageBlocks & 0.497 & 0.410 & 0.376 & \underline{0.533} & 0.424 & 0.292 & 0.516 & \textbf{0.554} & 0.333 & 0.460 & 0.457 & 0.454 & 0.513 & 0.396 & 0.491 & 0.517 & 0.378 & 0.490 \\
pendigits & \textbf{0.329} & 0.029 & 0.212 & 0.047 & 0.222 & 0.015 & 0.306 & 0.064 & 0.293 & 0.261 & \underline{0.327} & 0.065 & 0.187 & 0.038 & 0.235 & 0.236 & 0.045 & 0.217 \\
Pima & 0.530 & 0.447 & 0.552 & 0.415 & 0.502 & 0.350 & 0.505 & 0.533 & \textbf{0.566} & \underline{0.558} & 0.535 & 0.551 & 0.441 & 0.472 & 0.500 & 0.540 & 0.482 & 0.542 \\
satellite & 0.614 & 0.397 & 0.566 & 0.583 & 0.433 & 0.418 & 0.522 & 0.498 & \underline{0.672} & 0.659 & 0.547 & 0.500 & 0.619 & 0.377 & 0.576 & 0.596 & 0.472 & \textbf{0.751} \\
satimage-2 & 0.971 & 0.088 & 0.765 & 0.221 & 0.081 & 0.026 & 0.645 & 0.436 & 0.780 & 0.934 & \underline{0.971} & 0.391 & 0.805 & 0.043 & 0.827 & 0.857 & 0.261 & \textbf{0.973} \\
shuttle & 0.799 & 0.122 & \underline{0.966} & 0.932 & 0.818 & 0.124 & 0.904 & 0.882 & 0.964 & \textbf{0.976} & 0.327 & 0.204 & 0.488 & 0.138 & 0.853 & 0.924 & 0.203 & 0.924 \\
skin & 0.283 & 0.164 & 0.180 & N/A & 0.263 & 0.191 & 0.184 & 0.286 & 0.237 & 0.261 & 0.256 & \underline{0.287} & 0.184 & 0.183 & 0.190 & 0.174 & 0.246 & \textbf{0.287} \\
smtp & 0.242 & 0.611 & 0.011 & 0.500 & 0.002 & 0.500 & 0.500 & 0.345 & 0.352 & 0.012 & 0.667 & \underline{0.667} & 0.358 & 0.207 & 0.189 & \textbf{0.667} & 0.334 & 0.016 \\
SpamBase & 0.412 & 0.347 & \textbf{0.567} & N/A & 0.380 & 0.397 & \underline{0.540} & 0.401 & 0.500 & 0.518 & 0.422 & 0.414 & 0.359 & 0.352 & 0.401 & 0.416 & 0.400 & 0.417 \\
speech & 0.020 & 0.022 & 0.019 & 0.020 & \underline{0.028} & 0.016 & 0.020 & \textbf{0.028} & 0.021 & 0.023 & 0.020 & 0.020 & 0.018 & 0.025 & 0.020 & 0.020 & 0.021 & 0.017 \\
Stamps & 0.245 & 0.165 & 0.431 & 0.437 & \underline{0.474} & 0.121 & 0.332 & 0.350 & 0.352 & 0.395 & 0.356 & 0.235 & 0.346 & 0.213 & 0.314 & 0.411 & 0.203 & \textbf{0.509} \\
thyroid & 0.299 & 0.285 & 0.196 & 0.161 & 0.106 & 0.027 & 0.511 & 0.317 & 0.510 & \textbf{0.631} & 0.317 & 0.350 & 0.147 & 0.208 & 0.212 & 0.443 & 0.236 & \underline{0.568} \\
vertebral & 0.114 & 0.138 & 0.089 & \textbf{0.152} & 0.116 & 0.106 & 0.118 & 0.114 & 0.092 & 0.105 & 0.105 & 0.106 & 0.097 & \underline{0.142} & 0.109 & 0.105 & 0.118 & 0.130 \\
vowels & 0.351 & \underline{0.560} & 0.041 & 0.122 & 0.036 & 0.046 & 0.106 & 0.292 & 0.134 & 0.151 & 0.491 & \textbf{0.634} & 0.138 & 0.344 & 0.082 & 0.089 & 0.389 & 0.324 \\
Waveform & \underline{0.179} & 0.141 & 0.069 & 0.031 & 0.043 & 0.044 & 0.048 & 0.043 & 0.059 & 0.062 & \textbf{0.197} & 0.130 & 0.047 & 0.113 & 0.044 & 0.058 & 0.097 & 0.078 \\
WBC & 0.673 & 0.097 & 0.862 & N/A & 0.334 & 0.090 & 0.862 & 0.443 & 0.736 & \textbf{0.905} & 0.719 & 0.666 & 0.787 & 0.056 & \underline{0.899} & 0.823 & 0.540 & 0.831 \\
WDBC & 0.836 & 0.505 & \underline{0.848} & 0.185 & 0.289 & 0.076 & 0.579 & 0.356 & \textbf{0.890} & 0.785 & 0.123 & 0.437 & 0.661 & 0.149 & 0.719 & 0.755 & 0.356 & 0.600 \\
Wilt & 0.037 & 0.050 & 0.037 & 0.040 & 0.046 & 0.047 & 0.039 & \textbf{0.072} & 0.038 & 0.042 & 0.038 & 0.047 & 0.034 & 0.050 & 0.036 & 0.031 & \underline{0.055} & 0.052 \\
wine & 0.060 & 0.085 & 0.457 & 0.175 & 0.244 & 0.188 & 0.235 & 0.107 & 0.431 & 0.260 & 0.063 & 0.084 & \underline{0.488} & 0.078 & 0.216 & 0.309 & 0.080 & \textbf{0.496} \\
WPBC & 0.211 & 0.213 & 0.228 & 0.225 & 0.229 & 0.250 & 0.212 & 0.216 & 0.230 & 0.224 & 0.206 & 0.215 & \underline{0.254} & 0.203 & 0.229 & 0.230 & \textbf{0.256} & 0.249 \\
yeast & 0.310 & 0.313 & 0.307 & 0.299 & 0.274 & 0.304 & \underline{0.333} & 0.291 & 0.327 & 0.298 & 0.300 & 0.293 & \textbf{0.333} & 0.316 & 0.298 & 0.299 & 0.300 & 0.293 \\
\midrule
  Avg. Rank &  7.5   & 11.7  & 8.8   & 11.0  & 11.6  & 13.2  & 8.0   & 8.5   & 7.6   & 7.5   & 8.1   & 8.5   & 10.5  & 11.5  & 9.9   & 8.0   & 10.4  & 7.1  \\
\bottomrule
    \end{tabular}%

    \end{adjustbox}
\label{tab:aucpr}%
\end{table*}%



==> tables/aucpr_v2.tex <==
% Table generated by Excel2LaTeX from sheet 'pivot_aucpr'
\begin{table*}[htbp]
  \centering
  \caption{AUCPR of 17 unsupervised algorithms on 47 tabular benchmark datasets. 
  In each dataset, the highest score is highlighted in \textbf{bold}, and the second-highest score is \underline{underlined}.
  The table includes three summary statistics for each algorithm: Avg. Rank (average ranking across all datasets).}
  \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{c|ccccccccccccccccc|cc}
    \toprule
    \textbf{Dataset} & \textbf{CBLOF} & \textbf{COF} & \textbf{COPOD} & \makecell{\textbf{DA} \\ \textbf{GMM}} & \textbf{DCFOD} & \makecell{\textbf{Deep} \\ \textbf{SVDD}} & \textbf{ECOD} & \textbf{GMM} & \textbf{HBOS} & \textbf{IForest} & \textbf{KMeans-$ $-} & \textbf{KNN} & \textbf{LODA} & \textbf{LOF} & \textbf{OCSVM} & \textbf{PCA} & \textbf{SOD} & \makecell{\textbf{\model} \\ \textbf{(Scalar)}}  &   \makecell{\textbf{\model} \\ \textbf{(Vector)}}\\
    \midrule
ALOI & 4.50 & \underline{6.80}  & 3.60 & 4.30 & 4.10 & 3.70 & 3.90 & 4.80 & 3.70 & 3.90 & 4.70 & 6.00 & 4.50 & \textbf{8.10} & 5.00 & 4.20 & 6.00 & 4.00 & 4.00 \\
annthyroid & 13.70 & 14.40 & 16.60 & 9.60 & 10.00 & 21.80 & 25.40 & 13.60 & 17.00 & \textbf{30.50} & 15.40 & 16.70 & 7.10 & 15.70 & 10.40 & 16.10 & 18.80 & \underline{26.40}  & 25.00 \\
backdoor & 7.00 & 23.80 & 7.70 & 5.50 & 6.80 & \underline{55.70}  & 10.70 & \textbf{56.40} & 5.00 & 4.80 & 15.50 & 44.40 & 13.80 & 26.10 & 8.80 & 31.30 & 37.10 & 37.80 & 36.40 \\
breastw & 91.90 & 27.60 & \textbf{99.40} & N/A & 96.80 & 48.60 & \underline{98.50}  & 91.40 & 97.70 & 96.00 & 92.20 & 92.20 & 97.00 & 28.50 & 82.70 & 95.10 & 84.90 & 94.50 & 95.90 \\
campaign & 20.90 & 13.00 & \textbf{38.60} & 14.50 & 19.60 & 16.80 & 36.70 & 29.40 & \underline{38.00}  & 32.30 & 18.90 & 27.20 & 14.10 & 14.60 & 29.20 & 27.90 & 19.10 & 27.70 & 27.10 \\
cardio & 61.90 & 28.70 & 60.40 & 28.90 & 54.30 & 22.50 & 59.70 & 51.00 & 52.10 & 59.90 & 38.20 & 40.70 & 53.40 & 23.80 & \underline{62.90}  & \textbf{66.10} & 28.50 & 54.70 & 56.30 \\
Cardiotocography & 45.40 & 28.20 & 40.50 & 30.60 & 47.70 & 34.90 & \underline{49.90}  & 36.50 & 38.30 & 41.50 & 35.60 & 34.80 & 48.00 & 30.70 & \textbf{52.60} & 48.00 & 28.00 & 37.40 & 37.40 \\
celeba & 11.20 & 1.80 & 13.70 & 1.90 & \textbf{17.50} & 2.70 & 14.00 & 10.10 & 13.80 & 9.00 & 3.20 & 3.10 & 4.00 & 1.70 & 10.70 & \underline{15.90}  & 2.40 & 15.10 & 14.70 \\
census & 7.50 & 4.90 & 9.90 & 9.00 & \textbf{10.90} & 8.40 & 9.50 & 9.70 & 8.70 & 7.80 & 8.10 & 9.00 & 5.00 & 5.50 & 6.80 & \underline{10.00}  & 8.50 & 9.70 & 9.80 \\
cover & 4.50 & 4.00 & 11.40 & \textbf{27.60} & 1.50 & 3.30 & \underline{17.10}  & 10.40 & 6.80 & 8.90 & 9.80 & 6.20 & 13.10 & 8.10 & 11.40 & 9.80 & 3.90 & 9.20 & 3.90 \\
donors & 18.00 & 8.90 & 21.60 & 10.70 & 18.40 & 17.70 & \textbf{27.00} & 14.70 & \underline{24.40}  & 12.70 & N/A & 16.00 & 3.90 & 8.50 & 10.40 & 17.90 & 10.30 & 14.10 & 14.20 \\
fault & 46.80 & 41.60 & 30.50 & 33.50 & 33.80 & 35.50 & 31.90 & 43.00 & 36.50 & 41.10 & \underline{51.80}  & \textbf{54.50} & 31.00 & 38.40 & 38.40 & 32.80 & 48.00 & 38.40 & 33.70 \\
fraud & 39.20 & 21.50 & \underline{42.80}  & 15.70 & 3.50 & 21.50 & 37.40 & 11.80 & 28.00 & 21.70 & 39.50 & 37.60 & 39.60 & \textbf{46.60} & 40.30 & 22.90 & 17.50 & 36.60 & 42.30 \\
glass & 11.60 & 11.80 & 9.80 & \textbf{24.60} & 9.70 & 8.50 & 15.40 & 12.80 & 11.80 & 11.00 & 14.70 & \underline{20.30}  & 13.40 & 20.10 & 8.00 & 10.00 & 18.70 & 13.30 & 15.30 \\
Hepatitis & 36.50 & 14.40 & \underline{41.50}  & 22.90 & 19.50 & 30.00 & 32.80 & 33.20 & 37.70 & 26.30 & 25.10 & 22.00 & 30.90 & 13.70 & 29.40 & 36.60 & 24.70 & 36.10 & \textbf{43.40} \\
http & 47.50 & 9.60 & 35.20 & N/A & 44.00 & 13.40 & 16.60 & 55.40 & 44.80 & \textbf{90.80} & 45.10 & 0.70 & 0.70 & 3.80 & 46.90 & \underline{56.40}  & 8.30 & 43.50 & 43.50 \\
InternetAds & \underline{54.40}  & 38.70 & 51.00 & N/A & 32.70 & 31.90 & 51.10 & 38.40 & 54.00 & 48.60 & 50.10 & 43.20 & 23.90 & 40.10 & \textbf{54.70} & 32.50 & 26.90 & 23.10 & 24.20 \\
Ionosphere & 89.80 & 82.90 & 69.90 & 65.00 & 47.60 & 43.20 & 64.70 & \underline{90.60}  & 41.80 & 80.40 & \textbf{91.40} & 90.40 & 73.00 & 88.10 & 74.50 & 73.90 & 85.90 & 89.50 & 87.60 \\
landsat & \underline{31.10}  & 25.00 & 17.50 & 24.50 & 15.60 & \textbf{36.90} & 16.20 & 18.40 & 22.00 & 19.80 & 22.40 & 24.60 & 18.90 & 24.70 & 16.20 & 16.20 & 26.40 & 20.80 & 23.30 \\
letter & 13.90 & 21.40 & 6.80 & 11.70 & 6.30 & 8.80 & 7.60 & 18.30 & 8.40 & 8.50 & 15.30 & \underline{30.00}  & 6.90 & \textbf{34.00} & 6.10 & 6.90 & 28.60 & 13.70 & 14.30 \\
Lymphography & 97.30 & 36.70 & 88.70 & 19.50 & 12.30 & 34.60 & 90.90 & 71.50 & 91.80 & \underline{97.30}  & \textbf{100.00} & 38.70 & 44.50 & 23.10 & 93.60 & 97.00 & 22.00 & 91.70 & 96.70 \\
magic & \underline{68.80}  & 54.10 & 59.20 & 46.90 & 59.80 & 48.70 & 53.70 & 66.70 & 62.40 & 64.70 & 68.30 & \textbf{75.60} & 58.50 & 54.80 & 51.40 & 59.30 & 67.90 & 65.80 & 65.00 \\
mammography & 11.10 & 11.10 & \underline{40.70}  & N/A & 16.10 & 5.10 & \textbf{41.30} & 21.10 & 21.30 & 20.70 & N/A & 15.90 & 14.70 & 9.80 & 12.90 & 19.20 & 13.40 & 15.90 & 6.30 \\
mnist & 30.60 & 25.50 & 21.30 & 23.70 & 23.60 & 20.20 & 17.50 & 38.70 & 12.50 & 27.70 & 37.10 & 35.50 & 25.90 & 20.90 & 33.20 & 39.90 & 19.20 & \underline{41.20}  & \textbf{41.90} \\
musk & 100.00 & 2.60 & 34.80 & 32.80 & 2.90 & 8.80 & 50.10 & 90.30 & \underline{100.00}  & 99.60 & 37.50 & 9.70 & 47.60 & 2.80 & 10.60 & 99.90 & 7.60 & 97.70 & \textbf{100.00} \\
optdigits & \textbf{10.20} & 4.40 & 4.40 & 5.60 & 2.60 & 2.20 & 3.50 & 2.70 & \underline{10.00}  & 5.10 & 9.50 & 3.10 & 4.00 & 6.10 & 2.90 & 2.80 & 4.40 & 3.10 & 2.80 \\
PageBlocks & 49.70 & 41.00 & 37.60 & 53.30 & 42.40 & 29.20 & 51.60 & \underline{55.40}  & 33.30 & 46.00 & 45.70 & 45.40 & 51.30 & 39.60 & 49.10 & 51.70 & 37.80 & \textbf{55.40} & 49.00 \\
pendigits & \textbf{32.90} & 2.90 & 21.20 & 4.70 & 22.20 & 1.50 & 30.60 & 6.40 & 29.30 & 26.10 & \underline{32.70}  & 6.50 & 18.70 & 3.80 & 23.50 & 23.60 & 4.50 & 24.90 & 21.70 \\
Pima & 53.00 & 44.70 & 55.20 & 41.50 & 50.20 & 35.00 & 50.50 & 53.30 & \textbf{56.60} & \underline{55.80}  & 53.50 & 55.10 & 44.10 & 47.20 & 50.00 & 54.00 & 48.20 & 54.70 & 54.20 \\
satellite & 61.40 & 39.70 & 56.60 & 58.30 & 43.30 & 41.80 & 52.20 & 49.80 & 67.20 & 65.90 & 54.70 & 50.00 & 61.90 & 37.70 & 57.60 & 59.60 & 47.20 & \underline{71.70}  & \textbf{75.10} \\
satimage-2 & 97.10 & 8.80 & 76.50 & 22.10 & 8.10 & 2.60 & 64.50 & 43.60 & 78.00 & 93.40 & 97.10 & 39.10 & 80.50 & 4.30 & 82.70 & 85.70 & 26.10 & \underline{97.30}  & \textbf{97.30} \\
shuttle & 79.90 & 12.20 & \underline{96.60}  & 93.20 & 81.80 & 12.40 & 90.40 & 88.20 & 96.40 & \textbf{97.60} & 32.70 & 20.40 & 48.80 & 13.80 & 85.30 & 92.40 & 20.30 & 92.00 & 92.40 \\
skin & 28.30 & 16.40 & 18.00 & N/A & 26.30 & 19.10 & 18.40 & 28.60 & 23.70 & 26.10 & 25.60 & 28.70 & 18.40 & 18.30 & 19.00 & 17.40 & 24.60 & \textbf{28.90} & \underline{28.70}  \\
smtp & 24.20 & 61.10 & 1.10 & 50.00 & 0.20 & 50.00 & 50.00 & 34.50 & 35.20 & 1.20 & 66.70 & \underline{66.70}  & 35.80 & 20.70 & 18.90 & \textbf{66.70} & 33.40 & 26.70 & 1.60 \\
SpamBase & 41.20 & 34.70 & \textbf{56.70} & N/A & 38.00 & 39.70 & \underline{54.00}  & 40.10 & 50.00 & 51.80 & 42.20 & 41.40 & 35.90 & 35.20 & 40.10 & 41.60 & 40.00 & 41.70 & 41.70 \\
speech & 2.00 & 2.20 & 1.90 & 2.00 & \underline{2.80}  & 1.60 & 2.00 & \textbf{2.80} & 2.10 & 2.30 & 2.00 & 2.00 & 1.80 & 2.50 & 2.00 & 2.00 & 2.10 & 1.70 & 1.70 \\
Stamps & 24.50 & 16.50 & 43.10 & 43.70 & \underline{47.40}  & 12.10 & 33.20 & 35.00 & 35.20 & 39.50 & 35.60 & 23.50 & 34.60 & 21.30 & 31.40 & 41.10 & 20.30 & 42.40 & \textbf{50.90} \\
thyroid & 29.90 & 28.50 & 19.60 & 16.10 & 10.60 & 2.70 & 51.10 & 31.70 & 51.00 & \textbf{63.10} & 31.70 & 35.00 & 14.70 & 20.80 & 21.20 & 44.30 & 23.60 & \underline{61.00}  & 60.10 \\
vertebral & 11.40 & 13.80 & 8.90 & \textbf{15.20} & 11.60 & 10.60 & 11.80 & 11.40 & 9.20 & 10.50 & 10.50 & 10.60 & 9.70 & \underline{14.20}  & 10.90 & 10.50 & 11.80 & 9.80 & 13.00 \\
vowels & 35.10 & \underline{56.00}  & 4.10 & 12.20 & 3.60 & 4.60 & 10.60 & 29.20 & 13.40 & 15.10 & 49.10 & \textbf{63.40} & 13.80 & 34.40 & 8.20 & 8.90 & 38.90 & 26.50 & 32.40 \\
Waveform & \underline{17.90}  & 14.10 & 6.90 & 3.10 & 4.30 & 4.40 & 4.80 & 4.30 & 5.90 & 6.20 & \textbf{19.70} & 13.00 & 4.70 & 11.30 & 4.40 & 5.80 & 9.70 & 6.50 & 7.80 \\
WBC & 67.30 & 9.70 & 86.20 & N/A & 33.40 & 9.00 & 86.20 & 44.30 & 73.60 & \textbf{90.50} & 71.90 & 66.60 & 78.70 & 5.60 & \underline{89.90}  & 82.30 & 54.00 & 68.70 & 83.10 \\
WDBC & 83.60 & 50.50 & \underline{84.80}  & 18.50 & 28.90 & 7.60 & 57.90 & 35.60 & \textbf{89.00} & 78.50 & 12.30 & 43.70 & 66.10 & 14.90 & 71.90 & 75.50 & 35.60 & 63.00 & 60.00 \\
Wilt & 3.70 & 5.00 & 3.70 & 4.00 & 4.60 & 4.70 & 3.90 & \textbf{7.20} & 3.80 & 4.20 & 3.80 & 4.70 & 3.40 & 5.00 & 3.60 & 3.10 & \underline{5.50}  & 4.80 & 5.20 \\
wine & 6.00 & 8.50 & 45.70 & 17.50 & 24.40 & 18.80 & 23.50 & 10.70 & 43.10 & 26.00 & 6.30 & 8.40 & \underline{48.80}  & 7.80 & 21.60 & 30.90 & 8.00 & 21.40 & \textbf{49.60} \\
WPBC & 21.10 & 21.30 & 22.80 & 22.50 & 22.90 & 25.00 & 21.20 & 21.60 & 23.00 & 22.40 & 20.60 & 21.50 & \underline{25.40}  & 20.30 & 22.90 & 23.00 & \textbf{25.60} & 22.70 & 24.90 \\
yeast & 31.00 & 31.30 & 30.70 & 29.90 & 27.40 & 30.40 & \underline{33.30}  & 29.10 & 32.70 & 29.80 & 30.00 & 29.30 & \textbf{33.30} & 31.60 & 29.80 & 29.90 & 30.00 & 28.70 & 29.30 \\
    
    % ALOI  & 0.045  & 0.068  & 0.036  & 0.043  & 0.041  & 0.037  & 0.039  & 0.048  & 0.037  & 0.039  & 0.047  & 0.060  & 0.045  & 0.081  & 0.050  & 0.042  & 0.060  & 0.040  & 0.040  \\
    % annthyroid & 0.137  & 0.144  & 0.166  & 0.096  & 0.100  & 0.218  & 0.254  & 0.136  & 0.170  & 0.305  & 0.154  & 0.167  & 0.071  & 0.157  & 0.104  & 0.161  & 0.188  & 0.264  & 0.250  \\
    % backdoor & 0.070  & 0.238  & 0.077  & 0.055  & 0.068  & 0.557  & 0.107  & 0.564  & 0.050  & 0.048  & 0.155  & 0.444  & 0.138  & 0.261  & 0.088  & 0.313  & 0.371  & 0.378  & 0.364  \\
    % breastw & 0.919  & 0.276  & 0.994  & N/A   & 0.968  & 0.486  & 0.985  & 0.914  & 0.977  & 0.960  & 0.922  & 0.922  & 0.970  & 0.285  & 0.827  & 0.951  & 0.849  & 0.945  & 0.959  \\
    % campaign & 0.209  & 0.130  & 0.386  & 0.145  & 0.196  & 0.168  & 0.367  & 0.294  & 0.380  & 0.323  & 0.189  & 0.272  & 0.141  & 0.146  & 0.292  & 0.279  & 0.191  & 0.277  & 0.271  \\
    % cardio & 0.619  & 0.287  & 0.604  & 0.289  & 0.543  & 0.225  & 0.597  & 0.510  & 0.521  & 0.599  & 0.382  & 0.407  & 0.534  & 0.238  & 0.629  & 0.661  & 0.285  & 0.547  & 0.563  \\
    % Cardiotocography & 0.454  & 0.282  & 0.405  & 0.306  & 0.477  & 0.349  & 0.499  & 0.365  & 0.383  & 0.415  & 0.356  & 0.348  & 0.480  & 0.307  & 0.526  & 0.480  & 0.280  & 0.374  & 0.374  \\
    % celeba & 0.112  & 0.018  & 0.137  & 0.019  & 0.175  & 0.027  & 0.140  & 0.101  & 0.138  & 0.090  & 0.032  & 0.031  & 0.040  & 0.017  & 0.107  & 0.159  & 0.024  & 0.151  & 0.147  \\
    % census & 0.075  & 0.049  & 0.099  & 0.090  & 0.109  & 0.084  & 0.095  & 0.097  & 0.087  & 0.078  & 0.081  & 0.090  & 0.050  & 0.055  & 0.068  & 0.100  & 0.085  & 0.097  & 0.098  \\
    % cover & 0.045  & 0.040  & 0.114  & 0.276  & 0.015  & 0.033  & 0.171  & 0.104  & 0.068  & 0.089  & 0.098  & 0.062  & 0.131  & 0.081  & 0.114  & 0.098  & 0.039  & 0.092  & 0.039  \\
    % donors & 0.180  & 0.089  & 0.216  & 0.107  & 0.184  & 0.177  & 0.270  & 0.147  & 0.244  & 0.127  & N/A   & 0.160  & 0.039  & 0.085  & 0.104  & 0.179  & 0.103  & 0.141  & 0.142  \\
    % fault & 0.468  & 0.416  & 0.305  & 0.335  & 0.338  & 0.355  & 0.319  & 0.430  & 0.365  & 0.411  & 0.518  & 0.545  & 0.310  & 0.384  & 0.384  & 0.328  & 0.480  & 0.384  & 0.337  \\
    % fraud & 0.392  & 0.215  & 0.428  & 0.157  & 0.035  & 0.215  & 0.374  & 0.118  & 0.280  & 0.217  & 0.395  & 0.376  & 0.396  & 0.466  & 0.403  & 0.229  & 0.175  & 0.366  & 0.423  \\
    % glass & 0.116  & 0.118  & 0.098  & 0.246  & 0.097  & 0.085  & 0.154  & 0.128  & 0.118  & 0.110  & 0.147  & 0.203  & 0.134  & 0.201  & 0.080  & 0.100  & 0.187  & 0.133  & 0.153  \\
    % Hepatitis & 0.365  & 0.144  & 0.415  & 0.229  & 0.195  & 0.300  & 0.328  & 0.332  & 0.377  & 0.263  & 0.251  & 0.220  & 0.309  & 0.137  & 0.294  & 0.366  & 0.247  & 0.361  & 0.434  \\
    % http  & 0.475  & 0.096  & 0.352  & N/A   & 0.440  & 0.134  & 0.166  & 0.554  & 0.448  & 0.908  & 0.451  & 0.007  & 0.007  & 0.038  & 0.469  & 0.564  & 0.083  & 0.435  & 0.435  \\
    % InternetAds & 0.544  & 0.387  & 0.510  & N/A   & 0.327  & 0.319  & 0.511  & 0.384  & 0.540  & 0.486  & 0.501  & 0.432  & 0.239  & 0.401  & 0.547  & 0.325  & 0.269  & 0.231  & 0.242  \\
    % Ionosphere & 0.898  & 0.829  & 0.699  & 0.650  & 0.476  & 0.432  & 0.647  & 0.906  & 0.418  & 0.804  & 0.914  & 0.904  & 0.730  & 0.881  & 0.745  & 0.739  & 0.859  & 0.895  & 0.876  \\
    % landsat & 0.311  & 0.250  & 0.175  & 0.245  & 0.156  & 0.369  & 0.162  & 0.184  & 0.220  & 0.198  & 0.224  & 0.246  & 0.189  & 0.247  & 0.162  & 0.162  & 0.264  & 0.208  & 0.233  \\
    % letter & 0.139  & 0.214  & 0.068  & 0.117  & 0.063  & 0.088  & 0.076  & 0.183  & 0.084  & 0.085  & 0.153  & 0.300  & 0.069  & 0.340  & 0.061  & 0.069  & 0.286  & 0.137  & 0.143  \\
    % Lymphography & 0.973  & 0.367  & 0.887  & 0.195  & 0.123  & 0.346  & 0.909  & 0.715  & 0.918  & 0.973  & 1.000  & 0.387  & 0.445  & 0.231  & 0.936  & 0.970  & 0.220  & 0.917  & 0.967  \\
    % magic & 0.688  & 0.541  & 0.592  & 0.469  & 0.598  & 0.487  & 0.537  & 0.667  & 0.624  & 0.647  & 0.683  & 0.756  & 0.585  & 0.548  & 0.514  & 0.593  & 0.679  & 0.658  & 0.650  \\
    % mammography & 0.111  & 0.111  & 0.407  & N/A   & 0.161  & 0.051  & 0.413  & 0.211  & 0.213  & 0.207  & N/A   & 0.159  & 0.147  & 0.098  & 0.129  & 0.192  & 0.134  & 0.159  & 0.063  \\
    % mnist & 0.306  & 0.255  & 0.213  & 0.237  & 0.236  & 0.202  & 0.175  & 0.387  & 0.125  & 0.277  & 0.371  & 0.355  & 0.259  & 0.209  & 0.332  & 0.399  & 0.192  & 0.412  & 0.419  \\
    % musk  & 1.000  & 0.026  & 0.348  & 0.328  & 0.029  & 0.088  & 0.501  & 0.903  & 1.000  & 0.996  & 0.375  & 0.097  & 0.476  & 0.028  & 0.106  & 0.999  & 0.076  & 0.977  & 1.000  \\
    % optdigits & 0.102  & 0.044  & 0.044  & 0.056  & 0.026  & 0.022  & 0.035  & 0.027  & 0.100  & 0.051  & 0.095  & 0.031  & 0.040  & 0.061  & 0.029  & 0.028  & 0.044  & 0.031  & 0.028  \\
    % PageBlocks & 0.497  & 0.410  & 0.376  & 0.533  & 0.424  & 0.292  & 0.516  & 0.554  & 0.333  & 0.460  & 0.457  & 0.454  & 0.513  & 0.396  & 0.491  & 0.517  & 0.378  & 0.554  & 0.490  \\
    % pendigits & 0.329  & 0.029  & 0.212  & 0.047  & 0.222  & 0.015  & 0.306  & 0.064  & 0.293  & 0.261  & 0.327  & 0.065  & 0.187  & 0.038  & 0.235  & 0.236  & 0.045  & 0.249  & 0.217  \\
    % Pima  & 0.530  & 0.447  & 0.552  & 0.415  & 0.502  & 0.350  & 0.505  & 0.533  & 0.566  & 0.558  & 0.535  & 0.551  & 0.441  & 0.472  & 0.500  & 0.540  & 0.482  & 0.547  & 0.542  \\
    % satellite & 0.614  & 0.397  & 0.566  & 0.583  & 0.433  & 0.418  & 0.522  & 0.498  & 0.672  & 0.659  & 0.547  & 0.500  & 0.619  & 0.377  & 0.576  & 0.596  & 0.472  & 0.717  & 0.751  \\
    % satimage-2 & 0.971  & 0.088  & 0.765  & 0.221  & 0.081  & 0.026  & 0.645  & 0.436  & 0.780  & 0.934  & 0.971  & 0.391  & 0.805  & 0.043  & 0.827  & 0.857  & 0.261  & 0.973  & 0.973  \\
    % shuttle & 0.799  & 0.122  & 0.966  & 0.932  & 0.818  & 0.124  & 0.904  & 0.882  & 0.964  & 0.976  & 0.327  & 0.204  & 0.488  & 0.138  & 0.853  & 0.924  & 0.203  & 0.920  & 0.924  \\
    % skin  & 0.283  & 0.164  & 0.180  & N/A   & 0.263  & 0.191  & 0.184  & 0.286  & 0.237  & 0.261  & 0.256  & 0.287  & 0.184  & 0.183  & 0.190  & 0.174  & 0.246  & 0.289  & 0.287  \\
    % smtp  & 0.242  & 0.611  & 0.011  & 0.500  & 0.002  & 0.500  & 0.500  & 0.345  & 0.352  & 0.012  & 0.667  & 0.667  & 0.358  & 0.207  & 0.189  & 0.667  & 0.334  & 0.267  & 0.016  \\
    % SpamBase & 0.412  & 0.347  & 0.567  & N/A   & 0.380  & 0.397  & 0.540  & 0.401  & 0.500  & 0.518  & 0.422  & 0.414  & 0.359  & 0.352  & 0.401  & 0.416  & 0.400  & 0.417  & 0.417  \\
    % speech & 0.020  & 0.022  & 0.019  & 0.020  & 0.028  & 0.016  & 0.020  & 0.028  & 0.021  & 0.023  & 0.020  & 0.020  & 0.018  & 0.025  & 0.020  & 0.020  & 0.021  & 0.017  & 0.017  \\
    % Stamps & 0.245  & 0.165  & 0.431  & 0.437  & 0.474  & 0.121  & 0.332  & 0.350  & 0.352  & 0.395  & 0.356  & 0.235  & 0.346  & 0.213  & 0.314  & 0.411  & 0.203  & 0.424  & 0.509  \\
    % thyroid & 0.299  & 0.285  & 0.196  & 0.161  & 0.106  & 0.027  & 0.511  & 0.317  & 0.510  & 0.631  & 0.317  & 0.350  & 0.147  & 0.208  & 0.212  & 0.443  & 0.236  & 0.610  & 0.601  \\
    % vertebral & 0.114  & 0.138  & 0.089  & 0.152  & 0.116  & 0.106  & 0.118  & 0.114  & 0.092  & 0.105  & 0.105  & 0.106  & 0.097  & 0.142  & 0.109  & 0.105  & 0.118  & 0.098  & 0.130  \\
    % vowels & 0.351  & 0.560  & 0.041  & 0.122  & 0.036  & 0.046  & 0.106  & 0.292  & 0.134  & 0.151  & 0.491  & 0.634  & 0.138  & 0.344  & 0.082  & 0.089  & 0.389  & 0.265  & 0.324  \\
    % Waveform & 0.179  & 0.141  & 0.069  & 0.031  & 0.043  & 0.044  & 0.048  & 0.043  & 0.059  & 0.062  & 0.197  & 0.130  & 0.047  & 0.113  & 0.044  & 0.058  & 0.097  & 0.065  & 0.078  \\
    % WBC   & 0.673  & 0.097  & 0.862  & N/A   & 0.334  & 0.090  & 0.862  & 0.443  & 0.736  & 0.905  & 0.719  & 0.666  & 0.787  & 0.056  & 0.899  & 0.823  & 0.540  & 0.687  & 0.831  \\
    % WDBC  & 0.836  & 0.505  & 0.848  & 0.185  & 0.289  & 0.076  & 0.579  & 0.356  & 0.890  & 0.785  & 0.123  & 0.437  & 0.661  & 0.149  & 0.719  & 0.755  & 0.356  & 0.630  & 0.600  \\
    % Wilt  & 0.037  & 0.050  & 0.037  & 0.040  & 0.046  & 0.047  & 0.039  & 0.072  & 0.038  & 0.042  & 0.038  & 0.047  & 0.034  & 0.050  & 0.036  & 0.031  & 0.055  & 0.048  & 0.052  \\
    % wine  & 0.060  & 0.085  & 0.457  & 0.175  & 0.244  & 0.188  & 0.235  & 0.107  & 0.431  & 0.260  & 0.063  & 0.084  & 0.488  & 0.078  & 0.216  & 0.309  & 0.080  & 0.214  & 0.496  \\
    % WPBC  & 0.211  & 0.213  & 0.228  & 0.225  & 0.229  & 0.250  & 0.212  & 0.216  & 0.230  & 0.224  & 0.206  & 0.215  & 0.254  & 0.203  & 0.229  & 0.230  & 0.256  & 0.227  & 0.249  \\
    % yeast & 0.310  & 0.313  & 0.307  & 0.299  & 0.274  & 0.304  & 0.333  & 0.291  & 0.327  & 0.298  & 0.300  & 0.293  & 0.333  & 0.316  & 0.298  & 0.299  & 0.300  & 0.287  & 0.293  \\
    \midrule
    Avg. Rank & 8.0   & 12.4  & 9.4   & 11.7  & 12.4  & 14.0  & 8.6   & 9.1   & 8.2   & 8.0   & 8.6   & 9.1   & 11.2  & 12.2  & 10.5  & 8.5   & 11.1  & \underline{7.9}   & \textbf{7.4}  \\
    \bottomrule
    \end{tabular}%
    \end{adjustbox}
  \label{tab:aucpr}%
\end{table*}%




==> tables/aucroc.tex <==
% Table generated by Excel2LaTeX from sheet 'pivot_aucroc'
\begin{table*}%[htbp]
  \centering
    % \caption{AUCROC of 14 unsupervised algorithms on 47 tabular benchmark datasets.}  
  \caption{AUCROC of 17 unsupervised algorithms on 47 tabular benchmark datasets. 
  In each dataset, the highest score is highlighted in \textbf{bold}, and the second-highest score is \underline{underlined}.
  The table includes three summary statistics for each algorithm: Avg. rank (average ranking across all datasets).
  }

\begin{adjustbox}{max width=\linewidth}

\begin{tabular}{c|ccccccccccccccccc|c}
\toprule
    \textbf{Dataset} & \textbf{CBLOF} & \textbf{COF} & \textbf{COPOD} & \makecell{\textbf{DA} \\ \textbf{GMM}} & \textbf{DCFOD} & \makecell{\textbf{Deep} \\ \textbf{SVDD}} & \textbf{ECOD} & \textbf{GMM} & \textbf{HBOS} & \textbf{IForest} & \textbf{KMeans-$ $-} & \textbf{KNN} & \textbf{LODA} & \textbf{LOF} & \textbf{OCSVM} & \textbf{PCA} & \textbf{SOD} & \textbf{\model} \\
    \midrule
ALOI & 0.553 & \underline{0.647} & 0.537 & 0.520 & 0.528 & 0.505 & 0.563 & 0.590 & 0.526 & 0.567 & 0.549 & 0.615 & 0.513 & \textbf{0.666} & 0.558 & 0.566 & 0.611 & 0.566 \\
annthyroid & 0.623 & 0.659 & 0.768 & 0.565 & 0.550 & 0.761 & \underline{0.787} & 0.625 & 0.601 & \textbf{0.820} & 0.650 & 0.717 & 0.410 & 0.702 & 0.572 & 0.662 & 0.774 & 0.553 \\
backdoor & 0.819 & 0.731 & 0.810 & 0.560 & 0.796 & 0.788 & 0.861 & \textbf{0.927} & 0.716 & 0.722 & 0.891 & 0.806 & 0.664 & 0.858 & 0.850 & 0.802 & 0.688 & \underline{0.892} \\
breastw & 0.969 & 0.388 & \textbf{0.997} & N/A & 0.990 & 0.634 & \underline{0.992} & 0.965 & 0.989 & 0.983 & 0.970 & 0.970 & 0.985 & 0.406 & 0.803 & 0.951 & 0.940 & 0.986 \\
campaign & 0.643 & 0.574 & \underline{0.777} & 0.560 & 0.632 & 0.544 & 0.761 & 0.752 & \textbf{0.785} & 0.717 & 0.635 & 0.723 & 0.517 & 0.590 & 0.657 & 0.728 & 0.692 & 0.736 \\
cardio & 0.906 & 0.714 & 0.923 & 0.750 & 0.939 & 0.534 & 0.936 & 0.907 & 0.847 & 0.932 & 0.789 & 0.766 & 0.903 & 0.663 & \underline{0.939} & \textbf{0.956} & 0.732 & 0.922 \\
Cardiotocography & 0.644 & 0.538 & 0.670 & 0.620 & 0.767 & 0.550 & \textbf{0.784} & 0.603 & 0.609 & 0.676 & 0.614 & 0.562 & 0.737 & 0.595 & \underline{0.779} & 0.747 & 0.517 & 0.583 \\
celeba & 0.740 & 0.386 & 0.757 & 0.447 & \textbf{0.914} & 0.452 & 0.765 & 0.808 & 0.762 & 0.704 & 0.568 & 0.596 & 0.602 & 0.390 & 0.707 & 0.794 & 0.484 & \underline{0.820} \\
census & 0.602 & 0.416 & \underline{0.691} & 0.597 & \textbf{0.728} & 0.542 & 0.676 & 0.682 & 0.649 & 0.595 & 0.633 & 0.669 & 0.371 & 0.475 & 0.549 & 0.687 & 0.621 & 0.678 \\
cover & 0.879 & 0.769 & 0.886 & 0.899 & 0.511 & 0.436 & 0.919 & \underline{0.938} & 0.802 & 0.867 & \textbf{0.939} & 0.860 & 0.923 & 0.846 & 0.926 & 0.937 & 0.745 & 0.806 \\
donors & 0.814 & 0.708 & 0.818 & 0.708 & 0.822 & 0.580 & \textbf{0.890} & 0.812 & 0.784 & 0.777 & N/A & 0.819 & 0.270 & 0.589 & 0.724 & \underline{0.831} & 0.560 & 0.788 \\
fault & 0.657 & 0.621 & 0.439 & 0.459 & 0.457 & 0.476 & 0.454 & 0.613 & 0.513 & 0.570 & \underline{0.694} & \textbf{0.730} & 0.417 & 0.589 & 0.477 & 0.460 & 0.681 & 0.510 \\
fraud & 0.873 & \textbf{0.964} & 0.883 & 0.898 & 0.375 & 0.689 & 0.890 & 0.911 & 0.903 & 0.904 & 0.877 & 0.934 & 0.902 & \underline{0.955} & 0.911 & 0.904 & 0.947 & 0.905 \\
glass & 0.783 & 0.722 & 0.724 & 0.761 & 0.781 & 0.557 & 0.658 & 0.735 & 0.772 & 0.771 & 0.773 & \textbf{0.823} & 0.731 & 0.692 & 0.354 & 0.663 & 0.734 & \underline{0.822} \\
Hepatitis & 0.731 & 0.415 & \textbf{0.821} & 0.548 & 0.484 & 0.574 & 0.752 & 0.709 & 0.799 & 0.698 & 0.646 & 0.528 & 0.649 & 0.381 & 0.677 & 0.759 & 0.678 & \underline{0.806} \\
http & 0.996 & 0.888 & 0.993 & N/A & 0.995 & 0.604 & 0.981 & 0.997 & 0.995 & \textbf{1.000} & 0.996 & 0.034 & 0.125 & 0.275 & 0.996 & \underline{0.997} & 0.780 & 0.995 \\
InternetAds & 0.682 & 0.638 & 0.671 & N/A & 0.635 & 0.642 & 0.671 & \textbf{0.778} & 0.680 & 0.690 & 0.673 & \underline{0.700} & 0.554 & 0.655 & 0.683 & 0.617 & 0.609 & 0.550 \\
Ionosphere & 0.908 & 0.868 & 0.793 & 0.734 & 0.578 & 0.539 & 0.732 & \underline{0.910} & 0.625 & 0.845 & \textbf{0.914} & 0.883 & 0.784 & 0.906 & 0.759 & 0.792 & 0.864 & 0.904 \\
landsat & \textbf{0.637} & 0.535 & 0.415 & 0.439 & 0.334 & \underline{0.625} & 0.361 & 0.446 & 0.551 & 0.476 & 0.553 & 0.580 & 0.382 & 0.539 & 0.361 & 0.358 & 0.595 & 0.574 \\
letter & 0.737 & 0.800 & 0.543 & 0.504 & 0.532 & 0.559 & 0.560 & 0.777 & 0.597 & 0.611 & 0.760 & \textbf{0.862} & 0.502 & \underline{0.845} & 0.462 & 0.503 & 0.841 & 0.738 \\
Lymphography & 0.998 & 0.908 & 0.995 & 0.721 & 0.812 & 0.719 & 0.995 & 0.975 & 0.995 & 0.998 & \textbf{1.000} & 0.559 & 0.855 & 0.899 & 0.995 & \underline{0.998} & 0.712 & 0.997 \\
magic.gamma & 0.746 & 0.666 & 0.683 & 0.586 & 0.730 & 0.595 & 0.641 & 0.739 & 0.709 & 0.732 & \underline{0.759} & \textbf{0.824} & 0.680 & 0.685 & 0.606 & 0.672 & 0.754 & 0.730 \\
mammography & 0.837 & 0.775 & \underline{0.907} & N/A & 0.882 & 0.549 & \textbf{0.908} & 0.861 & 0.863 & 0.864 & N/A & 0.845 & 0.839 & 0.744 & 0.849 & 0.887 & 0.815 & 0.721 \\
mnist & 0.800 & 0.708 & 0.777 & 0.672 & 0.652 & 0.510 & 0.746 & 0.846 & 0.604 & 0.810 & 0.825 & 0.806 & 0.723 & 0.671 & 0.830 & \underline{0.853} & 0.601 & \textbf{0.866} \\
musk & 1.000 & 0.387 & 0.942 & 0.769 & 0.422 & 0.660 & 0.954 & 0.997 & 1.000 & 1.000 & 0.722 & 0.699 & 0.951 & 0.412 & 0.806 & \underline{1.000} & 0.741 & \textbf{1.000} \\
optdigits & \textbf{0.876} & 0.491 & 0.687 & 0.626 & 0.472 & 0.370 & 0.608 & 0.495 & \underline{0.816} & 0.709 & 0.646 & 0.417 & 0.617 & 0.561 & 0.540 & 0.517 & 0.590 & 0.524 \\
PageBlocks & 0.851 & 0.726 & 0.881 & 0.896 & 0.855 & 0.566 & \underline{0.915} & \textbf{0.919} & 0.806 & 0.896 & 0.824 & 0.819 & 0.833 & 0.759 & 0.888 & 0.906 & 0.778 & 0.793 \\
pendigits & \textbf{0.969} & 0.451 & 0.907 & 0.642 & 0.943 & 0.273 & 0.930 & 0.771 & 0.930 & 0.948 & 0.944 & 0.729 & 0.891 & 0.480 & 0.938 & 0.937 & 0.663 & \underline{0.955} \\
Pima & 0.715 & 0.610 & 0.691 & 0.559 & 0.722 & 0.495 & 0.631 & 0.698 & 0.711 & 0.729 & 0.704 & \underline{0.734} & 0.659 & 0.657 & 0.669 & 0.708 & 0.613 & \textbf{0.749} \\
satellite & 0.713 & 0.547 & 0.632 & 0.623 & 0.560 & 0.574 & 0.581 & 0.630 & \underline{0.748} & 0.704 & 0.677 & 0.652 & 0.620 & 0.559 & 0.590 & 0.596 & 0.640 & \textbf{0.777} \\
satimage-2 & 0.998 & 0.567 & 0.972 & 0.963 & 0.860 & 0.557 & 0.963 & 0.987 & 0.976 & 0.992 & \underline{0.999} & 0.926 & 0.976 & 0.474 & 0.973 & 0.976 & 0.831 & \textbf{0.999} \\
shuttle & 0.931 & 0.517 & \underline{0.994} & 0.979 & 0.972 & 0.518 & 0.991 & 0.981 & 0.986 & \textbf{0.996} & 0.700 & 0.696 & 0.609 & 0.571 & 0.974 & 0.986 & 0.695 & 0.987 \\
skin & 0.680 & 0.417 & 0.476 & N/A & 0.643 & 0.457 & 0.491 & \underline{0.714} & 0.602 & 0.682 & 0.655 & \textbf{0.715} & 0.458 & 0.465 & 0.495 & 0.453 & 0.603 & 0.697 \\
smtp & 0.807 & 0.796 & 0.791 & 0.713 & 0.529 & 0.778 & 0.856 & 0.801 & 0.705 & \textbf{0.897} & 0.859 & \underline{0.896} & 0.674 & 0.718 & 0.807 & 0.884 & 0.599 & 0.679 \\
SpamBase & 0.552 & 0.410 & \textbf{0.701} & N/A & 0.503 & 0.503 & \underline{0.669} & 0.521 & 0.647 & 0.648 & 0.563 & 0.534 & 0.420 & 0.433 & 0.525 & 0.547 & 0.523 & 0.544 \\
speech & 0.506 & \underline{0.560} & 0.529 & 0.528 & \textbf{0.565} & 0.468 & 0.509 & 0.538 & 0.506 & 0.507 & 0.507 & 0.510 & 0.498 & 0.525 & 0.502 & 0.508 & 0.559 & 0.481 \\
Stamps & 0.699 & 0.538 & 0.934 & 0.889 & \underline{0.934} & 0.595 & 0.879 & 0.875 & 0.907 & 0.912 & 0.798 & 0.686 & 0.872 & 0.513 & 0.839 & 0.915 & 0.733 & \textbf{0.942} \\
thyroid & 0.947 & 0.909 & 0.943 & 0.798 & 0.786 & 0.521 & \underline{0.979} & 0.942 & 0.956 & \textbf{0.983} & 0.923 & 0.959 & 0.743 & 0.869 & 0.879 & 0.963 & 0.928 & 0.916 \\
vertebral & 0.410 & 0.487 & 0.256 & \textbf{0.532} & 0.381 & 0.378 & 0.407 & 0.420 & 0.286 & 0.367 & 0.381 & 0.338 & 0.306 & \underline{0.493} & 0.380 & 0.371 & 0.403 & 0.474 \\
vowels & 0.921 & \underline{0.940} & 0.532 & 0.606 & 0.516 & 0.499 & 0.622 & 0.877 & 0.722 & 0.739 & 0.935 & \textbf{0.973} & 0.704 & 0.931 & 0.616 & 0.653 & 0.927 & 0.921 \\
Waveform & 0.713 & 0.726 & \textbf{0.750} & 0.493 & 0.635 & 0.539 & 0.624 & 0.560 & 0.688 & 0.715 & \underline{0.744} & 0.738 & 0.601 & 0.733 & 0.563 & 0.655 & 0.686 & 0.743 \\
WBC & 0.969 & 0.609 & \underline{0.991} & N/A & 0.949 & 0.625 & \textbf{0.991} & 0.956 & 0.987 & 0.990 & 0.974 & 0.906 & 0.969 & 0.542 & 0.990 & 0.982 & 0.946 & 0.989 \\
WDBC & 0.994 & 0.963 & \underline{0.994} & 0.767 & 0.961 & 0.686 & 0.972 & 0.952 & \textbf{0.995} & 0.989 & 0.756 & 0.917 & 0.983 & 0.890 & 0.989 & 0.991 & 0.921 & 0.982 \\
Wilt & 0.345 & 0.497 & 0.334 & 0.373 & 0.447 & 0.459 & 0.363 & \textbf{0.651} & 0.325 & 0.419 & 0.349 & 0.484 & 0.264 & 0.507 & 0.313 & 0.204 & \underline{0.533} & 0.526 \\
wine & 0.271 & 0.444 & 0.887 & 0.617 & 0.822 & 0.643 & 0.772 & 0.631 & \underline{0.914} & 0.804 & 0.274 & 0.450 & 0.901 & 0.377 & 0.731 & 0.844 & 0.461 & \textbf{0.952} \\
WPBC & 0.453 & 0.459 & 0.493 & 0.478 & 0.497 & 0.440 & 0.466 & 0.460 & \underline{0.512} & 0.466 & 0.450 & 0.466 & 0.493 & 0.414 & 0.454 & 0.460 & \textbf{0.513} & 0.499 \\
yeast & \underline{0.450} & 0.445 & 0.370 & 0.411 & 0.342 & 0.434 & 0.438 & 0.407 & 0.396 & 0.378 & 0.427 & 0.391 & 0.446 & \textbf{0.453} & 0.410 & 0.412 & 0.425 & 0.388 \\
\midrule
  Avg. Rank &  7.3   & 12.0  & 7.9   & 12.1  & 10.4  & 14.7  & 7.8   & 7.1   & 8.3   & 6.5   & 8.0   & 8.6   & 12.1  & 11.6  & 10.0  & 7.9   & 10.3  & 6.5  \\
\bottomrule
\end{tabular}%

%     \begin{tabular}{c|cccccccccccccc|c}
%     \toprule
%     \textbf{Datasets} & \textbf{CBLOF} & \textbf{COF} & \textbf{COPOD} & \textbf{DAGMM} & \textbf{DeepSVDD} & \textbf{ECOD} & \textbf{HBOS} & \textbf{IForest} & \textbf{KNN} & \textbf{LODA} & \textbf{LOF} & \textbf{OCSVM} & \textbf{PCA} & \textbf{SOD} & \textbf{\model} \\
%     \midrule

% ALOI & 0.553 & \underline{0.647} & 0.537 & 0.520 & 0.505 & 0.563 & 0.526 & 0.567 & 0.615 & 0.513 & \textbf{0.666} & 0.558 & 0.566 & 0.611 & 0.566 \\
% annthyroid & 0.623 & 0.659 & 0.768 & 0.565 & 0.761 & \underline{0.787} & 0.601 & \textbf{0.820} & 0.717 & 0.410 & 0.702 & 0.572 & 0.662 & 0.774 & 0.553 \\
% backdoor & 0.819 & 0.731 & 0.810 & 0.560 & 0.788 & \underline{0.861} & 0.716 & 0.722 & 0.806 & 0.664 & 0.858 & 0.850 & 0.802 & 0.688 & \textbf{0.892} \\
% breastw & 0.969 & 0.388 & \textbf{0.997} & N/A & 0.634 & \underline{0.992} & 0.989 & 0.983 & 0.970 & 0.985 & 0.406 & 0.803 & 0.951 & 0.940 & 0.986 \\
% campaign & 0.643 & 0.574 & \underline{0.777} & 0.560 & 0.544 & 0.761 & \textbf{0.785} & 0.717 & 0.723 & 0.517 & 0.590 & 0.657 & 0.728 & 0.692 & 0.736 \\
% cardio & 0.906 & 0.714 & 0.923 & 0.750 & 0.534 & 0.936 & 0.847 & 0.932 & 0.766 & 0.903 & 0.663 & \underline{0.939} & \textbf{0.956} & 0.732 & 0.922 \\
% Cardiotocography & 0.644 & 0.538 & 0.670 & 0.620 & 0.550 & \textbf{0.784} & 0.609 & 0.676 & 0.562 & 0.737 & 0.595 & \underline{0.779} & 0.747 & 0.517 & 0.583 \\
% celeba & 0.740 & 0.386 & 0.757 & 0.447 & 0.452 & 0.765 & 0.762 & 0.704 & 0.596 & 0.602 & 0.390 & 0.707 & \underline{0.794} & 0.484 & \textbf{0.820} \\
% census & 0.602 & 0.416 & \textbf{0.691} & 0.597 & 0.542 & 0.676 & 0.649 & 0.595 & 0.669 & 0.371 & 0.475 & 0.549 & \underline{0.687} & 0.621 & 0.678 \\
% cover & 0.879 & 0.769 & 0.886 & 0.899 & 0.436 & 0.919 & 0.802 & 0.867 & 0.860 & 0.923 & 0.846 & \underline{0.926} & \textbf{0.937} & 0.745 & 0.806 \\
% donors & 0.814 & 0.708 & 0.818 & 0.708 & 0.580 & \textbf{0.890} & 0.784 & 0.777 & 0.819 & 0.270 & 0.589 & 0.724 & \underline{0.831} & 0.560 & 0.788 \\
% fault & 0.657 & 0.621 & 0.439 & 0.459 & 0.476 & 0.454 & 0.513 & 0.570 & \textbf{0.730} & 0.417 & 0.589 & 0.477 & 0.460 & \underline{0.681} & 0.510 \\
% fraud & 0.873 & \textbf{0.964} & 0.883 & 0.898 & 0.689 & 0.890 & 0.903 & 0.904 & 0.934 & 0.902 & \underline{0.955} & 0.911 & 0.904 & 0.947 & 0.905 \\
% glass & 0.783 & 0.722 & 0.724 & 0.761 & 0.557 & 0.658 & 0.772 & 0.771 & \textbf{0.823} & 0.731 & 0.692 & 0.354 & 0.663 & 0.734 & \underline{0.822} \\
% Hepatitis & 0.731 & 0.415 & \textbf{0.821} & 0.548 & 0.574 & 0.752 & 0.799 & 0.698 & 0.528 & 0.649 & 0.381 & 0.677 & 0.759 & 0.678 & \underline{0.806} \\
% http & 0.996 & 0.888 & 0.993 & N/A & 0.604 & 0.981 & 0.995 & \textbf{1.000} & 0.034 & 0.125 & 0.275 & 0.996 & \underline{0.997} & 0.780 & 0.995 \\
% InternetAds & 0.682 & 0.638 & 0.671 & N/A & 0.642 & 0.671 & 0.680 & \underline{0.690} & \textbf{0.700} & 0.554 & 0.655 & 0.683 & 0.617 & 0.609 & 0.550 \\
% Ionosphere & \textbf{0.908} & 0.868 & 0.793 & 0.734 & 0.539 & 0.732 & 0.625 & 0.845 & 0.883 & 0.784 & \underline{0.906} & 0.759 & 0.792 & 0.864 & 0.904 \\
% landsat & \textbf{0.637} & 0.535 & 0.415 & 0.439 & \underline{0.625} & 0.361 & 0.551 & 0.476 & 0.580 & 0.382 & 0.539 & 0.361 & 0.358 & 0.595 & 0.574 \\
% letter & 0.737 & 0.800 & 0.543 & 0.504 & 0.559 & 0.560 & 0.597 & 0.611 & \textbf{0.862} & 0.502 & \underline{0.845} & 0.462 & 0.503 & 0.841 & 0.738 \\
% Lymphography & 0.998 & 0.908 & 0.995 & 0.721 & 0.719 & 0.995 & 0.995 & \underline{0.998} & 0.559 & 0.855 & 0.899 & 0.995 & \textbf{0.998} & 0.712 & 0.997 \\
% magic.gamma & 0.746 & 0.666 & 0.683 & 0.586 & 0.595 & 0.641 & 0.709 & 0.732 & \textbf{0.824} & 0.680 & 0.685 & 0.606 & 0.672 & \underline{0.754} & 0.730 \\
% mammography & 0.837 & 0.775 & \underline{0.907} & N/A & 0.549 & \textbf{0.908} & 0.863 & 0.864 & 0.845 & 0.839 & 0.744 & 0.849 & 0.887 & 0.815 & 0.721 \\
% mnist & 0.800 & 0.708 & 0.777 & 0.672 & 0.510 & 0.746 & 0.604 & 0.810 & 0.806 & 0.723 & 0.671 & 0.830 & \underline{0.853} & 0.601 & \textbf{0.866} \\
% musk & 1.000 & 0.387 & 0.942 & 0.769 & 0.660 & 0.954 & 1.000 & 1.000 & 0.699 & 0.951 & 0.412 & 0.806 & \underline{1.000} & 0.741 & \textbf{1.000} \\
% optdigits & \textbf{0.876} & 0.491 & 0.687 & 0.626 & 0.370 & 0.608 & \underline{0.816} & 0.709 & 0.417 & 0.617 & 0.561 & 0.540 & 0.517 & 0.590 & 0.524 \\
% PageBlocks & 0.851 & 0.726 & 0.881 & 0.896 & 0.566 & \textbf{0.915} & 0.806 & 0.896 & 0.819 & 0.833 & 0.759 & 0.888 & \underline{0.906} & 0.778 & 0.793 \\
% pendigits & \textbf{0.969} & 0.451 & 0.907 & 0.642 & 0.273 & 0.930 & 0.930 & 0.948 & 0.729 & 0.891 & 0.480 & 0.938 & 0.937 & 0.663 & \underline{0.955} \\
% Pima & 0.715 & 0.610 & 0.691 & 0.559 & 0.495 & 0.631 & 0.711 & 0.729 & \underline{0.734} & 0.659 & 0.657 & 0.669 & 0.708 & 0.613 & \textbf{0.749} \\
% satellite & 0.713 & 0.547 & 0.632 & 0.623 & 0.574 & 0.581 & \underline{0.748} & 0.704 & 0.652 & 0.620 & 0.559 & 0.590 & 0.596 & 0.640 & \textbf{0.777} \\
% satimage-2 & \underline{0.998} & 0.567 & 0.972 & 0.963 & 0.557 & 0.963 & 0.976 & 0.992 & 0.926 & 0.976 & 0.474 & 0.973 & 0.976 & 0.831 & \textbf{0.999} \\
% shuttle & 0.931 & 0.517 & \underline{0.994} & 0.979 & 0.518 & 0.991 & 0.986 & \textbf{0.996} & 0.696 & 0.609 & 0.571 & 0.974 & 0.986 & 0.695 & 0.987 \\
% skin & 0.680 & 0.417 & 0.476 & N/A & 0.457 & 0.491 & 0.602 & 0.682 & \textbf{0.715} & 0.458 & 0.465 & 0.495 & 0.453 & 0.603 & \underline{0.697} \\
% smtp & 0.807 & 0.796 & 0.791 & 0.713 & 0.778 & 0.856 & 0.705 & \textbf{0.897} & \underline{0.896} & 0.674 & 0.718 & 0.807 & 0.884 & 0.599 & 0.679 \\
% SpamBase & 0.552 & 0.410 & \textbf{0.701} & N/A & 0.503 & \underline{0.669} & 0.647 & 0.648 & 0.534 & 0.420 & 0.433 & 0.525 & 0.547 & 0.523 & 0.544 \\
% speech & 0.506 & \textbf{0.560} & 0.529 & 0.528 & 0.468 & 0.509 & 0.506 & 0.507 & 0.510 & 0.498 & 0.525 & 0.502 & 0.508 & \underline{0.559} & 0.481 \\
% Stamps & 0.699 & 0.538 & \underline{0.934} & 0.889 & 0.595 & 0.879 & 0.907 & 0.912 & 0.686 & 0.872 & 0.513 & 0.839 & 0.915 & 0.733 & \textbf{0.942} \\
% thyroid & 0.947 & 0.909 & 0.943 & 0.798 & 0.521 & \underline{0.979} & 0.956 & \textbf{0.983} & 0.959 & 0.743 & 0.869 & 0.879 & 0.963 & 0.928 & 0.916 \\
% vertebral & 0.410 & 0.487 & 0.256 & \textbf{0.532} & 0.378 & 0.407 & 0.286 & 0.367 & 0.338 & 0.306 & \underline{0.493} & 0.380 & 0.371 & 0.403 & 0.474 \\
% vowels & 0.921 & \underline{0.940} & 0.532 & 0.606 & 0.499 & 0.622 & 0.722 & 0.739 & \textbf{0.973} & 0.704 & 0.931 & 0.616 & 0.653 & 0.927 & 0.921 \\
% Waveform & 0.713 & 0.726 & \textbf{0.750} & 0.493 & 0.539 & 0.624 & 0.688 & 0.715 & 0.738 & 0.601 & 0.733 & 0.563 & 0.655 & 0.686 & \underline{0.743} \\
% WBC & 0.969 & 0.609 & \underline{0.991} & N/A & 0.625 & \textbf{0.991} & 0.987 & 0.990 & 0.906 & 0.969 & 0.542 & 0.990 & 0.982 & 0.946 & 0.989 \\
% WDBC & 0.994 & 0.963 & \underline{0.994} & 0.767 & 0.686 & 0.972 & \textbf{0.995} & 0.989 & 0.917 & 0.983 & 0.890 & 0.989 & 0.991 & 0.921 & 0.982 \\
% Wilt & 0.345 & 0.497 & 0.334 & 0.373 & 0.459 & 0.363 & 0.325 & 0.419 & 0.484 & 0.264 & 0.507 & 0.313 & 0.204 & \textbf{0.533} & \underline{0.526} \\
% wine & 0.271 & 0.444 & 0.887 & 0.617 & 0.643 & 0.772 & \underline{0.914} & 0.804 & 0.450 & 0.901 & 0.377 & 0.731 & 0.844 & 0.461 & \textbf{0.952} \\
% WPBC & 0.453 & 0.459 & 0.493 & 0.478 & 0.440 & 0.466 & \underline{0.512} & 0.466 & 0.466 & 0.493 & 0.414 & 0.454 & 0.460 & \textbf{0.513} & 0.499 \\
% yeast & \underline{0.450} & 0.445 & 0.370 & 0.411 & 0.434 & 0.438 & 0.396 & 0.378 & 0.391 & 0.446 & \textbf{0.453} & 0.410 & 0.412 & 0.425 & 0.388 \\

%     \midrule
%     Avg. rank & 6.0   & 9.9   & 6.5   & 10.0  & 12.2  & 6.5   & 6.8   & 5.4   & 7.1   & 10.0  & 9.5   & 8.3   & 6.6   & 8.5   & 5.4 \\
%     Win Nums & 5     & 2     & 5     & 1     & 0     & 5     & 3     & 5     & 7     & 0     & 2     & 0     & 3     & 2     & 8 \\
%     Top3 Nums & 14    & 5     & 12    & 2     & 1     & 14    & 9     & 13    & 12    & 3     & 9     & 6     & 14    & 9     & 18 \\
%     \bottomrule
%     \end{tabular}%
  
    
\end{adjustbox}
\label{tab:aucroc}%
\end{table*}%




==> tables/aucroc_v2.tex <==
% Table generated by Excel2LaTeX from sheet 'pivot_aucroc'
\begin{table*}[htbp]
  \centering
  \caption{AUCROC of 17 unsupervised algorithms on 47 tabular benchmark datasets. 
  In each dataset, the highest score is highlighted in \textbf{bold}, and the second-highest score is \underline{underlined}.
  The table includes three summary statistics for each algorithm: Avg. Rank (average ranking across all datasets).}
  \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{c|ccccccccccccccccc|cc}
    \toprule
    \textbf{Dataset} & \textbf{CBLOF} & \textbf{COF} & \textbf{COPOD} & \makecell{\textbf{DA} \\ \textbf{GMM}} & \textbf{DCFOD} & \makecell{\textbf{Deep} \\ \textbf{SVDD}} & \textbf{ECOD} & \textbf{GMM} & \textbf{HBOS} & \textbf{IForest} & \textbf{KMeans-$ $-} & \textbf{KNN} & \textbf{LODA} & \textbf{LOF} & \textbf{OCSVM} & \textbf{PCA} & \textbf{SOD} & \makecell{\textbf{\model} \\ \textbf{(Scalar)}}  &   \makecell{\textbf{\model} \\ \textbf{(Vector)}}\\
    \midrule
    
ALOI & 55.30 & \underline{64.70}  & 53.70 & 52.00 & 52.80 & 50.50 & 56.30 & 59.00 & 52.60 & 56.70 & 54.90 & 61.50 & 51.30 & \textbf{66.60} & 55.80 & 56.60 & 61.10 & 56.50 & 56.60 \\
annthyroid & 62.30 & 65.90 & 76.80 & 56.50 & 55.00 & 76.10 & \underline{78.70}  & 62.50 & 60.10 & \textbf{82.00} & 65.00 & 71.70 & 41.00 & 70.20 & 57.20 & 66.20 & 77.40 & 75.30 & 72.70 \\
backdoor & 81.90 & 73.10 & 81.00 & 56.00 & 79.60 & 78.80 & 86.10 & \textbf{92.70} & 71.60 & 72.20 & 89.10 & 80.60 & 66.40 & 85.80 & 85.00 & 80.20 & 68.80 & 87.30 & \underline{89.20}  \\
breastw & 96.90 & 38.80 & \textbf{99.70} & N/A & 99.00 & 63.40 & \underline{99.20}  & 96.50 & 98.90 & 98.30 & 97.00 & 97.00 & 98.50 & 40.60 & 80.30 & 95.10 & 94.00 & 98.10 & 98.60 \\
campaign & 64.30 & 57.40 & \underline{77.70}  & 56.00 & 63.20 & 54.40 & 76.10 & 75.20 & \textbf{78.50} & 71.70 & 63.50 & 72.30 & 51.70 & 59.00 & 65.70 & 72.80 & 69.20 & 73.50 & 73.60 \\
cardio & 90.60 & 71.40 & 92.30 & 75.00 & 93.90 & 53.40 & 93.60 & 90.70 & 84.70 & 93.20 & 78.90 & 76.60 & 90.30 & 66.30 & \underline{93.90}  & \textbf{95.60} & 73.20 & 91.80 & 92.20 \\
Cardiotocography & 64.40 & 53.80 & 67.00 & 62.00 & 76.70 & 55.00 & \textbf{78.40} & 60.30 & 60.90 & 67.60 & 61.40 & 56.20 & 73.70 & 59.50 & \underline{77.90}  & 74.70 & 51.70 & 59.60 & 58.30 \\
celeba & 74.00 & 38.60 & 75.70 & 44.70 & \textbf{91.40} & 45.20 & 76.50 & 80.80 & 76.20 & 70.40 & 56.80 & 59.60 & 60.20 & 39.00 & 70.70 & 79.40 & 48.40 & 81.40 & \underline{82.00}  \\
census & 60.20 & 41.60 & \underline{69.10}  & 59.70 & \textbf{72.80} & 54.20 & 67.60 & 68.20 & 64.90 & 59.50 & 63.30 & 66.90 & 37.10 & 47.50 & 54.90 & 68.70 & 62.10 & 67.90 & 67.80 \\
cover & 87.90 & 76.90 & 88.60 & 89.90 & 51.10 & 43.60 & 91.90 & \underline{93.80}  & 80.20 & 86.70 & \textbf{93.90} & 86.00 & 92.30 & 84.60 & 92.60 & 93.70 & 74.50 & 93.30 & 80.60 \\
donors & 81.40 & 70.80 & 81.80 & 70.80 & 82.20 & 58.00 & \textbf{89.00} & 81.20 & 78.40 & 77.70 & N/A & 81.90 & 27.00 & 58.90 & 72.40 & \underline{83.10}  & 56.00 & 77.00 & 78.80 \\
fault & 65.70 & 62.10 & 43.90 & 45.90 & 45.70 & 47.60 & 45.40 & 61.30 & 51.30 & 57.00 & \underline{69.40}  & \textbf{73.00} & 41.70 & 58.90 & 47.70 & 46.00 & 68.10 & 55.60 & 51.00 \\
fraud & 87.30 & \textbf{96.40} & 88.30 & 89.80 & 37.50 & 68.90 & 89.00 & 91.10 & 90.30 & 90.40 & 87.70 & 93.40 & 90.20 & \underline{95.50}  & 91.10 & 90.40 & 94.70 & 90.50 & 90.50 \\
glass & 78.30 & 72.20 & 72.40 & 76.10 & 78.10 & 55.70 & 65.80 & 73.50 & 77.20 & 77.10 & 77.30 & \textbf{82.30} & 73.10 & 69.20 & 35.40 & 66.30 & 73.40 & 79.50 & \underline{82.20}  \\
Hepatitis & 73.10 & 41.50 & \textbf{82.10} & 54.80 & 48.40 & 57.40 & 75.20 & 70.90 & 79.90 & 69.80 & 64.60 & 52.80 & 64.90 & 38.10 & 67.70 & 75.90 & 67.80 & 75.50 & \underline{80.60}  \\
http & 99.60 & 88.80 & 99.30 & N/A & 99.50 & 60.40 & 98.10 & 99.70 & 99.50 & \textbf{100.00} & 99.60 & 3.40 & 12.50 & 27.50 & 99.60 & \underline{99.70}  & 78.00 & 99.50 & 99.50 \\
InternetAds & 68.20 & 63.80 & 67.10 & N/A & 63.50 & 64.20 & 67.10 & \textbf{77.80} & 68.00 & 69.00 & 67.30 & \underline{70.00}  & 55.40 & 65.50 & 68.30 & 61.70 & 60.90 & 53.70 & 55.00 \\
Ionosphere & 90.80 & 86.80 & 79.30 & 73.40 & 57.80 & 53.90 & 73.20 & 91.00 & 62.50 & 84.50 & \underline{91.40}  & 88.30 & 78.40 & 90.60 & 75.90 & 79.20 & 86.40 & \textbf{92.00} & 90.40 \\
landsat & \textbf{63.70} & 53.50 & 41.50 & 43.90 & 33.40 & \underline{62.50}  & 36.10 & 44.60 & 55.10 & 47.60 & 55.30 & 58.00 & 38.20 & 53.90 & 36.10 & 35.80 & 59.50 & 49.60 & 57.40 \\
letter & 73.70 & 80.00 & 54.30 & 50.40 & 53.20 & 55.90 & 56.00 & 77.70 & 59.70 & 61.10 & 76.00 & \textbf{86.20} & 50.20 & \underline{84.50}  & 46.20 & 50.30 & 84.10 & 71.20 & 73.80 \\
Lymphography & 99.80 & 90.80 & 99.50 & 72.10 & 81.20 & 71.90 & 99.50 & 97.50 & 99.50 & 99.80 & \textbf{100.00} & 55.90 & 85.50 & 89.90 & 99.50 & \underline{99.80}  & 71.20 & 99.30 & 99.70 \\
magic & 74.60 & 66.60 & 68.30 & 58.60 & 73.00 & 59.50 & 64.10 & 73.90 & 70.90 & 73.20 & \underline{75.90}  & \textbf{82.40} & 68.00 & 68.50 & 60.60 & 67.20 & 75.40 & 72.80 & 73.00 \\
mammography & 83.70 & 77.50 & \underline{90.70}  & N/A & 88.20 & 54.90 & \textbf{90.80} & 86.10 & 86.30 & 86.40 & N/A & 84.50 & 83.90 & 74.40 & 84.90 & 88.70 & 81.50 & 85.10 & 72.10 \\
mnist & 80.00 & 70.80 & 77.70 & 67.20 & 65.20 & 51.00 & 74.60 & 84.60 & 60.40 & 81.00 & 82.50 & 80.60 & 72.30 & 67.10 & 83.00 & 85.30 & 60.10 & \underline{86.00}  & \textbf{86.60} \\
musk & 100.00 & 38.70 & 94.20 & 76.90 & 42.20 & 66.00 & 95.40 & 99.70 & 100.00 & 100.00 & 72.20 & 69.90 & 95.10 & 41.20 & 80.60 & \underline{100.00}  & 74.10 & 99.90 & \textbf{100.00} \\
optdigits & \textbf{87.60} & 49.10 & 68.70 & 62.60 & 47.20 & 37.00 & 60.80 & 49.50 & \underline{81.60}  & 70.90 & 64.60 & 41.70 & 61.70 & 56.10 & 54.00 & 51.70 & 59.00 & 56.20 & 52.40 \\
PageBlocks & 85.10 & 72.60 & 88.10 & 89.60 & 85.50 & 56.60 & \underline{91.50}  & \textbf{91.90} & 80.60 & 89.60 & 82.40 & 81.90 & 83.30 & 75.90 & 88.80 & 90.60 & 77.80 & 91.20 & 79.30 \\
pendigits & \textbf{96.90} & 45.10 & 90.70 & 64.20 & 94.30 & 27.30 & 93.00 & 77.10 & 93.00 & 94.80 & 94.40 & 72.90 & 89.10 & 48.00 & 93.80 & 93.70 & 66.30 & 95.10 & \underline{95.50}  \\
Pima & 71.50 & 61.00 & 69.10 & 55.90 & 72.20 & 49.50 & 63.10 & 69.80 & 71.10 & 72.90 & 70.40 & 73.40 & 65.90 & 65.70 & 66.90 & 70.80 & 61.30 & \textbf{75.20} & \underline{74.90}  \\
satellite & 71.30 & 54.70 & 63.20 & 62.30 & 56.00 & 57.40 & 58.10 & 63.00 & \underline{74.80}  & 70.40 & 67.70 & 65.20 & 62.00 & 55.90 & 59.00 & 59.60 & 64.00 & 72.50 & \textbf{77.70} \\
satimage-2 & 99.80 & 56.70 & 97.20 & 96.30 & 86.00 & 55.70 & 96.30 & 98.70 & 97.60 & 99.20 & 99.90 & 92.60 & 97.60 & 47.40 & 97.30 & 97.60 & 83.10 & \underline{99.90}  & \textbf{99.90} \\
shuttle & 93.10 & 51.70 & \underline{99.40}  & 97.90 & 97.20 & 51.80 & 99.10 & 98.10 & 98.60 & \textbf{99.60} & 70.00 & 69.60 & 60.90 & 57.10 & 97.40 & 98.60 & 69.50 & 99.20 & 98.70 \\
skin & 68.00 & 41.70 & 47.60 & N/A & 64.30 & 45.70 & 49.10 & 71.40 & 60.20 & 68.20 & 65.50 & \underline{71.50}  & 45.80 & 46.50 & 49.50 & 45.30 & 60.30 & \textbf{72.30} & 69.70 \\
smtp & 80.70 & 79.60 & 79.10 & 71.30 & 52.90 & 77.80 & 85.60 & 80.10 & 70.50 & \textbf{89.70} & 85.90 & \underline{89.60}  & 67.40 & 71.80 & 80.70 & 88.40 & 59.90 & 85.30 & 67.90 \\
SpamBase & 55.20 & 41.00 & \textbf{70.10} & N/A & 50.30 & 50.30 & \underline{66.90}  & 52.10 & 64.70 & 64.80 & 56.30 & 53.40 & 42.00 & 43.30 & 52.50 & 54.70 & 52.30 & 54.20 & 54.40 \\
speech & 50.60 & \underline{56.00}  & 52.90 & 52.80 & \textbf{56.50} & 46.80 & 50.90 & 53.80 & 50.60 & 50.70 & 50.70 & 51.00 & 49.80 & 52.50 & 50.20 & 50.80 & 55.90 & 47.50 & 48.10 \\
Stamps & 69.90 & 53.80 & 93.40 & 88.90 & \underline{93.40}  & 59.50 & 87.90 & 87.50 & 90.70 & 91.20 & 79.80 & 68.60 & 87.20 & 51.30 & 83.90 & 91.50 & 73.30 & 91.40 & \textbf{94.20} \\
thyroid & 94.70 & 90.90 & 94.30 & 79.80 & 78.60 & 52.10 & \underline{97.90}  & 94.20 & 95.60 & \textbf{98.30} & 92.30 & 95.90 & 74.30 & 86.90 & 87.90 & 96.30 & 92.80 & 97.70 & 97.50 \\
vertebral & 41.00 & 48.70 & 25.60 & \textbf{53.20} & 38.10 & 37.80 & 40.70 & 42.00 & 28.60 & 36.70 & 38.10 & 33.80 & 30.60 & \underline{49.30}  & 38.00 & 37.10 & 40.30 & 33.10 & 47.40 \\
vowels & 92.10 & \underline{94.00}  & 53.20 & 60.60 & 51.60 & 49.90 & 62.20 & 87.70 & 72.20 & 73.90 & 93.50 & \textbf{97.30} & 70.40 & 93.10 & 61.60 & 65.30 & 92.70 & 88.40 & 92.10 \\
Waveform & 71.30 & 72.60 & \textbf{75.00} & 49.30 & 63.50 & 53.90 & 62.40 & 56.00 & 68.80 & 71.50 & \underline{74.40}  & 73.80 & 60.10 & 73.30 & 56.30 & 65.50 & 68.60 & 71.80 & 74.30 \\
WBC & 96.90 & 60.90 & \underline{99.10}  & N/A & 94.90 & 62.50 & \textbf{99.10} & 95.60 & 98.70 & 99.00 & 97.40 & 90.60 & 96.90 & 54.20 & 99.00 & 98.20 & 94.60 & 97.70 & 98.90 \\
WDBC & 99.40 & 96.30 & \underline{99.40}  & 76.70 & 96.10 & 68.60 & 97.20 & 95.20 & \textbf{99.50} & 98.90 & 75.60 & 91.70 & 98.30 & 89.00 & 98.90 & 99.10 & 92.10 & 98.10 & 98.20 \\
Wilt & 34.50 & 49.70 & 33.40 & 37.30 & 44.70 & 45.90 & 36.30 & \textbf{65.10} & 32.50 & 41.90 & 34.90 & 48.40 & 26.40 & 50.70 & 31.30 & 20.40 & \underline{53.30}  & 49.00 & 52.60 \\
wine & 27.10 & 44.40 & 88.70 & 61.70 & 82.20 & 64.30 & 77.20 & 63.10 & \underline{91.40}  & 80.40 & 27.40 & 45.00 & 90.10 & 37.70 & 73.10 & 84.40 & 46.10 & 82.70 & \textbf{95.20} \\
WPBC & 45.30 & 45.90 & 49.30 & 47.80 & 49.70 & 44.00 & 46.60 & 46.00 & \underline{51.20}  & 46.60 & 45.00 & 46.60 & 49.30 & 41.40 & 45.40 & 46.00 & \textbf{51.30} & 48.00 & 49.90 \\
yeast & \underline{45.00}  & 44.50 & 37.00 & 41.10 & 34.20 & 43.40 & 43.80 & 40.70 & 39.60 & 37.80 & 42.70 & 39.10 & 44.60 & \textbf{45.30} & 41.00 & 41.20 & 42.50 & 37.50 & 38.80 \\

    % ALOI  & 0.553  & 0.647  & 0.537  & 0.520  & 0.528  & 0.505  & 0.563  & 0.590  & 0.526  & 0.567  & 0.549  & 0.615  & 0.513  & 0.666  & 0.558  & 0.566  & 0.611  & 0.565  & 0.566  \\
    % annthyroid & 0.623  & 0.659  & 0.768  & 0.565  & 0.550  & 0.761  & 0.787  & 0.625  & 0.601  & 0.820  & 0.650  & 0.717  & 0.410  & 0.702  & 0.572  & 0.662  & 0.774  & 0.753  & 0.727  \\
    % backdoor & 0.819  & 0.731  & 0.810  & 0.560  & 0.796  & 0.788  & 0.861  & 0.927  & 0.716  & 0.722  & 0.891  & 0.806  & 0.664  & 0.858  & 0.850  & 0.802  & 0.688  & 0.873  & 0.892  \\
    % breastw & 0.969  & 0.388  & 0.997  & N/A   & 0.990  & 0.634  & 0.992  & 0.965  & 0.989  & 0.983  & 0.970  & 0.970  & 0.985  & 0.406  & 0.803  & 0.951  & 0.940  & 0.981  & 0.986  \\
    % campaign & 0.643  & 0.574  & 0.777  & 0.560  & 0.632  & 0.544  & 0.761  & 0.752  & 0.785  & 0.717  & 0.635  & 0.723  & 0.517  & 0.590  & 0.657  & 0.728  & 0.692  & 0.735  & 0.736  \\
    % cardio & 0.906  & 0.714  & 0.923  & 0.750  & 0.939  & 0.534  & 0.936  & 0.907  & 0.847  & 0.932  & 0.789  & 0.766  & 0.903  & 0.663  & 0.939  & 0.956  & 0.732  & 0.918  & 0.922  \\
    % Cardiotocography & 0.644  & 0.538  & 0.670  & 0.620  & 0.767  & 0.550  & 0.784  & 0.603  & 0.609  & 0.676  & 0.614  & 0.562  & 0.737  & 0.595  & 0.779  & 0.747  & 0.517  & 0.596  & 0.583  \\
    % celeba & 0.740  & 0.386  & 0.757  & 0.447  & 0.914  & 0.452  & 0.765  & 0.808  & 0.762  & 0.704  & 0.568  & 0.596  & 0.602  & 0.390  & 0.707  & 0.794  & 0.484  & 0.814  & 0.820  \\
    % census & 0.602  & 0.416  & 0.691  & 0.597  & 0.728  & 0.542  & 0.676  & 0.682  & 0.649  & 0.595  & 0.633  & 0.669  & 0.371  & 0.475  & 0.549  & 0.687  & 0.621  & 0.679  & 0.678  \\
    % cover & 0.879  & 0.769  & 0.886  & 0.899  & 0.511  & 0.436  & 0.919  & 0.938  & 0.802  & 0.867  & 0.939  & 0.860  & 0.923  & 0.846  & 0.926  & 0.937  & 0.745  & 0.933  & 0.806  \\
    % donors & 0.814  & 0.708  & 0.818  & 0.708  & 0.822  & 0.580  & 0.890  & 0.812  & 0.784  & 0.777  & N/A   & 0.819  & 0.270  & 0.589  & 0.724  & 0.831  & 0.560  & 0.770  & 0.788  \\
    % fault & 0.657  & 0.621  & 0.439  & 0.459  & 0.457  & 0.476  & 0.454  & 0.613  & 0.513  & 0.570  & 0.694  & 0.730  & 0.417  & 0.589  & 0.477  & 0.460  & 0.681  & 0.556  & 0.510  \\
    % fraud & 0.873  & 0.964  & 0.883  & 0.898  & 0.375  & 0.689  & 0.890  & 0.911  & 0.903  & 0.904  & 0.877  & 0.934  & 0.902  & 0.955  & 0.911  & 0.904  & 0.947  & 0.905  & 0.905  \\
    % glass & 0.783  & 0.722  & 0.724  & 0.761  & 0.781  & 0.557  & 0.658  & 0.735  & 0.772  & 0.771  & 0.773  & 0.823  & 0.731  & 0.692  & 0.354  & 0.663  & 0.734  & 0.795  & 0.822  \\
    % Hepatitis & 0.731  & 0.415  & 0.821  & 0.548  & 0.484  & 0.574  & 0.752  & 0.709  & 0.799  & 0.698  & 0.646  & 0.528  & 0.649  & 0.381  & 0.677  & 0.759  & 0.678  & 0.755  & 0.806  \\
    % http  & 0.996  & 0.888  & 0.993  & N/A   & 0.995  & 0.604  & 0.981  & 0.997  & 0.995  & 1.000  & 0.996  & 0.034  & 0.125  & 0.275  & 0.996  & 0.997  & 0.780  & 0.995  & 0.995  \\
    % InternetAds & 0.682  & 0.638  & 0.671  & N/A   & 0.635  & 0.642  & 0.671  & 0.778  & 0.680  & 0.690  & 0.673  & 0.700  & 0.554  & 0.655  & 0.683  & 0.617  & 0.609  & 0.537  & 0.550  \\
    % Ionosphere & 0.908  & 0.868  & 0.793  & 0.734  & 0.578  & 0.539  & 0.732  & 0.910  & 0.625  & 0.845  & 0.914  & 0.883  & 0.784  & 0.906  & 0.759  & 0.792  & 0.864  & 0.920  & 0.904  \\
    % landsat & 0.637  & 0.535  & 0.415  & 0.439  & 0.334  & 0.625  & 0.361  & 0.446  & 0.551  & 0.476  & 0.553  & 0.580  & 0.382  & 0.539  & 0.361  & 0.358  & 0.595  & 0.496  & 0.574  \\
    % letter & 0.737  & 0.800  & 0.543  & 0.504  & 0.532  & 0.559  & 0.560  & 0.777  & 0.597  & 0.611  & 0.760  & 0.862  & 0.502  & 0.845  & 0.462  & 0.503  & 0.841  & 0.712  & 0.738  \\
    % Lymphography & 0.998  & 0.908  & 0.995  & 0.721  & 0.812  & 0.719  & 0.995  & 0.975  & 0.995  & 0.998  & 1.000  & 0.559  & 0.855  & 0.899  & 0.995  & 0.998  & 0.712  & 0.993  & 0.997  \\
    % magic & 0.746  & 0.666  & 0.683  & 0.586  & 0.730  & 0.595  & 0.641  & 0.739  & 0.709  & 0.732  & 0.759  & 0.824  & 0.680  & 0.685  & 0.606  & 0.672  & 0.754  & 0.728  & 0.730  \\
    % mammography & 0.837  & 0.775  & 0.907  & N/A   & 0.882  & 0.549  & 0.908  & 0.861  & 0.863  & 0.864  & N/A   & 0.845  & 0.839  & 0.744  & 0.849  & 0.887  & 0.815  & 0.851  & 0.721  \\
    % mnist & 0.800  & 0.708  & 0.777  & 0.672  & 0.652  & 0.510  & 0.746  & 0.846  & 0.604  & 0.810  & 0.825  & 0.806  & 0.723  & 0.671  & 0.830  & 0.853  & 0.601  & 0.860  & 0.866  \\
    % musk  & 1.000  & 0.387  & 0.942  & 0.769  & 0.422  & 0.660  & 0.954  & 0.997  & 1.000  & 1.000  & 0.722  & 0.699  & 0.951  & 0.412  & 0.806  & 1.000  & 0.741  & 0.999  & 1.000  \\
    % optdigits & 0.876  & 0.491  & 0.687  & 0.626  & 0.472  & 0.370  & 0.608  & 0.495  & 0.816  & 0.709  & 0.646  & 0.417  & 0.617  & 0.561  & 0.540  & 0.517  & 0.590  & 0.562  & 0.524  \\
    % PageBlocks & 0.851  & 0.726  & 0.881  & 0.896  & 0.855  & 0.566  & 0.915  & 0.919  & 0.806  & 0.896  & 0.824  & 0.819  & 0.833  & 0.759  & 0.888  & 0.906  & 0.778  & 0.912  & 0.793  \\
    % pendigits & 0.969  & 0.451  & 0.907  & 0.642  & 0.943  & 0.273  & 0.930  & 0.771  & 0.930  & 0.948  & 0.944  & 0.729  & 0.891  & 0.480  & 0.938  & 0.937  & 0.663  & 0.951  & 0.955  \\
    % Pima  & 0.715  & 0.610  & 0.691  & 0.559  & 0.722  & 0.495  & 0.631  & 0.698  & 0.711  & 0.729  & 0.704  & 0.734  & 0.659  & 0.657  & 0.669  & 0.708  & 0.613  & 0.752  & 0.749  \\
    % satellite & 0.713  & 0.547  & 0.632  & 0.623  & 0.560  & 0.574  & 0.581  & 0.630  & 0.748  & 0.704  & 0.677  & 0.652  & 0.620  & 0.559  & 0.590  & 0.596  & 0.640  & 0.725  & 0.777  \\
    % satimage-2 & 0.998  & 0.567  & 0.972  & 0.963  & 0.860  & 0.557  & 0.963  & 0.987  & 0.976  & 0.992  & 0.999  & 0.926  & 0.976  & 0.474  & 0.973  & 0.976  & 0.831  & 0.999  & 0.999  \\
    % shuttle & 0.931  & 0.517  & 0.994  & 0.979  & 0.972  & 0.518  & 0.991  & 0.981  & 0.986  & 0.996  & 0.700  & 0.696  & 0.609  & 0.571  & 0.974  & 0.986  & 0.695  & 0.992  & 0.987  \\
    % skin  & 0.680  & 0.417  & 0.476  & N/A   & 0.643  & 0.457  & 0.491  & 0.714  & 0.602  & 0.682  & 0.655  & 0.715  & 0.458  & 0.465  & 0.495  & 0.453  & 0.603  & 0.723  & 0.697  \\
    % smtp  & 0.807  & 0.796  & 0.791  & 0.713  & 0.529  & 0.778  & 0.856  & 0.801  & 0.705  & 0.897  & 0.859  & 0.896  & 0.674  & 0.718  & 0.807  & 0.884  & 0.599  & 0.853  & 0.679  \\
    % SpamBase & 0.552  & 0.410  & 0.701  & N/A   & 0.503  & 0.503  & 0.669  & 0.521  & 0.647  & 0.648  & 0.563  & 0.534  & 0.420  & 0.433  & 0.525  & 0.547  & 0.523  & 0.542  & 0.544  \\
    % speech & 0.506  & 0.560  & 0.529  & 0.528  & 0.565  & 0.468  & 0.509  & 0.538  & 0.506  & 0.507  & 0.507  & 0.510  & 0.498  & 0.525  & 0.502  & 0.508  & 0.559  & 0.475  & 0.481  \\
    % Stamps & 0.699  & 0.538  & 0.934  & 0.889  & 0.934  & 0.595  & 0.879  & 0.875  & 0.907  & 0.912  & 0.798  & 0.686  & 0.872  & 0.513  & 0.839  & 0.915  & 0.733  & 0.914  & 0.942  \\
    % thyroid & 0.947  & 0.909  & 0.943  & 0.798  & 0.786  & 0.521  & 0.979  & 0.942  & 0.956  & 0.983  & 0.923  & 0.959  & 0.743  & 0.869  & 0.879  & 0.963  & 0.928  & 0.977  & 0.975  \\
    % vertebral & 0.410  & 0.487  & 0.256  & 0.532  & 0.381  & 0.378  & 0.407  & 0.420  & 0.286  & 0.367  & 0.381  & 0.338  & 0.306  & 0.493  & 0.380  & 0.371  & 0.403  & 0.331  & 0.474  \\
    % vowels & 0.921  & 0.940  & 0.532  & 0.606  & 0.516  & 0.499  & 0.622  & 0.877  & 0.722  & 0.739  & 0.935  & 0.973  & 0.704  & 0.931  & 0.616  & 0.653  & 0.927  & 0.884  & 0.921  \\
    % Waveform & 0.713  & 0.726  & 0.750  & 0.493  & 0.635  & 0.539  & 0.624  & 0.560  & 0.688  & 0.715  & 0.744  & 0.738  & 0.601  & 0.733  & 0.563  & 0.655  & 0.686  & 0.718  & 0.743  \\
    % WBC   & 0.969  & 0.609  & 0.991  & N/A   & 0.949  & 0.625  & 0.991  & 0.956  & 0.987  & 0.990  & 0.974  & 0.906  & 0.969  & 0.542  & 0.990  & 0.982  & 0.946  & 0.977  & 0.989  \\
    % WDBC  & 0.994  & 0.963  & 0.994  & 0.767  & 0.961  & 0.686  & 0.972  & 0.952  & 0.995  & 0.989  & 0.756  & 0.917  & 0.983  & 0.890  & 0.989  & 0.991  & 0.921  & 0.981  & 0.982  \\
    % Wilt  & 0.345  & 0.497  & 0.334  & 0.373  & 0.447  & 0.459  & 0.363  & 0.651  & 0.325  & 0.419  & 0.349  & 0.484  & 0.264  & 0.507  & 0.313  & 0.204  & 0.533  & 0.490  & 0.526  \\
    % wine  & 0.271  & 0.444  & 0.887  & 0.617  & 0.822  & 0.643  & 0.772  & 0.631  & 0.914  & 0.804  & 0.274  & 0.450  & 0.901  & 0.377  & 0.731  & 0.844  & 0.461  & 0.827  & 0.952  \\
    % WPBC  & 0.453  & 0.459  & 0.493  & 0.478  & 0.497  & 0.440  & 0.466  & 0.460  & 0.512  & 0.466  & 0.450  & 0.466  & 0.493  & 0.414  & 0.454  & 0.460  & 0.513  & 0.480  & 0.499  \\
    % yeast & 0.450  & 0.445  & 0.370  & 0.411  & 0.342  & 0.434  & 0.438  & 0.407  & 0.396  & 0.378  & 0.427  & 0.391  & 0.446  & 0.453  & 0.410  & 0.412  & 0.425  & 0.375  & 0.388  \\
    \midrule
    Avg. Rank & 8.0   & 12.8  & 8.5   & 13.0  & 11.2  & 15.7  & 8.4   & 7.8   & 8.9   & \underline{7.0}   & 8.6   & 9.3   & 13.0  & 12.4  & 10.8  & 8.5   & 11.0  & 7.1   & \textbf{6.8}  \\
    \bottomrule
    \end{tabular}%
    \end{adjustbox}
  \label{tab:aucroc}%
\end{table*}%


==> tables/compare_pr.tex <==
% Table generated by Excel2LaTeX from sheet 'pivot_aucpr'
\begin{table*}[htbp]
  \centering
  \caption{AUCPR of 14 unsupervised algorithms on tabular benchmark datasets. 
  In each dataset, the highest score is highlighted in \textbf{bold}, and the second-highest score is \underline{underlined}.
    }
  \begin{adjustbox}{max width=\linewidth}

\begin{tabular}{c|cccccccccccccc|c}
    \toprule
    \textbf{Datasets} & \textbf{CBLOF} & \textbf{COF} & \textbf{COPOD} & \textbf{DAGMM} & \textbf{DeepSVDD} & \textbf{ECOD} & \textbf{HBOS} & \textbf{IForest} & \textbf{KNN} & \textbf{LODA} & \textbf{LOF} & \textbf{OCSVM} & \textbf{PCA} & \textbf{SOD} & \textbf{Galaxy} \\
    \midrule
    
celeba & 0.112 & 0.018 & 0.137 & 0.019 & 0.027 & 0.140 & 0.138 & 0.090 & 0.031 & 0.040 & 0.017 & 0.107 & \textbf{0.159} & 0.024 & \underline{0.145} \\
fraud & 0.392 & 0.215 & 0.428 & 0.157 & 0.215 & 0.374 & 0.280 & 0.217 & 0.376 & 0.396 & \textbf{0.466} & 0.403 & 0.229 & 0.175 & \underline{0.435} \\
Hepatitis & 0.365 & 0.144 & \underline{0.415} & 0.229 & 0.300 & 0.328 & 0.377 & 0.263 & 0.220 & 0.309 & 0.137 & 0.294 & 0.366 & 0.247 & \textbf{0.426} \\
mnist & 0.306 & 0.255 & 0.213 & 0.237 & 0.202 & 0.175 & 0.125 & 0.277 & 0.355 & 0.259 & 0.209 & 0.332 & \underline{0.399} & 0.192 & \textbf{0.412} \\
musk & 1.000 & 0.026 & 0.348 & 0.328 & 0.088 & 0.501 & \underline{1.000} & 0.996 & 0.097 & 0.476 & 0.028 & 0.106 & 0.999 & 0.076 & \textbf{1.000} \\
PageBlocks & 0.497 & 0.410 & 0.376 & \underline{0.533} & 0.292 & 0.516 & 0.333 & 0.460 & 0.454 & 0.513 & 0.396 & 0.491 & 0.517 & 0.378 & \textbf{0.546} \\
satellite & 0.614 & 0.397 & 0.566 & 0.583 & 0.418 & 0.522 & \underline{0.672} & 0.659 & 0.500 & 0.619 & 0.377 & 0.576 & 0.596 & 0.472 & \textbf{0.746} \\
satimage-2 & \underline{0.971} & 0.088 & 0.765 & 0.221 & 0.026 & 0.645 & 0.780 & 0.934 & 0.391 & 0.805 & 0.043 & 0.827 & 0.857 & 0.261 & \textbf{0.972} \\
skin & 0.283 & 0.164 & 0.180 & N/A & 0.191 & 0.184 & 0.237 & 0.261 & \underline{0.287} & 0.184 & 0.183 & 0.190 & 0.174 & 0.246 & \textbf{0.292} \\
Stamps & 0.245 & 0.165 & 0.431 & \underline{0.437} & 0.121 & 0.332 & 0.352 & 0.395 & 0.235 & 0.346 & 0.213 & 0.314 & 0.411 & 0.203 & \textbf{0.482} \\
thyroid & 0.299 & 0.285 & 0.196 & 0.161 & 0.027 & 0.511 & 0.510 & \textbf{0.631} & 0.350 & 0.147 & 0.208 & 0.212 & 0.443 & 0.236 & \underline{0.568} \\
Wilt & 0.037 & 0.050 & 0.037 & 0.040 & 0.047 & 0.039 & 0.038 & 0.042 & 0.047 & 0.034 & 0.050 & 0.036 & 0.031 & \textbf{0.055} & \underline{0.053} \\

    \bottomrule
    \end{tabular}%

    \end{adjustbox}
\label{tab:compare_pr}%
\end{table*}%


==> tables/notations.tex <==

\begin{table}[t]
\centering
\caption{Main notations and descriptions}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{c|l|c} 
\toprule
\textbf{Notation} & \textbf{Description} & \textbf{Type} \\
\midrule
\( N \) & Number of data points & Input \\
\( K \) & Number of prototypes & Input \\
\( D \) & Dimension of features & Input \\
\( d \) & Dimension of representations & Input \\
\( \mathbf{X} \) & Set of Observed data & Input \\
\midrule
% \( \mathbf{x}_i \) & Individual data point in the observed data set & Input \\
\( \Theta \) & Network parameters & Learnable \\
\( \bm{\mu}_k \) & Prototypes of t-distribution & Learnable \\
% \( \mathbf{c}_k \) & Individual latent data prototype & Learnable \\
% \( \Theta^* \) & Optimal network parameters & Learnable \\
\( \Sigma_{k} \) & Scale parameter of t-distribution & Learnable \\
\( \omega_k \) & Prior distribution of cluster & Learnable \\
\midrule
\( \mathbf{Z} \) & Data representation & Output \\
\( \bm{\tau} \) & Soft cluster assignment  & Output \\
\( \mathbf{o} \) & Anomaly score  & Output \\
\midrule
% \( \Gamma \) & Gamma function & - \\
% \( \nu \) & Degrees of freedom in Student's t-distribution & Input \\
\( \vec{{\mathbf{F}}}_{ik} \) & Vector form of gravitational force & Conceptual \\
 % $ {\mathbf{F}}_{ik}$ & Analogy for joint distribution & Conceptual \\
\( \hat{r}_{ik} \) & Unit vector in representation space & Conceptual \\

\bottomrule
\end{tabular}
\end{adjustbox}
\label{table:notations}
\end{table}


==> tables/score.tex <==
\begin{table}[t] 
  \centering
  \caption{Evaluation of Anomaly Score in Ablation Studies.}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabular}{cc|ccc}
    \toprule
    \textbf{Metric} & \textbf{Score} & \textbf{Avg. Rank} & \textbf{Win Nums} & \textbf{Top3 Nums} \\
    \midrule
    % \multirow{2}[0]{*}{AUC-ROC} & $o_i^S$ & 7.4   & 4 & 11 \\
    %       & $o_i^V$ & {5.4}$\uparrow$  & 8$\uparrow$ & 18$\uparrow$ \\
    % \midrule
    % \multirow{2}[0]{*}{AUC-PR} & $o_i^S$ & 8.0 & 2  & 8 \\
    %       & $o_i^V$ & 6.1$\uparrow$   & 7$\uparrow$ & 15$\uparrow$ \\

    \multirow{2}[0]{*}{AUC-ROC} & $o_i^S$ & 6.3   & 1 & 8 \\
          & $o_i^V$ & {3.7}$\uparrow$  & 6 $\uparrow$ & 16 $\uparrow$ \\
    \midrule
    \multirow{2}[0]{*}{AUC-PR} & $o_i^S$ & 7.3 & 2  & 5 \\
          & $o_i^V$ & 4.6 $\uparrow$   & 6 $\uparrow$ & 11 $\uparrow$ \\
    
    \bottomrule
  \end{tabular}
  \label{tab:score}
\end{table}


==> tables/sel30_auc.tex <==

% Table generated by Excel2LaTeX from sheet 'aucroc_with_rank'
\begin{table*}[t]
  \centering
  \caption{AUCROC of 14 unsupervised algorithms on 30 tabular benchmark datasets. 
  % In each dataset, the highest score is highlighted in \textbf{bold}, and the second-highest score is \underline{underlined}.}
  In each dataset, the algorithm with the highest AUCROC is marked in \textcolor{red}{red}, the second highest in \textcolor{blue}{blue}, and the third highest in \textcolor{darkgreen}{green}.}
  \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{c|ccccccccccccccccccc}
    \toprule
    \textbf{Dataset} & \textbf{SOD} & \textbf{HBOS} & \textbf{PCA} & \textbf{OCSVM} & \textbf{LOF} & \textbf{KNN} & \textbf{LODA} & \textbf{IForest} & \textbf{DAGMM} & \textbf{ECOD} & \textbf{COPOD} & \textbf{DBSCAN} & \textbf{CBLOF} & \textbf{DCOD} & \textbf{KMeans--} & \textbf{DeepSVDD} & \textbf{DIF} & \textbf{Scalar} & \textbf{Vector} \\
    \midrule
    annthyroid & 77.38 & 60.15 & 66.24 & 57.23 & 70.20 & 71.69 & 41.02 & 82.01 & 56.53 & 78.66 & 76.80 & 50.08 & 62.28 & 55.01 & 64.99 & 76.09 & 66.76 & 75.27 & 72.72 \\
    backdoor & 68.77 & 71.56 & 80.16 & 85.04 & 85.79 & 80.58 & 66.38 & 72.15 & 55.98 & 86.08 & 80.97 & 76.55 & 81.91 & 79.57 & 89.11 & 78.83 & 92.87 & 87.28 & 89.24 \\
    breastw & 93.97 & 98.94 & 95.13 & 80.30 & 40.61 & 97.01 & 98.49 & 98.32 & N/A   & 99.17 & 99.68 & 85.20 & 96.86 & 99.02 & 97.05 & 63.36 & 77.45 & 98.15 & 98.56 \\
    campaign & 69.16 & 78.55 & 72.78 & 65.70 & 59.04 & 72.27 & 51.67 & 71.71 & 56.03 & 76.10 & 77.69 & 50.60 & 64.34 & 63.16 & 63.51 & 54.42 & 67.53 & 73.52 & 73.64 \\
    celeba & 48.44 & 76.18 & 79.38 & 70.70 & 38.95 & 59.63 & 60.17 & 70.41 & 44.74 & 76.48 & 75.68 & 50.36 & 73.99 & 91.41 & 56.76 & 45.17 & 65.29 & 81.38 & 82.00 \\
    census & 62.12 & 64.89 & 68.74 & 54.90 & 47.46 & 66.88 & 37.14 & 59.52 & 59.65 & 67.63 & 69.07 & 58.50 & 60.17 & 72.84 & 63.33 & 54.16 & 59.66 & 67.90 & 67.84 \\
    glass & 73.36 & 77.23 & 66.29 & 35.36 & 69.20 & 82.29 & 73.13 & 77.13 & 76.09 & 65.83 & 72.43 & 54.55 & 78.30 & 78.07 & 77.30 & 55.71 & 84.57 & 79.52 & 82.17 \\
    Hepatitis & 67.83 & 79.85 & 75.95 & 67.75 & 38.06 & 52.76 & 64.87 & 69.75 & 54.80 & 75.22 & 82.05 & 68.12 & 73.05 & 48.38 & 64.64 & 57.45 & 74.24 & 75.53 & 80.62 \\
    http  & 78.04 & 99.53 & 99.72 & 99.59 & 27.46 & 3.37  & 12.48 & 99.96 & N/A   & 98.10 & 99.29 & 49.97 & 99.60 & 99.53 & 99.55 & 60.38 & 99.49 & 99.53 & 99.52 \\
    Ionosphere & 86.37 & 62.49 & 79.19 & 75.92 & 90.59 & 88.26 & 78.42 & 84.50 & 73.41 & 73.15 & 79.34 & 81.12 & 90.79 & 57.78 & 91.36 & 53.94 & 89.74 & 92.04 & 90.37 \\
    landsat & 59.54 & 55.14 & 35.76 & 36.15 & 53.90 & 57.95 & 38.17 & 47.64 & 43.92 & 36.10 & 41.55 & 50.17 & 63.69 & 33.40 & 55.31 & 62.48 & 54.84 & 49.60 & 57.37 \\
    Lymphography & 71.22 & 99.49 & 99.82 & 99.54 & 89.86 & 55.91 & 85.55 & 99.81 & 72.11 & 99.52 & 99.48 & 74.16 & 99.81 & 81.19 & 100.00 & 71.91 & 83.67 & 99.29 & 99.73 \\
    mnist & 60.10 & 60.42 & 85.29 & 82.95 & 67.13 & 80.58 & 72.27 & 80.98 & 67.23 & 74.61 & 77.74 & 50.00 & 79.96 & 65.23 & 82.45 & 50.98 & 88.16 & 86.00 & 86.64 \\
    musk  & 74.09 & 100.00 & 100.00 & 80.58 & 41.18 & 69.89 & 95.11 & 99.99 & 76.85 & 95.40 & 94.20 & 50.00 & 100.00 & 42.19 & 72.16 & 66.02 & 98.22 & 99.92 & 100.00 \\
    pendigits & 66.29 & 93.04 & 93.73 & 93.75 & 47.99 & 72.95 & 89.10 & 94.76 & 64.22 & 93.01 & 90.68 & 55.33 & 96.93 & 94.33 & 94.37 & 27.32 & 93.79 & 95.12 & 95.52 \\
    Pima  & 61.25 & 71.07 & 70.77 & 66.92 & 65.71 & 73.43 & 65.93 & 72.87 & 55.93 & 63.05 & 69.10 & 51.39 & 71.49 & 72.16 & 70.44 & 49.49 & 67.28 & 75.16 & 74.87 \\
    satellite & 63.96 & 74.80 & 59.62 & 59.02 & 55.88 & 65.18 & 61.98 & 70.43 & 62.33 & 58.09 & 63.20 & 55.52 & 71.32 & 55.97 & 67.71 & 57.40 & 74.52 & 72.46 & 77.65 \\
    satimage-2 & 83.08 & 97.65 & 97.62 & 97.35 & 47.36 & 92.60 & 97.56 & 99.16 & 96.29 & 96.28 & 97.21 & 75.74 & 99.84 & 86.01 & 99.88 & 55.68 & 99.63 & 99.87 & 99.88 \\
    shuttle & 69.51 & 98.63 & 98.62 & 97.40 & 57.11 & 69.64 & 60.95 & 99.56 & 97.92 & 99.13 & 99.35 & 50.40 & 93.07 & 97.20 & 69.97 & 51.81 & 97.00 & 99.15 & 98.75 \\
    skin  & 60.35 & 60.15 & 45.26 & 49.45 & 46.47 & 71.46 & 45.75 & 68.21 & N/A   & 49.08 & 47.55 & 50.00 & 68.03 & 64.34 & 65.47 & 45.69 & 66.36 & 72.26 & 69.69 \\
    Stamps & 73.26 & 90.73 & 91.47 & 83.86 & 51.26 & 68.61 & 87.18 & 91.21 & 88.89 & 87.87 & 93.40 & 52.08 & 69.89 & 93.41 & 79.78 & 59.48 & 87.95 & 91.37 & 94.18 \\
    thyroid & 92.81 & 95.62 & 96.34 & 87.92 & 86.86 & 95.93 & 74.30 & 98.30 & 79.75 & 97.94 & 94.30 & 53.57 & 94.74 & 78.55 & 92.26 & 52.14 & 96.26 & 97.66 & 97.48 \\
    vertebral & 40.32 & 28.56 & 37.06 & 37.99 & 49.29 & 33.79 & 30.57 & 36.66 & 53.20 & 40.66 & 25.64 & 49.74 & 41.01 & 38.13 & 38.14 & 37.81 & 47.20 & 33.11 & 47.37 \\
    vowels & 92.65 & 72.21 & 65.29 & 61.59 & 93.12 & 97.26 & 70.36 & 73.94 & 60.58 & 62.24 & 53.15 & 57.50 & 92.12 & 51.56 & 93.45 & 49.87 & 81.02 & 88.38 & 92.09 \\
    Waveform & 68.57 & 68.77 & 65.48 & 56.29 & 73.32 & 73.78 & 60.13 & 71.47 & 49.35 & 62.36 & 75.03 & 66.41 & 71.27 & 63.47 & 74.35 & 53.94 & 75.33 & 71.81 & 74.29 \\
    WBC   & 94.60 & 98.72 & 98.20 & 99.03 & 54.17 & 90.56 & 96.91 & 99.01 & N/A   & 99.11 & 99.11 & 87.43 & 96.88 & 94.92 & 97.45 & 62.46 & 81.27 & 97.68 & 98.93 \\
    Wilt  & 53.25 & 32.49 & 20.39 & 31.28 & 50.65 & 48.42 & 26.42 & 41.94 & 37.29 & 36.30 & 33.40 & 49.96 & 34.50 & 44.71 & 34.91 & 45.90 & 39.46 & 48.95 & 52.56 \\
    wine  & 46.11 & 91.36 & 84.37 & 73.07 & 37.74 & 44.98 & 90.12 & 80.37 & 61.70 & 77.22 & 88.65 & 40.33 & 27.14 & 82.18 & 27.36 & 64.26 & 41.69 & 82.72 & 95.25 \\
    WPBC  & 51.28 & 51.24 & 46.01 & 45.35 & 41.41 & 46.59 & 49.31 & 46.63 & 47.80 & 46.65 & 49.34 & 52.22 & 45.32 & 49.67 & 45.01 & 44.01 & 44.69 & 48.02 & 49.90 \\
    \midrule
    Avg. Rank & 11.00 & 8.26  & 8.98  & 11.59 & 13.59 & 10.00 & 13.24 & 7.09  & 13.24 & 9.19  & 8.29  & 14.21 & 8.07  & 10.90 & 8.71  & 15.48 & 8.38  & 5.41  & 3.59 \\
    \bottomrule
    \end{tabular}%
   \end{adjustbox} 
  \label{tab:sel30_auc}%
\end{table*}%


% % Table generated by Excel2LaTeX from sheet 'report_auc'
% \begin{table*}[t]
%   \centering
%   \caption{AUCROC of 14 unsupervised algorithms on 30 tabular benchmark datasets. 
%   % In each dataset, the highest score is highlighted in \textbf{bold}, and the second-highest score is \underline{underlined}.}
%   In each dataset, the algorithm with the highest AUCROC is marked in \textcolor{red}{red}, the second highest in \textcolor{blue}{blue}, and the third highest in \textcolor{darkgreen}{green}.}
%   \begin{adjustbox}{max width=\linewidth}
  
% % \begin{tabular}{c|cccccccccccccc|cc}
% %   \toprule
% %     \textbf{Dataset} & \textbf{CBLOF} & \textbf{COF} & \textbf{COPOD} & \makecell{\textbf{DA} \\ \textbf{GMM} } & \textbf{DCFOD} & \makecell{\textbf{Deep} \\ \textbf{SVDD} } & \textbf{ECOD} & \textbf{HBOS} & \textbf{IForest} & \textbf{KMeans-$ $-} & \textbf{KNN} & \textbf{LOF} & \textbf{PCA} & \textbf{SOD} & \makecell{\textbf{Galaxy} \\ \textbf{(Scalar)}} & \makecell{\textbf{Galaxy} \\ \textbf{(Vector)}} \\
% %     \midrule

% % % ALOI & 55.28 & \underline{64.68}  & 53.75 & 51.95 & 52.76 & 50.47 & 56.33 & 52.63 & 56.66 & 54.91 & 61.47 & \textbf{66.63} & 56.65 & 61.09 & 56.59 & 56.64 \\
% % % backdoor & 81.91 & 73.06 & 80.97 & 55.98 & 79.57 & 78.83 & 86.08 & 71.56 & 72.15 & 89.11 & 80.58 & 85.79 & 80.16 & 68.77 & \textbf{89.49} & \underline{89.24}  \\
% % % breastw & 96.86 & 38.84 & \textbf{99.68} & N/A & 99.02 & 63.36 & \underline{99.17}  & 98.94 & 98.32 & 97.05 & 97.01 & 40.61 & 95.13 & 93.97 & 98.41 & 98.56 \\
% % % campaign & 64.34 & 57.35 & \underline{77.69}  & 56.03 & 63.16 & 54.42 & 76.10 & \textbf{78.55} & 71.71 & 63.51 & 72.27 & 59.04 & 72.78 & 69.16 & 73.43 & 73.64 \\
% % % celeba & 73.99 & 38.58 & 75.68 & 44.74 & \textbf{91.41} & 45.17 & 76.48 & 76.18 & 70.41 & 56.76 & 59.63 & 38.95 & 79.38 & 48.44 & \underline{82.70}  & 82.00 \\
% % % census & 60.17 & 41.57 & \underline{69.07}  & 59.65 & \textbf{72.84} & 54.16 & 67.63 & 64.89 & 59.52 & 63.33 & 66.88 & 47.46 & 68.74 & 62.12 & 67.83 & 67.84 \\
% % % fraud & 87.26 & \textbf{96.41} & 88.32 & 89.77 & 37.50 & 68.86 & 89.04 & 90.29 & 90.38 & 87.71 & 93.36 & \underline{95.51}  & 90.35 & 94.72 & 90.21 & 90.45 \\
% % % glass & 78.30 & 72.24 & 72.43 & 76.09 & 78.07 & 55.71 & 65.83 & 77.23 & 77.13 & 77.30 & \textbf{82.29} & 69.20 & 66.29 & 73.36 & 79.32 & \underline{82.17}  \\
% % % Hepatitis & 73.05 & 41.45 & \textbf{82.05} & 54.80 & 48.38 & 57.45 & 75.22 & 79.85 & 69.75 & 64.64 & 52.76 & 38.06 & 75.95 & 67.83 & 79.88 & \underline{80.62}  \\
% % % Ionosphere & \underline{90.79}  & 86.76 & 79.34 & 73.41 & 57.78 & 53.94 & 73.15 & 62.49 & 84.50 & \textbf{91.36} & 88.26 & 90.59 & 79.19 & 86.37 & 90.07 & 90.37 \\
% % % landsat & \textbf{63.69} & 53.50 & 41.55 & 43.92 & 33.40 & \underline{62.48}  & 36.10 & 55.14 & 47.64 & 55.31 & 57.95 & 53.90 & 35.76 & 59.54 & 57.68 & 57.37 \\
% % % letter & 73.72 & 80.03 & 54.32 & 50.42 & 53.23 & 55.93 & 56.04 & 59.74 & 61.07 & 75.96 & \textbf{86.19} & \underline{84.49}  & 50.29 & 84.09 & 73.23 & 73.85 \\
% % % Lymphography & 99.81 & 90.85 & 99.48 & 72.11 & 81.19 & 71.91 & 99.52 & 99.49 & 99.81 & \textbf{100.00} & 55.91 & 89.86 & \underline{99.82}  & 71.22 & 99.50 & 99.73 \\
% % % mnist & 79.96 & 70.78 & 77.74 & 67.23 & 65.23 & 50.98 & 74.61 & 60.42 & 80.98 & 82.45 & 80.58 & 67.13 & 85.29 & 60.10 & \underline{86.56}  & \textbf{86.64} \\
% % % musk & 100.00 & 38.69 & 94.20 & 76.85 & 42.19 & 66.02 & 95.40 & 100.00 & 99.99 & 72.16 & 69.89 & 41.18 & 100.00 & 74.09 & \underline{100.00}  & \textbf{100.00} \\
% % % pendigits & \textbf{96.93} & 45.07 & 90.68 & 64.22 & 94.33 & 27.32 & 93.01 & 93.04 & 94.76 & 94.37 & 72.95 & 47.99 & 93.73 & 66.29 & 95.32 & \underline{95.52}  \\
% % % Pima & 71.49 & 61.05 & 69.10 & 55.93 & 72.16 & 49.49 & 63.05 & 71.07 & 72.87 & 70.44 & 73.43 & 65.71 & 70.77 & 61.25 & \underline{74.59}  & \textbf{74.87} \\
% % % satellite & 71.32 & 54.74 & 63.20 & 62.33 & 55.97 & 57.40 & 58.09 & 74.80 & 70.43 & 67.71 & 65.18 & 55.88 & 59.62 & 63.96 & \textbf{77.80} & \underline{77.65}  \\
% % % satimage-2 & 99.84 & 56.70 & 97.21 & 96.29 & 86.01 & 55.68 & 96.28 & 97.65 & 99.16 & \underline{99.88}  & 92.60 & 47.36 & 97.62 & 83.08 & 99.87 & \textbf{99.88} \\
% % % shuttle & 93.07 & 51.72 & \underline{99.35}  & 97.92 & 97.20 & 51.81 & 99.13 & 98.63 & \textbf{99.56} & 69.97 & 69.64 & 57.11 & 98.62 & 69.51 & 98.52 & 98.75 \\
% % % skin & 68.03 & 41.66 & 47.55 & N/A & 64.34 & 45.69 & 49.08 & 60.15 & 68.21 & 65.47 & \textbf{71.46} & 46.47 & 45.26 & 60.35 & \underline{70.98}  & 69.69 \\
% % % SpamBase & 55.22 & 40.96 & \textbf{70.09} & N/A & 50.26 & 50.31 & \underline{66.89}  & 64.74 & 64.76 & 56.31 & 53.35 & 43.33 & 54.66 & 52.35 & 54.31 & 54.38 \\
% % % Stamps & 69.89 & 53.81 & 93.40 & 88.89 & \underline{93.41}  & 59.48 & 87.87 & 90.73 & 91.21 & 79.78 & 68.61 & 51.26 & 91.47 & 73.26 & 90.83 & \textbf{94.18} \\
% % % vertebral & 41.01 & 48.71 & 25.64 & \textbf{53.20} & 38.13 & 37.81 & 40.66 & 28.56 & 36.66 & 38.14 & 33.79 & \underline{49.29}  & 37.06 & 40.32 & 40.66 & 47.37 \\
% % % vowels & 92.12 & \underline{94.04}  & 53.15 & 60.58 & 51.56 & 49.87 & 62.24 & 72.21 & 73.94 & 93.45 & \textbf{97.26} & 93.12 & 65.29 & 92.65 & 90.79 & 92.09 \\
% % % Waveform & 71.27 & 72.56 & \textbf{75.03} & 49.35 & 63.47 & 53.94 & 62.36 & 68.77 & 71.47 & \underline{74.35}  & 73.78 & 73.32 & 65.48 & 68.57 & 73.54 & 74.29 \\
% % % WBC & 96.88 & 60.90 & \underline{99.11}  & N/A & 94.92 & 62.46 & \textbf{99.11} & 98.72 & 99.01 & 97.45 & 90.56 & 54.17 & 98.20 & 94.60 & 98.91 & 98.93 \\
% % % Wilt & 34.50 & 49.66 & 33.40 & 37.29 & 44.71 & 45.90 & 36.30 & 32.49 & 41.94 & 34.91 & 48.42 & 50.65 & 20.39 & \textbf{53.25} & 50.00 & \underline{52.56}  \\
% % % wine & 27.14 & 44.44 & 88.65 & 61.70 & 82.18 & 64.26 & 77.22 & 91.36 & 80.37 & 27.36 & 44.98 & 37.74 & 84.37 & 46.11 & \underline{93.24}  & \textbf{95.25} \\
% % % WPBC & 45.32 & 45.88 & 49.34 & 47.80 & 49.67 & 44.01 & 46.65 & \underline{51.24}  & 46.63 & 45.01 & 46.59 & 41.41 & 46.01 & \textbf{51.28} & 50.29 & 49.90 \\

    
% % % ALOI & 55.28 & \textcolor{blue}{ \underline{64.68} } & 53.75 & 51.95 & 52.76 & 50.47 & 56.33 & 52.63 & 56.66 & 54.91 & 61.47 & \textcolor{red}{ \textbf{66.63} } & 56.65 & 61.09 & 56.59 & 56.64 \\
% % % backdoor & 81.91 & 73.06 & 80.97 & 55.98 & 79.57 & 78.83 & 86.08 & 71.56 & 72.15 & 89.11 & 80.58 & 85.79 & 80.16 & 68.77 & \textcolor{red}{ \textbf{89.49} } & \textcolor{blue}{ \underline{89.24} } \\
% % % breastw & 96.86 & 38.84 & \textcolor{red}{ \textbf{99.68} } & N/A & 99.02 & 63.36 & \textcolor{blue}{ \underline{99.17} } & 98.94 & 98.32 & 97.05 & 97.01 & 40.61 & 95.13 & 93.97 & 98.41 & 98.56 \\
% % % campaign & 64.34 & 57.35 & \textcolor{blue}{ \underline{77.69} } & 56.03 & 63.16 & 54.42 & 76.10 & \textcolor{red}{ \textbf{78.55} } & 71.71 & 63.51 & 72.27 & 59.04 & 72.78 & 69.16 & 73.43 & 73.64 \\
% % % celeba & 73.99 & 38.58 & 75.68 & 44.74 & \textcolor{red}{ \textbf{91.41} } & 45.17 & 76.48 & 76.18 & 70.41 & 56.76 & 59.63 & 38.95 & 79.38 & 48.44 & \textcolor{blue}{ \underline{82.70} } & 82.00 \\
% % % census & 60.17 & 41.57 & \textcolor{blue}{ \underline{69.07} } & 59.65 & \textcolor{red}{ \textbf{72.84} } & 54.16 & 67.63 & 64.89 & 59.52 & 63.33 & 66.88 & 47.46 & 68.74 & 62.12 & 67.83 & 67.84 \\
% % % fraud & 87.26 & \textcolor{red}{ \textbf{96.41} } & 88.32 & 89.77 & 37.50 & 68.86 & 89.04 & 90.29 & 90.38 & 87.71 & 93.36 & \textcolor{blue}{ \underline{95.51} } & 90.35 & 94.72 & 90.21 & 90.45 \\
% % % glass & 78.30 & 72.24 & 72.43 & 76.09 & 78.07 & 55.71 & 65.83 & 77.23 & 77.13 & 77.30 & \textcolor{red}{ \textbf{82.29} } & 69.20 & 66.29 & 73.36 & 79.32 & \textcolor{blue}{ \underline{82.17} } \\
% % % Hepatitis & 73.05 & 41.45 & \textcolor{red}{ \textbf{82.05} } & 54.80 & 48.38 & 57.45 & 75.22 & 79.85 & 69.75 & 64.64 & 52.76 & 38.06 & 75.95 & 67.83 & 79.88 & \textcolor{blue}{ \underline{80.62} } \\
% % % Ionosphere & \textcolor{blue}{ \underline{90.79} } & 86.76 & 79.34 & 73.41 & 57.78 & 53.94 & 73.15 & 62.49 & 84.50 & \textcolor{red}{ \textbf{91.36} } & 88.26 & 90.59 & 79.19 & 86.37 & 90.07 & 90.37 \\
% % % landsat & \textcolor{red}{ \textbf{63.69} } & 53.50 & 41.55 & 43.92 & 33.40 & \textcolor{blue}{ \underline{62.48} } & 36.10 & 55.14 & 47.64 & 55.31 & 57.95 & 53.90 & 35.76 & 59.54 & 57.68 & 57.37 \\
% % % letter & 73.72 & 80.03 & 54.32 & 50.42 & 53.23 & 55.93 & 56.04 & 59.74 & 61.07 & 75.96 & \textcolor{red}{ \textbf{86.19} } & \textcolor{blue}{ \underline{84.49} } & 50.29 & 84.09 & 73.23 & 73.85 \\
% % % Lymphography & 99.81 & 90.85 & 99.48 & 72.11 & 81.19 & 71.91 & 99.52 & 99.49 & 99.81 & \textcolor{red}{ \textbf{100.00} } & 55.91 & 89.86 & \textcolor{blue}{ \underline{99.82} } & 71.22 & 99.50 & 99.73 \\
% % % mnist & 79.96 & 70.78 & 77.74 & 67.23 & 65.23 & 50.98 & 74.61 & 60.42 & 80.98 & 82.45 & 80.58 & 67.13 & 85.29 & 60.10 & \textcolor{blue}{ \underline{86.56} } & \textcolor{red}{ \textbf{86.64} } \\
% % % musk & 100.00 & 38.69 & 94.20 & 76.85 & 42.19 & 66.02 & 95.40 & 100.00 & 99.99 & 72.16 & 69.89 & 41.18 & 100.00 & 74.09 & \textcolor{blue}{ \underline{100.00} } & \textcolor{red}{ \textbf{100.00} } \\
% % % pendigits & \textcolor{red}{ \textbf{96.93} } & 45.07 & 90.68 & 64.22 & 94.33 & 27.32 & 93.01 & 93.04 & 94.76 & 94.37 & 72.95 & 47.99 & 93.73 & 66.29 & 95.32 & \textcolor{blue}{ \underline{95.52} } \\
% % % Pima & 71.49 & 61.05 & 69.10 & 55.93 & 72.16 & 49.49 & 63.05 & 71.07 & 72.87 & 70.44 & 73.43 & 65.71 & 70.77 & 61.25 & \textcolor{blue}{ \underline{74.59} } & \textcolor{red}{ \textbf{74.87} } \\
% % % satellite & 71.32 & 54.74 & 63.20 & 62.33 & 55.97 & 57.40 & 58.09 & 74.80 & 70.43 & 67.71 & 65.18 & 55.88 & 59.62 & 63.96 & \textcolor{red}{ \textbf{77.80} } & \textcolor{blue}{ \underline{77.65} } \\
% % % satimage-2 & 99.84 & 56.70 & 97.21 & 96.29 & 86.01 & 55.68 & 96.28 & 97.65 & 99.16 & \textcolor{blue}{ \underline{99.88} } & 92.60 & 47.36 & 97.62 & 83.08 & 99.87 & \textcolor{red}{ \textbf{99.88} } \\
% % % shuttle & 93.07 & 51.72 & \textcolor{blue}{ \underline{99.35} } & 97.92 & 97.20 & 51.81 & 99.13 & 98.63 & \textcolor{red}{ \textbf{99.56} } & 69.97 & 69.64 & 57.11 & 98.62 & 69.51 & 98.52 & 98.75 \\
% % % skin & 68.03 & 41.66 & 47.55 & N/A & 64.34 & 45.69 & 49.08 & 60.15 & 68.21 & 65.47 & \textcolor{red}{ \textbf{71.46} } & 46.47 & 45.26 & 60.35 & \textcolor{blue}{ \underline{70.98} } & 69.69 \\
% % % SpamBase & 55.22 & 40.96 & \textcolor{red}{ \textbf{70.09} } & N/A & 50.26 & 50.31 & \textcolor{blue}{ \underline{66.89} } & 64.74 & 64.76 & 56.31 & 53.35 & 43.33 & 54.66 & 52.35 & 54.31 & 54.38 \\
% % % Stamps & 69.89 & 53.81 & 93.40 & 88.89 & \textcolor{blue}{ \underline{93.41} } & 59.48 & 87.87 & 90.73 & 91.21 & 79.78 & 68.61 & 51.26 & 91.47 & 73.26 & 90.83 & \textcolor{red}{ \textbf{94.18} } \\
% % % vertebral & 41.01 & 48.71 & 25.64 & \textcolor{red}{ \textbf{53.20} } & 38.13 & 37.81 & 40.66 & 28.56 & 36.66 & 38.14 & 33.79 & \textcolor{blue}{ \underline{49.29} } & 37.06 & 40.32 & 40.66 & 47.37 \\
% % % vowels & 92.12 & \textcolor{blue}{ \underline{94.04} } & 53.15 & 60.58 & 51.56 & 49.87 & 62.24 & 72.21 & 73.94 & 93.45 & \textcolor{red}{ \textbf{97.26} } & 93.12 & 65.29 & 92.65 & 90.79 & 92.09 \\
% % % Waveform & 71.27 & 72.56 & \textcolor{red}{ \textbf{75.03} } & 49.35 & 63.47 & 53.94 & 62.36 & 68.77 & 71.47 & \textcolor{blue}{ \underline{74.35} } & 73.78 & 73.32 & 65.48 & 68.57 & 73.54 & 74.29 \\
% % % WBC & 96.88 & 60.90 & \textcolor{blue}{ \underline{99.11} } & N/A & 94.92 & 62.46 & \textcolor{red}{ \textbf{99.11} } & 98.72 & 99.01 & 97.45 & 90.56 & 54.17 & 98.20 & 94.60 & 98.91 & 98.93 \\
% % % Wilt & 34.50 & 49.66 & 33.40 & 37.29 & 44.71 & 45.90 & 36.30 & 32.49 & 41.94 & 34.91 & 48.42 & 50.65 & 20.39 & \textcolor{red}{ \textbf{53.25} } & 50.00 & \textcolor{blue}{ \underline{52.56} } \\
% % % wine & 27.14 & 44.44 & 88.65 & 61.70 & 82.18 & 64.26 & 77.22 & 91.36 & 80.37 & 27.36 & 44.98 & 37.74 & 84.37 & 46.11 & \textcolor{blue}{ \underline{93.24} } & \textcolor{red}{ \textbf{95.25} } \\
% % % WPBC & 45.32 & 45.88 & 49.34 & 47.80 & 49.67 & 44.01 & 46.65 & \textcolor{blue}{ \underline{51.24} } & 46.63 & 45.01 & 46.59 & 41.41 & 46.01 & \textcolor{red}{ \textbf{51.28} } & 50.29 & 49.90 \\


% % ALOI & 55.28 & \textcolor{blue}{ {64.68} } & 53.75 & 51.95 & 52.76 & 50.47 & 56.33 & 52.63 & 56.66 & 54.91 & \textcolor{darkgreen}{ 61.47 } & \textcolor{red}{ \textbf{66.63} } & 56.65 & 61.09 & 56.59 & 56.64 \\
% % backdoor & 81.91 & 73.06 & 80.97 & 55.98 & 79.57 & 78.83 & 86.08 & 71.56 & 72.15 & \textcolor{darkgreen}{ 89.11 } & 80.58 & 85.79 & 80.16 & 68.77 & \textcolor{red}{ \textbf{89.49} } & \textcolor{blue}{ {89.24} } \\
% % breastw & 96.86 & 38.84 & \textcolor{red}{ \textbf{99.68} } & N/A & \textcolor{darkgreen}{ 99.02 } & 63.36 & \textcolor{blue}{ {99.17} } & 98.94 & 98.32 & 97.05 & 97.01 & 40.61 & 95.13 & 93.97 & 98.41 & 98.56 \\
% % campaign & 64.34 & 57.35 & \textcolor{blue}{ {77.69} } & 56.03 & 63.16 & 54.42 & \textcolor{darkgreen}{ 76.10 } & \textcolor{red}{ \textbf{78.55} } & 71.71 & 63.51 & 72.27 & 59.04 & 72.78 & 69.16 & 73.43 & 73.64 \\
% % celeba & 73.99 & 38.58 & 75.68 & 44.74 & \textcolor{red}{ \textbf{91.41} } & 45.17 & 76.48 & 76.18 & 70.41 & 56.76 & 59.63 & 38.95 & 79.38 & 48.44 & \textcolor{blue}{ {82.70} } & \textcolor{darkgreen}{ 82.00 } \\
% % census & 60.17 & 41.57 & \textcolor{blue}{ {69.07} } & 59.65 & \textcolor{red}{ \textbf{72.84} } & 54.16 & 67.63 & 64.89 & 59.52 & 63.33 & 66.88 & 47.46 & \textcolor{darkgreen}{ 68.74 } & 62.12 & 67.83 & 67.84 \\
% % fraud & 87.26 & \textcolor{red}{ \textbf{96.41} } & 88.32 & 89.77 & 37.50 & 68.86 & 89.04 & 90.29 & 90.38 & 87.71 & 93.36 & \textcolor{blue}{ {95.51} } & 90.35 & \textcolor{darkgreen}{ 94.72 } & 90.21 & 90.45 \\
% % glass & 78.30 & 72.24 & 72.43 & 76.09 & 78.07 & 55.71 & 65.83 & 77.23 & 77.13 & 77.30 & \textcolor{red}{ \textbf{82.29} } & 69.20 & 66.29 & 73.36 & \textcolor{darkgreen}{ 79.32 } & \textcolor{blue}{ {82.17} } \\
% % Hepatitis & 73.05 & 41.45 & \textcolor{red}{ \textbf{82.05} } & 54.80 & 48.38 & 57.45 & 75.22 & 79.85 & 69.75 & 64.64 & 52.76 & 38.06 & 75.95 & 67.83 & \textcolor{darkgreen}{ 79.88 } & \textcolor{blue}{ {80.62} } \\
% % Ionosphere & \textcolor{blue}{ {90.79} } & 86.76 & 79.34 & 73.41 & 57.78 & 53.94 & 73.15 & 62.49 & 84.50 & \textcolor{red}{ \textbf{91.36} } & 88.26 & \textcolor{darkgreen}{ 90.59 } & 79.19 & 86.37 & 90.07 & 90.37 \\
% % landsat & \textcolor{red}{ \textbf{63.69} } & 53.50 & 41.55 & 43.92 & 33.40 & \textcolor{blue}{ {62.48} } & 36.10 & 55.14 & 47.64 & 55.31 & 57.95 & 53.90 & 35.76 & \textcolor{darkgreen}{ 59.54 } & 57.68 & 57.37 \\
% % letter & 73.72 & 80.03 & 54.32 & 50.42 & 53.23 & 55.93 & 56.04 & 59.74 & 61.07 & 75.96 & \textcolor{red}{ \textbf{86.19} } & \textcolor{blue}{ {84.49} } & 50.29 & \textcolor{darkgreen}{ 84.09 } & 73.23 & 73.85 \\
% % Lymphography & 99.81 & 90.85 & 99.48 & 72.11 & 81.19 & 71.91 & 99.52 & 99.49 & \textcolor{darkgreen}{ 99.81 } & \textcolor{red}{ \textbf{100.00} } & 55.91 & 89.86 & \textcolor{blue}{ {99.82} } & 71.22 & 99.50 & 99.73 \\
% % mnist & 79.96 & 70.78 & 77.74 & 67.23 & 65.23 & 50.98 & 74.61 & 60.42 & 80.98 & 82.45 & 80.58 & 67.13 & \textcolor{darkgreen}{ 85.29 } & 60.10 & \textcolor{blue}{ {86.56} } & \textcolor{red}{ \textbf{86.64} } \\
% % musk & 100.00 & 38.69 & 94.20 & 76.85 & 42.19 & 66.02 & 95.40 & 100.00 & 99.99 & 72.16 & 69.89 & 41.18 & \textcolor{darkgreen}{ 100.00 } & 74.09 & \textcolor{blue}{ {100.00} } & \textcolor{red}{ \textbf{100.00} } \\
% % pendigits & \textcolor{red}{ \textbf{96.93} } & 45.07 & 90.68 & 64.22 & 94.33 & 27.32 & 93.01 & 93.04 & 94.76 & 94.37 & 72.95 & 47.99 & 93.73 & 66.29 & \textcolor{darkgreen}{ 95.32 } & \textcolor{blue}{ {95.52} } \\
% % Pima & 71.49 & 61.05 & 69.10 & 55.93 & 72.16 & 49.49 & 63.05 & 71.07 & 72.87 & 70.44 & \textcolor{darkgreen}{ 73.43 } & 65.71 & 70.77 & 61.25 & \textcolor{blue}{ {74.59} } & \textcolor{red}{ \textbf{74.87} } \\
% % satellite & 71.32 & 54.74 & 63.20 & 62.33 & 55.97 & 57.40 & 58.09 & \textcolor{darkgreen}{ 74.80 } & 70.43 & 67.71 & 65.18 & 55.88 & 59.62 & 63.96 & \textcolor{red}{ \textbf{77.80} } & \textcolor{blue}{ {77.65} } \\
% % satimage-2 & 99.84 & 56.70 & 97.21 & 96.29 & 86.01 & 55.68 & 96.28 & 97.65 & 99.16 & \textcolor{blue}{ {99.88} } & 92.60 & 47.36 & 97.62 & 83.08 & \textcolor{darkgreen}{ 99.87 } & \textcolor{red}{ \textbf{99.88} } \\
% % shuttle & 93.07 & 51.72 & \textcolor{blue}{ {99.35} } & 97.92 & 97.20 & 51.81 & \textcolor{darkgreen}{ 99.13 } & 98.63 & \textcolor{red}{ \textbf{99.56} } & 69.97 & 69.64 & 57.11 & 98.62 & 69.51 & 98.52 & 98.75 \\
% % skin & 68.03 & 41.66 & 47.55 & N/A & 64.34 & 45.69 & 49.08 & 60.15 & 68.21 & 65.47 & \textcolor{red}{ \textbf{71.46} } & 46.47 & 45.26 & 60.35 & \textcolor{blue}{ {70.98} } & \textcolor{darkgreen}{ 69.69 } \\
% % SpamBase & 55.22 & 40.96 & \textcolor{red}{ \textbf{70.09} } & N/A & 50.26 & 50.31 & \textcolor{blue}{ {66.89} } & 64.74 & \textcolor{darkgreen}{ 64.76 } & 56.31 & 53.35 & 43.33 & 54.66 & 52.35 & 54.31 & 54.38 \\
% % Stamps & 69.89 & 53.81 & \textcolor{darkgreen}{ 93.40 } & 88.89 & \textcolor{blue}{ {93.41} } & 59.48 & 87.87 & 90.73 & 91.21 & 79.78 & 68.61 & 51.26 & 91.47 & 73.26 & 90.83 & \textcolor{red}{ \textbf{94.18} } \\
% % vertebral & 41.01 & \textcolor{darkgreen}{ 48.71 } & 25.64 & \textcolor{red}{ \textbf{53.20} } & 38.13 & 37.81 & 40.66 & 28.56 & 36.66 & 38.14 & 33.79 & \textcolor{blue}{ {49.29} } & 37.06 & 40.32 & 40.66 & 47.37 \\
% % vowels & 92.12 & \textcolor{blue}{ {94.04} } & 53.15 & 60.58 & 51.56 & 49.87 & 62.24 & 72.21 & 73.94 & \textcolor{darkgreen}{ 93.45 } & \textcolor{red}{ \textbf{97.26} } & 93.12 & 65.29 & 92.65 & 90.79 & 92.09 \\
% % Waveform & 71.27 & 72.56 & \textcolor{red}{ \textbf{75.03} } & 49.35 & 63.47 & 53.94 & 62.36 & 68.77 & 71.47 & \textcolor{blue}{ {74.35} } & 73.78 & 73.32 & 65.48 & 68.57 & 73.54 & \textcolor{darkgreen}{ 74.29 } \\
% % WBC & 96.88 & 60.90 & \textcolor{blue}{ {99.11} } & N/A & 94.92 & 62.46 & \textcolor{red}{ \textbf{99.11} } & 98.72 & \textcolor{darkgreen}{ 99.01 } & 97.45 & 90.56 & 54.17 & 98.20 & 94.60 & 98.91 & 98.93 \\
% % Wilt & 34.50 & 49.66 & 33.40 & 37.29 & 44.71 & 45.90 & 36.30 & 32.49 & 41.94 & 34.91 & 48.42 & \textcolor{darkgreen}{ 50.65 } & 20.39 & \textcolor{red}{ \textbf{53.25} } & 50.00 & \textcolor{blue}{ {52.56} } \\
% % wine & 27.14 & 44.44 & 88.65 & 61.70 & 82.18 & 64.26 & 77.22 & \textcolor{darkgreen}{ 91.36 } & 80.37 & 27.36 & 44.98 & 37.74 & 84.37 & 46.11 & \textcolor{blue}{ {93.24} } & \textcolor{red}{ \textbf{95.25} } \\
% % WPBC & 45.32 & 45.88 & 49.34 & 47.80 & 49.67 & 44.01 & 46.65 & \textcolor{blue}{ {51.24} } & 46.63 & 45.01 & 46.59 & 41.41 & 46.01 & \textcolor{red}{ \textbf{51.28} } & \textcolor{darkgreen}{ 50.29 } & 49.90 \\




% % % ALOI & 0.553 & \textcolor{blue}{ \underline{0.647} } & 0.537 & 0.520 & 0.528 & 0.505 & 0.563 & 0.526 & 0.567 & 0.549 & 0.615 & \textcolor{red}{ \textbf{0.666} } & 0.566 & 0.611 & 0.566 & 0.566 \\
% % % backdoor & 0.819 & 0.731 & 0.810 & 0.560 & 0.796 & 0.788 & 0.861 & 0.716 & 0.722 & 0.891 & 0.806 & 0.858 & 0.802 & 0.688 & \textcolor{red}{ \textbf{0.895} } & \textcolor{blue}{ \underline{0.892} } \\
% % % breastw & 0.969 & 0.388 & \textcolor{red}{ \textbf{0.997} } & N/A & 0.990 & 0.634 & \textcolor{blue}{ \underline{0.992} } & 0.989 & 0.983 & 0.970 & 0.970 & 0.406 & 0.951 & 0.940 & 0.984 & 0.986 \\
% % % campaign & 0.643 & 0.574 & \textcolor{blue}{ \underline{0.777} } & 0.560 & 0.632 & 0.544 & 0.761 & \textcolor{red}{ \textbf{0.785} } & 0.717 & 0.635 & 0.723 & 0.590 & 0.728 & 0.692 & 0.734 & 0.736 \\
% % % celeba & 0.740 & 0.386 & 0.757 & 0.447 & \textcolor{red}{ \textbf{0.914} } & 0.452 & 0.765 & 0.762 & 0.704 & 0.568 & 0.596 & 0.390 & 0.794 & 0.484 & \textcolor{blue}{ \underline{0.827} } & 0.820 \\
% % % census & 0.602 & 0.416 & \textcolor{blue}{ \underline{0.691} } & 0.597 & \textcolor{red}{ \textbf{0.728} } & 0.542 & 0.676 & 0.649 & 0.595 & 0.633 & 0.669 & 0.475 & 0.687 & 0.621 & 0.678 & 0.678 \\
% % % fraud & 0.873 & \textcolor{red}{ \textbf{0.964} } & 0.883 & 0.898 & 0.375 & 0.689 & 0.890 & 0.903 & 0.904 & 0.877 & 0.934 & \textcolor{blue}{ \underline{0.955} } & 0.904 & 0.947 & 0.902 & 0.905 \\
% % % glass & 0.783 & 0.722 & 0.724 & 0.761 & 0.781 & 0.557 & 0.658 & 0.772 & 0.771 & 0.773 & \textcolor{red}{ \textbf{0.823} } & 0.692 & 0.663 & 0.734 & 0.793 & \textcolor{blue}{ \underline{0.822} } \\
% % % Hepatitis & 0.731 & 0.415 & \textcolor{red}{ \textbf{0.821} } & 0.548 & 0.484 & 0.574 & 0.752 & 0.799 & 0.698 & 0.646 & 0.528 & 0.381 & 0.759 & 0.678 & 0.799 & \textcolor{blue}{ \underline{0.806} } \\
% % % Ionosphere & \textcolor{blue}{ \underline{0.908} } & 0.868 & 0.793 & 0.734 & 0.578 & 0.539 & 0.732 & 0.625 & 0.845 & \textcolor{red}{ \textbf{0.914} } & 0.883 & 0.906 & 0.792 & 0.864 & 0.901 & 0.904 \\
% % % landsat & \textcolor{red}{ \textbf{0.637} } & 0.535 & 0.415 & 0.439 & 0.334 & \textcolor{blue}{ \underline{0.625} } & 0.361 & 0.551 & 0.476 & 0.553 & 0.580 & 0.539 & 0.358 & 0.595 & 0.577 & 0.574 \\
% % % letter & 0.737 & 0.800 & 0.543 & 0.504 & 0.532 & 0.559 & 0.560 & 0.597 & 0.611 & 0.760 & \textcolor{red}{ \textbf{0.862} } & \textcolor{blue}{ \underline{0.845} } & 0.503 & 0.841 & 0.732 & 0.738 \\
% % % Lymphography & 0.998 & 0.908 & 0.995 & 0.721 & 0.812 & 0.719 & 0.995 & 0.995 & 0.998 & \textcolor{red}{ \textbf{1.000} } & 0.559 & 0.899 & \textcolor{blue}{ \underline{0.998} } & 0.712 & 0.995 & 0.997 \\
% % % mnist & 0.800 & 0.708 & 0.777 & 0.672 & 0.652 & 0.510 & 0.746 & 0.604 & 0.810 & 0.825 & 0.806 & 0.671 & 0.853 & 0.601 & \textcolor{blue}{ \underline{0.866} } & \textcolor{red}{ \textbf{0.866} } \\
% % % musk & 1.000 & 0.387 & 0.942 & 0.769 & 0.422 & 0.660 & 0.954 & 1.000 & 1.000 & 0.722 & 0.699 & 0.412 & 1.000 & 0.741 & \textcolor{blue}{ \underline{1.000} } & \textcolor{red}{ \textbf{1.000} } \\
% % % pendigits & \textcolor{red}{ \textbf{0.969} } & 0.451 & 0.907 & 0.642 & 0.943 & 0.273 & 0.930 & 0.930 & 0.948 & 0.944 & 0.729 & 0.480 & 0.937 & 0.663 & 0.953 & \textcolor{blue}{ \underline{0.955} } \\
% % % Pima & 0.715 & 0.610 & 0.691 & 0.559 & 0.722 & 0.495 & 0.631 & 0.711 & 0.729 & 0.704 & 0.734 & 0.657 & 0.708 & 0.613 & \textcolor{blue}{ \underline{0.746} } & \textcolor{red}{ \textbf{0.749} } \\
% % % satellite & 0.713 & 0.547 & 0.632 & 0.623 & 0.560 & 0.574 & 0.581 & 0.748 & 0.704 & 0.677 & 0.652 & 0.559 & 0.596 & 0.640 & \textcolor{red}{ \textbf{0.778} } & \textcolor{blue}{ \underline{0.777} } \\
% % % satimage-2 & 0.998 & 0.567 & 0.972 & 0.963 & 0.860 & 0.557 & 0.963 & 0.976 & 0.992 & 0.999 & 0.926 & 0.474 & 0.976 & 0.831 & \textcolor{blue}{ \underline{0.999} } & \textcolor{red}{ \textbf{0.999} } \\
% % % shuttle & 0.931 & 0.517 & \textcolor{blue}{ \underline{0.994} } & 0.979 & 0.972 & 0.518 & 0.991 & 0.986 & \textcolor{red}{ \textbf{0.996} } & 0.700 & 0.696 & 0.571 & 0.986 & 0.695 & 0.985 & 0.987 \\
% % % skin & 0.680 & 0.417 & 0.476 & N/A & 0.643 & 0.457 & 0.491 & 0.602 & 0.682 & 0.655 & \textcolor{red}{ \textbf{0.715} } & 0.465 & 0.453 & 0.603 & \textcolor{blue}{ \underline{0.710} } & 0.697 \\
% % % SpamBase & 0.552 & 0.410 & \textcolor{red}{ \textbf{0.701} } & N/A & 0.503 & 0.503 & \textcolor{blue}{ \underline{0.669} } & 0.647 & 0.648 & 0.563 & 0.534 & 0.433 & 0.547 & 0.523 & 0.543 & 0.544 \\
% % % Stamps & 0.699 & 0.538 & 0.934 & 0.889 & \textcolor{blue}{ \underline{0.934} } & 0.595 & 0.879 & 0.907 & 0.912 & 0.798 & 0.686 & 0.513 & 0.915 & 0.733 & 0.908 & \textcolor{red}{ \textbf{0.942} } \\
% % % vertebral & 0.410 & 0.487 & 0.256 & \textcolor{red}{ \textbf{0.532} } & 0.381 & 0.378 & 0.407 & 0.286 & 0.367 & 0.381 & 0.338 & \textcolor{blue}{ \underline{0.493} } & 0.371 & 0.403 & 0.407 & 0.474 \\
% % % vowels & 0.921 & \textcolor{blue}{ \underline{0.940} } & 0.532 & 0.606 & 0.516 & 0.499 & 0.622 & 0.722 & 0.739 & 0.935 & \textcolor{red}{ \textbf{0.973} } & 0.931 & 0.653 & 0.927 & 0.908 & 0.921 \\
% % % Waveform & 0.713 & 0.726 & \textcolor{red}{ \textbf{0.750} } & 0.493 & 0.635 & 0.539 & 0.624 & 0.688 & 0.715 & \textcolor{blue}{ \underline{0.744} } & 0.738 & 0.733 & 0.655 & 0.686 & 0.735 & 0.743 \\
% % % WBC & 0.969 & 0.609 & \textcolor{blue}{ \underline{0.991} } & N/A & 0.949 & 0.625 & \textcolor{red}{ \textbf{0.991} } & 0.987 & 0.990 & 0.974 & 0.906 & 0.542 & 0.982 & 0.946 & 0.989 & 0.989 \\
% % % Wilt & 0.345 & 0.497 & 0.334 & 0.373 & 0.447 & 0.459 & 0.363 & 0.325 & 0.419 & 0.349 & 0.484 & 0.507 & 0.204 & \textcolor{red}{ \textbf{0.533} } & 0.500 & \textcolor{blue}{ \underline{0.526} } \\
% % % wine & 0.271 & 0.444 & 0.887 & 0.617 & 0.822 & 0.643 & 0.772 & 0.914 & 0.804 & 0.274 & 0.450 & 0.377 & 0.844 & 0.461 & \textcolor{blue}{ \underline{0.932} } & \textcolor{red}{ \textbf{0.952} } \\
% % % WPBC & 0.453 & 0.459 & 0.493 & 0.478 & 0.497 & 0.440 & 0.466 & \textcolor{blue}{ \underline{0.512} } & 0.466 & 0.450 & 0.466 & 0.414 & 0.460 & \textcolor{red}{ \textbf{0.513} } & 0.503 & 0.499 \\
% % \midrule
% % Avg. Rank & 7.4 & 11.2 & 7.6 & 11.3 & 9.8 & 13.3 & 8.3 & 7.7 & \textcolor{darkgreen}{7.0} & 7.6 & 7.8 & 10.6 & 8.5 & 9.2 & \textcolor{blue}{{4.6}} & \textcolor{red}{\textbf{3.6}} \\
% % \bottomrule
% %     \end{tabular}%


%     \begin{tabular}{c|cccccccccccccc|cc}
%     \toprule
%     \textbf{Dataset} & \textbf{SOD} & \textbf{COF} & \textbf{HBOS} & \textbf{PCA} & \textbf{LOF} & \textbf{KNN} & \textbf{IForest} & \textbf{DAGMM} & \textbf{ECOD} & \textbf{COPOD} & \textbf{CBLOF} & \textbf{DCFOD} & \boldmath{}\textbf{KMeans-$ $-}\unboldmath{} & \makecell{\textbf{Deep} \\ \textbf{SVDD} } & \makecell{\textbf{\model} \\ \textbf{(Scalar)}} & \makecell{\textbf{\model} \\ \textbf{(Vector)}} \\
%     \midrule
%     % ALOI  & 0.611  & 0.647  & 0.526  & 0.567  & 0.666  & 0.615  & 0.567  & 0.520  & 0.563  & 0.538  & 0.553  & 0.528  & 0.549  & 0.505  & 0.566  & 0.566  \\
%     % backdoor & 0.688  & 0.731  & 0.716  & 0.802  & 0.858  & 0.806  & 0.722  & 0.560  & 0.861  & 0.810  & 0.819  & 0.796  & 0.891  & 0.788  & 0.895  & 0.892  \\
%     % breastw & 0.940  & 0.388  & 0.989  & 0.951  & 0.406  & 0.970  & 0.983  & N/A   & 0.992  & 0.997  & 0.969  & 0.990  & 0.971  & 0.634  & 0.984  & 0.986  \\
%     % campaign & 0.692  & 0.574  & 0.786  & 0.728  & 0.590  & 0.723  & 0.717  & 0.560  & 0.761  & 0.777  & 0.643  & 0.632  & 0.635  & 0.544  & 0.734  & 0.736  \\
%     % celeba & 0.484  & 0.386  & 0.762  & 0.794  & 0.390  & 0.596  & 0.704  & 0.447  & 0.765  & 0.757  & 0.740  & 0.914  & 0.568  & 0.452  & 0.827  & 0.820  \\
%     % census & 0.621  & 0.416  & 0.649  & 0.687  & 0.475  & 0.669  & 0.595  & 0.597  & 0.676  & 0.691  & 0.602  & 0.728  & 0.633  & 0.542  & 0.678  & 0.678  \\
%     % fraud & 0.947  & 0.964  & 0.903  & 0.904  & 0.955  & 0.934  & 0.904  & 0.898  & 0.890  & 0.883  & 0.873  & 0.375  & 0.877  & 0.689  & 0.902  & 0.905  \\
%     % glass & 0.734  & 0.722  & 0.772  & 0.663  & 0.692  & 0.823  & 0.771  & 0.761  & 0.658  & 0.724  & 0.783  & 0.781  & 0.773  & 0.557  & 0.793  & 0.822  \\
%     % Hepatitis & 0.678  & 0.415  & 0.799  & 0.760  & 0.381  & 0.528  & 0.698  & 0.548  & 0.752  & 0.821  & 0.731  & 0.484  & 0.646  & 0.575  & 0.799  & 0.806  \\
%     % Ionosphere & 0.864  & 0.868  & 0.625  & 0.792  & 0.906  & 0.883  & 0.845  & 0.734  & 0.732  & 0.793  & 0.908  & 0.578  & 0.914  & 0.539  & 0.901  & 0.904  \\
%     % landsat & 0.595  & 0.535  & 0.551  & 0.358  & 0.539  & 0.580  & 0.476  & 0.439  & 0.361  & 0.416  & 0.637  & 0.334  & 0.553  & 0.625  & 0.577  & 0.574  \\
%     % letter & 0.841  & 0.800  & 0.597  & 0.503  & 0.845  & 0.862  & 0.611  & 0.504  & 0.560  & 0.543  & 0.737  & 0.532  & 0.760  & 0.559  & 0.732  & 0.739  \\
%     % Lymphography & 0.712  & 0.909  & 0.995  & 0.998  & 0.899  & 0.559  & 0.998  & 0.721  & 0.995  & 0.995  & 0.998  & 0.812  & 1.000  & 0.719  & 0.995  & 0.997  \\
%     % mnist & 0.601  & 0.708  & 0.604  & 0.853  & 0.671  & 0.806  & 0.810  & 0.672  & 0.746  & 0.777  & 0.800  & 0.652  & 0.825  & 0.510  & 0.866  & 0.866  \\
%     % musk  & 0.741  & 0.387  & 1.000  & 1.000  & 0.412  & 0.699  & 1.000  & 0.769  & 0.954  & 0.942  & 1.000  & 0.422  & 0.722  & 0.660  & 1.000  & 1.000  \\
%     % pendigits & 0.663  & 0.451  & 0.930  & 0.937  & 0.480  & 0.730  & 0.948  & 0.642  & 0.930  & 0.907  & 0.969  & 0.943  & 0.944  & 0.273  & 0.953  & 0.955  \\
%     % Pima  & 0.613  & 0.611  & 0.711  & 0.708  & 0.657  & 0.734  & 0.729  & 0.559  & 0.631  & 0.691  & 0.715  & 0.722  & 0.704  & 0.495  & 0.746  & 0.749  \\
%     % satellite & 0.640  & 0.547  & 0.748  & 0.596  & 0.559  & 0.652  & 0.704  & 0.623  & 0.581  & 0.632  & 0.713  & 0.560  & 0.677  & 0.574  & 0.778  & 0.777  \\
%     % satimage-2 & 0.831  & 0.567  & 0.977  & 0.976  & 0.474  & 0.926  & 0.992  & 0.963  & 0.963  & 0.972  & 0.998  & 0.860  & 0.999  & 0.557  & 0.999  & 0.999  \\
%     % shuttle & 0.695  & 0.517  & 0.986  & 0.986  & 0.571  & 0.696  & 0.996  & 0.979  & 0.991  & 0.994  & 0.931  & 0.972  & 0.700  & 0.518  & 0.985  & 0.988  \\
%     % skin  & 0.604  & 0.417  & 0.602  & 0.453  & 0.465  & 0.715  & 0.682  & N/A   & 0.491  & 0.476  & 0.680  & 0.643  & 0.655  & 0.457  & 0.710  & 0.697  \\
%     % SpamBase & 0.524  & 0.410  & 0.647  & 0.547  & 0.433  & 0.534  & 0.648  & N/A   & 0.669  & 0.701  & 0.552  & 0.503  & 0.563  & 0.503  & 0.543  & 0.544  \\
%     % Stamps & 0.733  & 0.538  & 0.907  & 0.915  & 0.513  & 0.686  & 0.912  & 0.889  & 0.879  & 0.934  & 0.699  & 0.934  & 0.798  & 0.595  & 0.908  & 0.942  \\
%     % vertebral & 0.403  & 0.487  & 0.286  & 0.371  & 0.493  & 0.338  & 0.367  & 0.532  & 0.407  & 0.256  & 0.410  & 0.381  & 0.381  & 0.378  & 0.407  & 0.474  \\
%     % vowels & 0.927  & 0.940  & 0.722  & 0.653  & 0.931  & 0.973  & 0.739  & 0.606  & 0.622  & 0.532  & 0.921  & 0.516  & 0.935  & 0.499  & 0.908  & 0.921  \\
%     % Waveform & 0.686  & 0.726  & 0.688  & 0.655  & 0.733  & 0.738  & 0.715  & 0.494  & 0.624  & 0.750  & 0.713  & 0.635  & 0.744  & 0.539  & 0.735  & 0.743  \\
%     % WBC   & 0.946  & 0.609  & 0.987  & 0.982  & 0.542  & 0.906  & 0.990  & N/A   & 0.991  & 0.991  & 0.969  & 0.949  & 0.975  & 0.625  & 0.989  & 0.989  \\
%     % Wilt  & 0.533  & 0.497  & 0.325  & 0.204  & 0.507  & 0.484  & 0.419  & 0.373  & 0.363  & 0.334  & 0.345  & 0.447  & 0.349  & 0.459  & 0.500  & 0.526  \\
%     % wine  & 0.461  & 0.444  & 0.914  & 0.844  & 0.377  & 0.450  & 0.804  & 0.617  & 0.772  & 0.887  & 0.271  & 0.822  & 0.274  & 0.643  & 0.932  & 0.953  \\
%     % WPBC  & 0.513  & 0.459  & 0.512  & 0.460  & 0.414  & 0.466  & 0.466  & 0.478  & 0.467  & 0.493  & 0.453  & 0.497  & 0.450  & 0.440  & 0.503  & 0.499  \\
%     ALOI & 61.10 & \textcolor{blue}{ 64.70 } & 52.60 & 56.70 & \textcolor{red}{ 66.60 } & \textcolor{darkgreen}{ 61.50 } & 56.70 & 52.00 & 56.30 & 53.80 & 55.30 & 52.80 & 54.90 & 50.50 & 56.60 & 56.60 \\
% backdoor & 68.80 & 73.10 & 71.60 & 80.20 & 85.80 & 80.60 & 72.20 & 56.00 & 86.10 & 81.00 & 81.90 & 79.60 & \textcolor{darkgreen}{ 89.10 } & 78.80 & \textcolor{red}{ 89.50 } & \textcolor{blue}{ 89.20 } \\
% breastw & 94.00 & 38.80 & 98.90 & 95.10 & 40.60 & 97.00 & 98.30 & N/A & \textcolor{blue}{ 99.20 } & \textcolor{red}{ 99.70 } & 96.90 & \textcolor{darkgreen}{ 99.00 } & 97.10 & 63.40 & 98.40 & 98.60 \\
% campaign & 69.20 & 57.40 & \textcolor{red}{ 78.60 } & 72.80 & 59.00 & 72.30 & 71.70 & 56.00 & \textcolor{darkgreen}{ 76.10 } & \textcolor{blue}{ 77.70 } & 64.30 & 63.20 & 63.50 & 54.40 & 73.40 & 73.60 \\
% celeba & 48.40 & 38.60 & 76.20 & 79.40 & 39.00 & 59.60 & 70.40 & 44.70 & 76.50 & 75.70 & 74.00 & \textcolor{red}{ 91.40 } & 56.80 & 45.20 & \textcolor{blue}{ 82.70 } & \textcolor{darkgreen}{ 82.00 } \\
% census & 62.10 & 41.60 & 64.90 & \textcolor{darkgreen}{ 68.70 } & 47.50 & 66.90 & 59.50 & 59.70 & 67.60 & \textcolor{blue}{ 69.10 } & 60.20 & \textcolor{red}{ 72.80 } & 63.30 & 54.20 & 67.80 & 67.80 \\
% fraud & \textcolor{darkgreen}{ 94.70 } & \textcolor{red}{ 96.40 } & 90.30 & 90.40 & \textcolor{blue}{ 95.50 } & 93.40 & 90.40 & 89.80 & 89.00 & 88.30 & 87.30 & 37.50 & 87.70 & 68.90 & 90.20 & 90.50 \\
% glass & 73.40 & 72.20 & 77.20 & 66.30 & 69.20 & \textcolor{red}{ 82.30 } & 77.10 & 76.10 & 65.80 & 72.40 & 78.30 & 78.10 & 77.30 & 55.70 & \textcolor{darkgreen}{ 79.30 } & \textcolor{blue}{ 82.20 } \\
% Hepatitis & 67.80 & 41.50 & 79.90 & 76.00 & 38.10 & 52.80 & 69.80 & 54.80 & 75.20 & \textcolor{red}{ 82.10 } & 73.10 & 48.40 & 64.60 & 57.50 & \textcolor{darkgreen}{ 79.90 } & \textcolor{blue}{ 80.60 } \\
% Ionosphere & 86.40 & 86.80 & 62.50 & 79.20 & \textcolor{darkgreen}{ 90.60 } & 88.30 & 84.50 & 73.40 & 73.20 & 79.30 & \textcolor{blue}{ 90.80 } & 57.80 & \textcolor{red}{ 91.40 } & 53.90 & 90.10 & 90.40 \\
% landsat & \textcolor{darkgreen}{ 59.50 } & 53.50 & 55.10 & 35.80 & 53.90 & 58.00 & 47.60 & 43.90 & 36.10 & 41.60 & \textcolor{red}{ 63.70 } & 33.40 & 55.30 & \textcolor{blue}{ 62.50 } & 57.70 & 57.40 \\
% letter & \textcolor{darkgreen}{ 84.10 } & 80.00 & 59.70 & 50.30 & \textcolor{blue}{ 84.50 } & \textcolor{red}{ 86.20 } & 61.10 & 50.40 & 56.00 & 54.30 & 73.70 & 53.20 & 76.00 & 55.90 & 73.20 & 73.90 \\
% Lymphography & 71.20 & 90.90 & 99.50 & 99.80 & 89.90 & 55.90 & \textcolor{darkgreen}{ 99.80 } & 72.10 & 99.50 & 99.50 & \textcolor{blue}{ 99.80 } & 81.20 & \textcolor{red}{ 100.00 } & 71.90 & 99.50 & 99.70 \\
% mnist & 60.10 & 70.80 & 60.40 & \textcolor{darkgreen}{ 85.30 } & 67.10 & 80.60 & 81.00 & 67.20 & 74.60 & 77.70 & 80.00 & 65.20 & 82.50 & 51.00 & \textcolor{blue}{ 86.60 } & \textcolor{red}{ 86.60 } \\
% musk & 74.10 & 38.70 & 100.00 & 100.00 & 41.20 & 69.90 & 100.00 & 76.90 & 95.40 & 94.20 & \textcolor{darkgreen}{ 100.00 } & 42.20 & 72.20 & 66.00 & \textcolor{blue}{ 100.00 } & \textcolor{red}{ 100.00 } \\
% pendigits & 66.30 & 45.10 & 93.00 & 93.70 & 48.00 & 73.00 & 94.80 & 64.20 & 93.00 & 90.70 & \textcolor{red}{ 96.90 } & 94.30 & 94.40 & 27.30 & \textcolor{darkgreen}{ 95.30 } & \textcolor{blue}{ 95.50 } \\
% Pima & 61.30 & 61.10 & 71.10 & 70.80 & 65.70 & \textcolor{darkgreen}{ 73.40 } & 72.90 & 55.90 & 63.10 & 69.10 & 71.50 & 72.20 & 70.40 & 49.50 & \textcolor{blue}{ 74.60 } & \textcolor{red}{ 74.90 } \\
% satellite & 64.00 & 54.70 & \textcolor{darkgreen}{ 74.80 } & 59.60 & 55.90 & 65.20 & 70.40 & 62.30 & 58.10 & 63.20 & 71.30 & 56.00 & 67.70 & 57.40 & \textcolor{red}{ 77.80 } & \textcolor{blue}{ 77.70 } \\
% satimage-2 & 83.10 & 56.70 & 97.70 & 97.60 & 47.40 & 92.60 & 99.20 & 96.30 & 96.30 & 97.20 & 99.80 & 86.00 & \textcolor{darkgreen}{ 99.90 } & 55.70 & \textcolor{blue}{ 99.90 } & \textcolor{red}{ 99.90 } \\
% shuttle & 69.50 & 51.70 & 98.60 & 98.60 & 57.10 & 69.60 & \textcolor{red}{ 99.60 } & 97.90 & \textcolor{darkgreen}{ 99.10 } & \textcolor{blue}{ 99.40 } & 93.10 & 97.20 & 70.00 & 51.80 & 98.50 & 98.80 \\
% skin & 60.40 & 41.70 & 60.20 & 45.30 & 46.50 & \textcolor{red}{ 71.50 } & 68.20 & N/A & 49.10 & 47.60 & 68.00 & 64.30 & 65.50 & 45.70 & \textcolor{blue}{ 71.00 } & \textcolor{darkgreen}{ 69.70 } \\
% SpamBase & 52.40 & 41.00 & 64.70 & 54.70 & 43.30 & 53.40 & \textcolor{darkgreen}{ 64.80 } & N/A & \textcolor{blue}{ 66.90 } & \textcolor{red}{ 70.10 } & 55.20 & 50.30 & 56.30 & 50.30 & 54.30 & 54.40 \\
% Stamps & 73.30 & 53.80 & 90.70 & 91.50 & 51.30 & 68.60 & 91.20 & 88.90 & 87.90 & \textcolor{darkgreen}{ 93.40 } & 69.90 & \textcolor{blue}{ 93.40 } & 79.80 & 59.50 & 90.80 & \textcolor{red}{ 94.20 } \\
% vertebral & 40.30 & \textcolor{darkgreen}{ 48.70 } & 28.60 & 37.10 & \textcolor{blue}{ 49.30 } & 33.80 & 36.70 & \textcolor{red}{ 53.20 } & 40.70 & 25.60 & 41.00 & 38.10 & 38.10 & 37.80 & 40.70 & 47.40 \\
% vowels & 92.70 & \textcolor{blue}{ 94.00 } & 72.20 & 65.30 & 93.10 & \textcolor{red}{ 97.30 } & 73.90 & 60.60 & 62.20 & 53.20 & 92.10 & 51.60 & \textcolor{darkgreen}{ 93.50 } & 49.90 & 90.80 & 92.10 \\
% Waveform & 68.60 & 72.60 & 68.80 & 65.50 & 73.30 & 73.80 & 71.50 & 49.40 & 62.40 & \textcolor{red}{ 75.00 } & 71.30 & 63.50 & \textcolor{blue}{ 74.40 } & 53.90 & 73.50 & \textcolor{darkgreen}{ 74.30 } \\
% WBC & 94.60 & 60.90 & 98.70 & 98.20 & 54.20 & 90.60 & \textcolor{darkgreen}{ 99.00 } & N/A & \textcolor{blue}{ 99.10 } & \textcolor{red}{ 99.10 } & 96.90 & 94.90 & 97.50 & 62.50 & 98.90 & 98.90 \\
% Wilt & \textcolor{red}{ 53.30 } & 49.70 & 32.50 & 20.40 & \textcolor{darkgreen}{ 50.70 } & 48.40 & 41.90 & 37.30 & 36.30 & 33.40 & 34.50 & 44.70 & 34.90 & 45.90 & 50.00 & \textcolor{blue}{ 52.60 } \\
% wine & 46.10 & 44.40 & \textcolor{darkgreen}{ 91.40 } & 84.40 & 37.70 & 45.00 & 80.40 & 61.70 & 77.20 & 88.70 & 27.10 & 82.20 & 27.40 & 64.30 & \textcolor{blue}{ 93.20 } & \textcolor{red}{ 95.30 } \\
% WPBC & \textcolor{red}{ 51.30 } & 45.90 & \textcolor{blue}{ 51.20 } & 46.00 & 41.40 & 46.60 & 46.60 & 47.80 & 46.70 & 49.30 & 45.30 & 49.70 & 45.00 & 44.00 & \textcolor{darkgreen}{ 50.30 } & 49.90 \\

%     \midrule
%     \textbf{Avg. Rank} & \textbf{9.2 } & \textbf{11.2 } & \textbf{7.7 } & \textbf{8.5 } & \textbf{10.6 } & \textbf{7.8 } & \textcolor{darkgreen}{\textbf{7.0}} & \textbf{11.3 } & \textbf{8.3 } & \textbf{7.6 } & \textbf{7.4 } & \textbf{9.8 } & \textbf{7.6 } & \textbf{13.3 } & \textcolor{blue}{\textbf{4.6 }} & \textcolor{red}{\textbf{3.6 }} \\
%     \bottomrule
%     \end{tabular}%

%    \end{adjustbox} 
%   \label{tab:sel30_auc}%
% \end{table*}%



==> tables/sel30_pr.tex <==
\begin{table*}[htbp]
  \centering
  \caption{AUCPR of 14 unsupervised algorithms on tabular benchmark datasets. 
  In each dataset, the highest score is highlighted in \textbf{bold}, and the second-highest score is \underline{underlined}.}
  \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{c|cccccccccccccccc|c}
    \toprule
    \textbf{Dataset} & \textbf{CBLOF} & \textbf{COF} & \textbf{COPOD} & \makecell{\textbf{DA} \\ \textbf{GMM}} & \makecell{\textbf{Deep} \\ \textbf{SVDD}} & \textbf{ECOD} & \textbf{GMM} & \textbf{HBOS} & \textbf{IForest} & \textbf{KNN} & \textbf{LODA} & \textbf{LOF} & \makecell{\textbf{OC} \\ \textbf{SVM}} & \textbf{PCA} & \textbf{SOD} & \textbf{KMeans-$ $-} & \textbf{Galaxy} \\
    \midrule
    
backdoor & 0.070 & 0.238 & 0.077 & 0.055 & \underline{0.557} & 0.107 & \textbf{0.564} & 0.050 & 0.048 & 0.444 & 0.138 & 0.261 & 0.088 & 0.313 & 0.371 & 0.155 & 0.364 \\
breastw & 0.919 & 0.276 & \textbf{0.994} & N/A & 0.486 & \underline{0.985} & 0.914 & 0.977 & 0.960 & 0.922 & 0.970 & 0.285 & 0.827 & 0.951 & 0.849 & 0.922 & 0.959 \\
campaign & 0.209 & 0.130 & \textbf{0.386} & 0.145 & 0.168 & 0.367 & 0.294 & \underline{0.380} & 0.323 & 0.272 & 0.141 & 0.146 & 0.292 & 0.279 & 0.191 & 0.189 & 0.271 \\
cardio & 0.619 & 0.287 & 0.604 & 0.289 & 0.225 & 0.597 & 0.510 & 0.521 & 0.599 & 0.407 & 0.534 & 0.238 & \underline{0.629} & \textbf{0.661} & 0.285 & 0.382 & 0.563 \\
celeba & 0.112 & 0.018 & 0.137 & 0.019 & 0.027 & 0.140 & 0.101 & 0.138 & 0.090 & 0.031 & 0.040 & 0.017 & 0.107 & \textbf{0.159} & 0.024 & 0.032 & \underline{0.147} \\
census & 0.075 & 0.049 & \underline{0.099} & 0.090 & 0.084 & 0.095 & 0.097 & 0.087 & 0.078 & 0.090 & 0.050 & 0.055 & 0.068 & \textbf{0.100} & 0.085 & 0.081 & 0.098 \\
donors & 0.180 & 0.089 & 0.216 & 0.107 & 0.177 & \textbf{0.270} & 0.147 & \underline{0.244} & 0.127 & 0.160 & 0.039 & 0.085 & 0.104 & 0.179 & 0.103 & N/A & 0.142 \\
fraud & 0.392 & 0.215 & \underline{0.428} & 0.157 & 0.215 & 0.374 & 0.118 & 0.280 & 0.217 & 0.376 & 0.396 & \textbf{0.466} & 0.403 & 0.229 & 0.175 & 0.395 & 0.423 \\
glass & 0.116 & 0.118 & 0.098 & \textbf{0.246} & 0.085 & 0.154 & 0.128 & 0.118 & 0.110 & \underline{0.203} & 0.134 & 0.201 & 0.080 & 0.100 & 0.187 & 0.147 & 0.153 \\
Hepatitis & 0.365 & 0.144 & \underline{0.415} & 0.229 & 0.300 & 0.328 & 0.332 & 0.377 & 0.263 & 0.220 & 0.309 & 0.137 & 0.294 & 0.366 & 0.247 & 0.251 & \textbf{0.434} \\
Ionosphere & 0.898 & 0.829 & 0.699 & 0.650 & 0.432 & 0.647 & \underline{0.906} & 0.418 & 0.804 & 0.904 & 0.730 & 0.881 & 0.745 & 0.739 & 0.859 & \textbf{0.914} & 0.876 \\
landsat & \underline{0.311} & 0.250 & 0.175 & 0.245 & \textbf{0.369} & 0.162 & 0.184 & 0.220 & 0.198 & 0.246 & 0.189 & 0.247 & 0.162 & 0.162 & 0.264 & 0.224 & 0.233 \\
letter & 0.139 & 0.214 & 0.068 & 0.117 & 0.088 & 0.076 & 0.183 & 0.084 & 0.085 & \underline{0.300} & 0.069 & \textbf{0.340} & 0.061 & 0.069 & 0.286 & 0.153 & 0.143 \\
Lymphography & 0.973 & 0.367 & 0.887 & 0.195 & 0.346 & 0.909 & 0.715 & 0.918 & \underline{0.973} & 0.387 & 0.445 & 0.231 & 0.936 & 0.970 & 0.220 & \textbf{1.000} & 0.967 \\
magic.gamma & \underline{0.688} & 0.541 & 0.592 & 0.469 & 0.487 & 0.537 & 0.667 & 0.624 & 0.647 & \textbf{0.756} & 0.585 & 0.548 & 0.514 & 0.593 & 0.679 & 0.683 & 0.650 \\
mnist & 0.306 & 0.255 & 0.213 & 0.237 & 0.202 & 0.175 & 0.387 & 0.125 & 0.277 & 0.355 & 0.259 & 0.209 & 0.332 & \underline{0.399} & 0.192 & 0.371 & \textbf{0.419} \\
musk & 1.000 & 0.026 & 0.348 & 0.328 & 0.088 & 0.501 & 0.903 & \underline{1.000} & 0.996 & 0.097 & 0.476 & 0.028 & 0.106 & 0.999 & 0.076 & 0.375 & \textbf{1.000} \\
pendigits & \textbf{0.329} & 0.029 & 0.212 & 0.047 & 0.015 & 0.306 & 0.064 & 0.293 & 0.261 & 0.065 & 0.187 & 0.038 & 0.235 & 0.236 & 0.045 & \underline{0.327} & 0.217 \\
Pima & 0.530 & 0.447 & 0.552 & 0.415 & 0.350 & 0.505 & 0.533 & \textbf{0.566} & \underline{0.558} & 0.551 & 0.441 & 0.472 & 0.500 & 0.540 & 0.482 & 0.535 & 0.542 \\
satellite & 0.614 & 0.397 & 0.566 & 0.583 & 0.418 & 0.522 & 0.498 & \underline{0.672} & 0.659 & 0.500 & 0.619 & 0.377 & 0.576 & 0.596 & 0.472 & 0.547 & \textbf{0.751} \\
satimage-2 & 0.971 & 0.088 & 0.765 & 0.221 & 0.026 & 0.645 & 0.436 & 0.780 & 0.934 & 0.391 & 0.805 & 0.043 & 0.827 & 0.857 & 0.261 & \underline{0.971} & \textbf{0.973} \\
shuttle & 0.799 & 0.122 & \underline{0.966} & 0.932 & 0.124 & 0.904 & 0.882 & 0.964 & \textbf{0.976} & 0.204 & 0.488 & 0.138 & 0.853 & 0.924 & 0.203 & 0.327 & 0.924 \\
skin & 0.283 & 0.164 & 0.180 & N/A & 0.191 & 0.184 & 0.286 & 0.237 & 0.261 & \underline{0.287} & 0.184 & 0.183 & 0.190 & 0.174 & 0.246 & 0.256 & \textbf{0.287} \\
Stamps & 0.245 & 0.165 & 0.431 & \underline{0.437} & 0.121 & 0.332 & 0.350 & 0.352 & 0.395 & 0.235 & 0.346 & 0.213 & 0.314 & 0.411 & 0.203 & 0.356 & \textbf{0.509} \\
vertebral & 0.114 & 0.138 & 0.089 & \textbf{0.152} & 0.106 & 0.118 & 0.114 & 0.092 & 0.105 & 0.106 & 0.097 & \underline{0.142} & 0.109 & 0.105 & 0.118 & 0.105 & 0.130 \\
Waveform & \underline{0.179} & 0.141 & 0.069 & 0.031 & 0.044 & 0.048 & 0.043 & 0.059 & 0.062 & 0.130 & 0.047 & 0.113 & 0.044 & 0.058 & 0.097 & \textbf{0.197} & 0.078 \\
WBC & 0.673 & 0.097 & 0.862 & N/A & 0.090 & 0.862 & 0.443 & 0.736 & \textbf{0.905} & 0.666 & 0.787 & 0.056 & \underline{0.899} & 0.823 & 0.540 & 0.719 & 0.831 \\
Wilt & 0.037 & 0.050 & 0.037 & 0.040 & 0.047 & 0.039 & \textbf{0.072} & 0.038 & 0.042 & 0.047 & 0.034 & 0.050 & 0.036 & 0.031 & \underline{0.055} & 0.038 & 0.052 \\
wine & 0.060 & 0.085 & 0.457 & 0.175 & 0.188 & 0.235 & 0.107 & 0.431 & 0.260 & 0.084 & \underline{0.488} & 0.078 & 0.216 & 0.309 & 0.080 & 0.063 & \textbf{0.496} \\
WPBC & 0.211 & 0.213 & 0.228 & 0.225 & 0.250 & 0.212 & 0.216 & 0.230 & 0.224 & 0.215 & \underline{0.254} & 0.203 & 0.229 & 0.230 & \textbf{0.256} & 0.206 & 0.249 \\

    \midrule
    Avg. Rank & 7.3   & 12.4  & 7.8   & 10.9  & 12.1  & 8.5   & 8.2   & 7.5   & 7.5   & 8.2   & 10.0  & 11.6  & 9.9   & 7.5   & 10.1  & 8.0   & 4.5  \\
    Win Nums & 1     & 0     & 2     & 2     & 1     & 1     & 2     & 2     & 2     & 2     & 0     & 2     & 0     & 3     & 1     & 3     & 6  \\
    Top3 Nums & 8     & 2     & 10    & 3     & 3     & 5     & 5     & 8     & 5     & 6     & 2     & 4     & 2     & 4     & 4     & 6     & 12  \\
    \bottomrule
    \end{tabular}%
\end{adjustbox}
  \label{tab:sel30_pr}%
\end{table*}%


==> tables/top30.tex <==
% Table generated by Excel2LaTeX from sheet 'report_auc'
\begin{table*}[t]
  \centering
  \caption{AUCROC of 14 unsupervised algorithms on 30 tabular benchmark datasets. 
  In each dataset, the algorithm with the highest AUCROC is marked in \textcolor{red}{red}, the second highest in \textcolor{blue}{blue}, and the third highest in \textcolor{darkgreen}{green}.}
  \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{c|cccccccccccccc|cc}
    \toprule
    \textbf{Dataset} & \textbf{SOD} & \textbf{COF} & \textbf{HBOS} & \textbf{PCA} & \textbf{LOF} & \textbf{KNN} & \textbf{IForest} & \textbf{DAGMM} & \textbf{ECOD} & \textbf{COPOD} & \textbf{CBLOF} & \textbf{DCFOD} & \boldmath{}\textbf{KMeans-$ $-}\unboldmath{} & \makecell{\textbf{Deep} \\ \textbf{SVDD} } & \makecell{\textbf{\model} \\ \textbf{(Scalar)}} & \makecell{\textbf{\model} \\ \textbf{(Vector)}} \\
\midrule
    annthyroid & \textcolor{darkgreen}{ 77.40 } & 65.90 & 60.10 & 66.20 & 70.20 & 71.70 & \textcolor{red}{ 82.00 } & 56.50 & \textcolor{blue}{ 78.70 } & 76.80 & 62.30 & 55.00 & 65.00 & 76.10 & 75.30 & 72.70 \\
backdoor & 68.80 & 73.10 & 71.60 & 80.20 & 85.80 & 80.60 & 72.20 & 56.00 & 86.10 & 81.00 & 81.90 & 79.60 & \textcolor{blue}{ 89.10 } & 78.80 & \textcolor{darkgreen}{ 87.30 } & \textcolor{red}{ 89.20 } \\
breastw & 94.00 & 38.80 & 98.90 & 95.10 & 40.60 & 97.00 & 98.30 & N/A & \textcolor{blue}{ 99.20 } & \textcolor{red}{ 99.70 } & 96.90 & \textcolor{darkgreen}{ 99.00 } & 97.00 & 63.40 & 98.10 & 98.60 \\
campaign & 69.20 & 57.40 & \textcolor{red}{ 78.50 } & 72.80 & 59.00 & 72.30 & 71.70 & 56.00 & \textcolor{darkgreen}{ 76.10 } & \textcolor{blue}{ 77.70 } & 64.30 & 63.20 & 63.50 & 54.40 & 73.50 & 73.60 \\
cardio & 73.20 & 71.40 & 84.70 & \textcolor{red}{ 95.60 } & 66.30 & 76.60 & 93.20 & 75.00 & \textcolor{darkgreen}{ 93.60 } & 92.30 & 90.60 & \textcolor{blue}{ 93.90 } & 78.90 & 53.40 & 91.80 & 92.20 \\
celeba & 48.40 & 38.60 & 76.20 & 79.40 & 39.00 & 59.60 & 70.40 & 44.70 & 76.50 & 75.70 & 74.00 & \textcolor{red}{ 91.40 } & 56.80 & 45.20 & \textcolor{darkgreen}{ 81.40 } & \textcolor{blue}{ 82.00 } \\
census & 62.10 & 41.60 & 64.90 & \textcolor{darkgreen}{ 68.70 } & 47.50 & 66.90 & 59.50 & 59.70 & 67.60 & \textcolor{blue}{ 69.10 } & 60.20 & \textcolor{red}{ 72.80 } & 63.30 & 54.20 & 67.90 & 67.80 \\
glass & 73.40 & 72.20 & 77.20 & 66.30 & 69.20 & \textcolor{red}{ 82.30 } & 77.10 & 76.10 & 65.80 & 72.40 & 78.30 & 78.10 & 77.30 & 55.70 & \textcolor{darkgreen}{ 79.50 } & \textcolor{blue}{ 82.20 } \\
Hepatitis & 67.80 & 41.50 & \textcolor{darkgreen}{ 79.90 } & 75.90 & 38.10 & 52.80 & 69.80 & 54.80 & 75.20 & \textcolor{red}{ 82.10 } & 73.10 & 48.40 & 64.60 & 57.40 & 75.50 & \textcolor{blue}{ 80.60 } \\
Ionosphere & 86.40 & 86.80 & 62.50 & 79.20 & 90.60 & 88.30 & 84.50 & 73.40 & 73.20 & 79.30 & \textcolor{darkgreen}{ 90.80 } & 57.80 & \textcolor{blue}{ 91.40 } & 53.90 & \textcolor{red}{ 92.00 } & 90.40 \\
landsat & \textcolor{darkgreen}{ 59.50 } & 53.50 & 55.10 & 35.80 & 53.90 & 58.00 & 47.60 & 43.90 & 36.10 & 41.50 & \textcolor{red}{ 63.70 } & 33.40 & 55.30 & \textcolor{blue}{ 62.50 } & 49.60 & 57.40 \\
letter & \textcolor{darkgreen}{ 84.10 } & 80.00 & 59.70 & 50.30 & \textcolor{blue}{ 84.50 } & \textcolor{red}{ 86.20 } & 61.10 & 50.40 & 56.00 & 54.30 & 73.70 & 53.20 & 76.00 & 55.90 & 71.20 & 73.80 \\
Lymphography & 71.20 & 90.80 & 99.50 & 99.80 & 89.90 & 55.90 & \textcolor{darkgreen}{ 99.80 } & 72.10 & 99.50 & 99.50 & \textcolor{blue}{ 99.80 } & 81.20 & \textcolor{red}{ 100.00 } & 71.90 & 99.30 & 99.70 \\
mnist & 60.10 & 70.80 & 60.40 & \textcolor{darkgreen}{ 85.30 } & 67.10 & 80.60 & 81.00 & 67.20 & 74.60 & 77.70 & 80.00 & 65.20 & 82.50 & 51.00 & \textcolor{blue}{ 86.00 } & \textcolor{red}{ 86.60 } \\
musk & 74.10 & 38.70 & 100.00 & 100.00 & 41.20 & 69.90 & \textcolor{darkgreen}{ 100.00 } & 76.90 & 95.40 & 94.20 & \textcolor{blue}{ 100.00 } & 42.20 & 72.20 & 66.00 & 99.90 & \textcolor{red}{ 100.00 } \\
pendigits & 66.30 & 45.10 & 93.00 & 93.70 & 48.00 & 72.90 & 94.80 & 64.20 & 93.00 & 90.70 & \textcolor{red}{ 96.90 } & 94.30 & 94.40 & 27.30 & \textcolor{darkgreen}{ 95.10 } & \textcolor{blue}{ 95.50 } \\
Pima & 61.30 & 61.00 & 71.10 & 70.80 & 65.70 & \textcolor{darkgreen}{ 73.40 } & 72.90 & 55.90 & 63.10 & 69.10 & 71.50 & 72.20 & 70.40 & 49.50 & \textcolor{red}{ 75.20 } & \textcolor{blue}{ 74.90 } \\
satellite & 64.00 & 54.70 & \textcolor{blue}{ 74.80 } & 59.60 & 55.90 & 65.20 & 70.40 & 62.30 & 58.10 & 63.20 & 71.30 & 56.00 & 67.70 & 57.40 & \textcolor{darkgreen}{ 72.50 } & \textcolor{red}{ 77.70 } \\
satimage-2 & 83.10 & 56.70 & 97.60 & 97.60 & 47.40 & 92.60 & 99.20 & 96.30 & 96.30 & 97.20 & 99.80 & 86.00 & \textcolor{darkgreen}{ 99.90 } & 55.70 & \textcolor{blue}{ 99.90 } & \textcolor{red}{ 99.90 } \\
shuttle & 69.50 & 51.70 & 98.60 & 98.60 & 57.10 & 69.60 & \textcolor{red}{ 99.60 } & 97.90 & 99.10 & \textcolor{blue}{ 99.40 } & 93.10 & 97.20 & 70.00 & 51.80 & \textcolor{darkgreen}{ 99.20 } & 98.70 \\
skin & 60.30 & 41.70 & 60.20 & 45.30 & 46.50 & \textcolor{blue}{ 71.50 } & 68.20 & N/A & 49.10 & 47.60 & 68.00 & 64.30 & 65.50 & 45.70 & \textcolor{red}{ 72.30 } & \textcolor{darkgreen}{ 69.70 } \\
Stamps & 73.30 & 53.80 & 90.70 & 91.50 & 51.30 & 68.60 & 91.20 & 88.90 & 87.90 & \textcolor{darkgreen}{ 93.40 } & 69.90 & \textcolor{blue}{ 93.40 } & 79.80 & 59.50 & 91.40 & \textcolor{red}{ 94.20 } \\
thyroid & 92.80 & 90.90 & 95.60 & 96.30 & 86.90 & 95.90 & \textcolor{red}{ 98.30 } & 79.80 & \textcolor{blue}{ 97.90 } & 94.30 & 94.70 & 78.60 & 92.30 & 52.10 & \textcolor{darkgreen}{ 97.70 } & 97.50 \\
vertebral & 40.30 & \textcolor{darkgreen}{ 48.70 } & 28.60 & 37.10 & \textcolor{blue}{ 49.30 } & 33.80 & 36.70 & \textcolor{red}{ 53.20 } & 40.70 & 25.60 & 41.00 & 38.10 & 38.10 & 37.80 & 33.10 & 47.40 \\
vowels & 92.70 & \textcolor{blue}{ 94.00 } & 72.20 & 65.30 & 93.10 & \textcolor{red}{ 97.30 } & 73.90 & 60.60 & 62.20 & 53.20 & 92.10 & 51.60 & \textcolor{darkgreen}{ 93.50 } & 49.90 & 88.40 & 92.10 \\
Waveform & 68.60 & 72.60 & 68.80 & 65.50 & 73.30 & 73.80 & 71.50 & 49.30 & 62.40 & \textcolor{red}{ 75.00 } & 71.30 & 63.50 & \textcolor{blue}{ 74.40 } & 53.90 & 71.80 & \textcolor{darkgreen}{ 74.30 } \\
WBC & 94.60 & 60.90 & 98.70 & 98.20 & 54.20 & 90.60 & \textcolor{darkgreen}{ 99.00 } & N/A & \textcolor{blue}{ 99.10 } & \textcolor{red}{ 99.10 } & 96.90 & 94.90 & 97.40 & 62.50 & 97.70 & 98.90 \\
Wilt & \textcolor{red}{ 53.30 } & 49.70 & 32.50 & 20.40 & \textcolor{darkgreen}{ 50.70 } & 48.40 & 41.90 & 37.30 & 36.30 & 33.40 & 34.50 & 44.70 & 34.90 & 45.90 & 49.00 & \textcolor{blue}{ 52.60 } \\
wine & 46.10 & 44.40 & \textcolor{blue}{ 91.40 } & 84.40 & 37.70 & 45.00 & 80.40 & 61.70 & 77.20 & \textcolor{darkgreen}{ 88.70 } & 27.10 & 82.20 & 27.40 & 64.30 & 82.70 & \textcolor{red}{ 95.20 } \\
WPBC & \textcolor{red}{ 51.30 } & 45.90 & \textcolor{blue}{ 51.20 } & 46.00 & 41.40 & 46.60 & 46.60 & 47.80 & 46.60 & 49.30 & 45.30 & 49.70 & 45.00 & 44.00 & 48.00 & \textcolor{darkgreen}{ 49.90 } \\
\midrule
    % annthyroid & 0.774  & 0.659  & 0.601  & 0.662  & 0.702  & 0.717  & 0.820  & 0.565  & 0.787  & 0.768  & 0.623  & 0.550  & 0.650  & 0.761  & 0.753  & 0.727  \\
    % backdoor & 0.688  & 0.731  & 0.716  & 0.802  & 0.858  & 0.806  & 0.722  & 0.560  & 0.861  & 0.810  & 0.819  & 0.796  & 0.891  & 0.788  & 0.873  & 0.892  \\
    % breastw & 0.940  & 0.388  & 0.989  & 0.951  & 0.406  & 0.970  & 0.983  & N/A   & 0.992  & 0.997  & 0.969  & 0.990  & 0.970  & 0.634  & 0.981  & 0.986  \\
    % campaign & 0.692  & 0.574  & 0.785  & 0.728  & 0.590  & 0.723  & 0.717  & 0.560  & 0.761  & 0.777  & 0.643  & 0.632  & 0.635  & 0.544  & 0.735  & 0.736  \\
    % cardio & 0.732  & 0.714  & 0.847  & 0.956  & 0.663  & 0.766  & 0.932  & 0.750  & 0.936  & 0.923  & 0.906  & 0.939  & 0.789  & 0.534  & 0.918  & 0.922  \\
    % celeba & 0.484  & 0.386  & 0.762  & 0.794  & 0.390  & 0.596  & 0.704  & 0.447  & 0.765  & 0.757  & 0.740  & 0.914  & 0.568  & 0.452  & 0.814  & 0.820  \\
    % census & 0.621  & 0.416  & 0.649  & 0.687  & 0.475  & 0.669  & 0.595  & 0.597  & 0.676  & 0.691  & 0.602  & 0.728  & 0.633  & 0.542  & 0.679  & 0.678  \\
    % glass & 0.734  & 0.722  & 0.772  & 0.663  & 0.692  & 0.823  & 0.771  & 0.761  & 0.658  & 0.724  & 0.783  & 0.781  & 0.773  & 0.557  & 0.795  & 0.822  \\
    % Hepatitis & 0.678  & 0.415  & 0.799  & 0.759  & 0.381  & 0.528  & 0.698  & 0.548  & 0.752  & 0.821  & 0.731  & 0.484  & 0.646  & 0.574  & 0.755  & 0.806  \\
    % Ionosphere & 0.864  & 0.868  & 0.625  & 0.792  & 0.906  & 0.883  & 0.845  & 0.734  & 0.732  & 0.793  & 0.908  & 0.578  & 0.914  & 0.539  & 0.920  & 0.904  \\
    % landsat & 0.595  & 0.535  & 0.551  & 0.358  & 0.539  & 0.580  & 0.476  & 0.439  & 0.361  & 0.415  & 0.637  & 0.334  & 0.553  & 0.625  & 0.496  & 0.574  \\
    % letter & 0.841  & 0.800  & 0.597  & 0.503  & 0.845  & 0.862  & 0.611  & 0.504  & 0.560  & 0.543  & 0.737  & 0.532  & 0.760  & 0.559  & 0.712  & 0.738  \\
    % Lymphography & 0.712  & 0.908  & 0.995  & 0.998  & 0.899  & 0.559  & 0.998  & 0.721  & 0.995  & 0.995  & 0.998  & 0.812  & 1.000  & 0.719  & 0.993  & 0.997  \\
    % mnist & 0.601  & 0.708  & 0.604  & 0.853  & 0.671  & 0.806  & 0.810  & 0.672  & 0.746  & 0.777  & 0.800  & 0.652  & 0.825  & 0.510  & 0.860  & 0.866  \\
    % musk  & 0.741  & 0.387  & 1.000  & 1.000  & 0.412  & 0.699  & 1.000  & 0.769  & 0.954  & 0.942  & 1.000  & 0.422  & 0.722  & 0.660  & 0.999  & 1.000  \\
    % pendigits & 0.663  & 0.451  & 0.930  & 0.937  & 0.480  & 0.729  & 0.948  & 0.642  & 0.930  & 0.907  & 0.969  & 0.943  & 0.944  & 0.273  & 0.951  & 0.955  \\
    % Pima  & 0.613  & 0.610  & 0.711  & 0.708  & 0.657  & 0.734  & 0.729  & 0.559  & 0.631  & 0.691  & 0.715  & 0.722  & 0.704  & 0.495  & 0.752  & 0.749  \\
    % satellite & 0.640  & 0.547  & 0.748  & 0.596  & 0.559  & 0.652  & 0.704  & 0.623  & 0.581  & 0.632  & 0.713  & 0.560  & 0.677  & 0.574  & 0.725  & 0.777  \\
    % satimage-2 & 0.831  & 0.567  & 0.976  & 0.976  & 0.474  & 0.926  & 0.992  & 0.963  & 0.963  & 0.972  & 0.998  & 0.860  & 0.999  & 0.557  & 0.999  & 0.999  \\
    % shuttle & 0.695  & 0.517  & 0.986  & 0.986  & 0.571  & 0.696  & 0.996  & 0.979  & 0.991  & 0.994  & 0.931  & 0.972  & 0.700  & 0.518  & 0.992  & 0.987  \\
    % skin  & 0.603  & 0.417  & 0.602  & 0.453  & 0.465  & 0.715  & 0.682  & N/A   & 0.491  & 0.476  & 0.680  & 0.643  & 0.655  & 0.457  & 0.723  & 0.697  \\
    % Stamps & 0.733  & 0.538  & 0.907  & 0.915  & 0.513  & 0.686  & 0.912  & 0.889  & 0.879  & 0.934  & 0.699  & 0.934  & 0.798  & 0.595  & 0.914  & 0.942  \\
    % thyroid & 0.928  & 0.909  & 0.956  & 0.963  & 0.869  & 0.959  & 0.983  & 0.798  & 0.979  & 0.943  & 0.947  & 0.786  & 0.923  & 0.521  & 0.977  & 0.975  \\
    % vertebral & 0.403  & 0.487  & 0.286  & 0.371  & 0.493  & 0.338  & 0.367  & 0.532  & 0.407  & 0.256  & 0.410  & 0.381  & 0.381  & 0.378  & 0.331  & 0.474  \\
    % vowels & 0.927  & 0.940  & 0.722  & 0.653  & 0.931  & 0.973  & 0.739  & 0.606  & 0.622  & 0.532  & 0.921  & 0.516  & 0.935  & 0.499  & 0.884  & 0.921  \\
    % Waveform & 0.686  & 0.726  & 0.688  & 0.655  & 0.733  & 0.738  & 0.715  & 0.493  & 0.624  & 0.750  & 0.713  & 0.635  & 0.744  & 0.539  & 0.718  & 0.743  \\
    % WBC   & 0.946  & 0.609  & 0.987  & 0.982  & 0.542  & 0.906  & 0.990  & N/A   & 0.991  & 0.991  & 0.969  & 0.949  & 0.974  & 0.625  & 0.977  & 0.989  \\
    % Wilt  & 0.533  & 0.497  & 0.325  & 0.204  & 0.507  & 0.484  & 0.419  & 0.373  & 0.363  & 0.334  & 0.345  & 0.447  & 0.349  & 0.459  & 0.490  & 0.526  \\
    % wine  & 0.461  & 0.444  & 0.914  & 0.844  & 0.377  & 0.450  & 0.804  & 0.617  & 0.772  & 0.887  & 0.271  & 0.822  & 0.274  & 0.643  & 0.827  & 0.952  \\
    % WPBC  & 0.513  & 0.459  & 0.512  & 0.460  & 0.414  & 0.466  & 0.466  & 0.478  & 0.466  & 0.493  & 0.453  & 0.497  & 0.450  & 0.440  & 0.480  & 0.499  \\
    \textbf{Avg. Rank} & \textbf{9.4 } & \textbf{12.0 } & \textbf{7.8 } & \textbf{8.2 } & \textbf{11.0 } & \textbf{8.0 } & \textcolor{darkgreen}{\textbf{6.6 }} & \textbf{12.0 } & \textbf{7.8 } & \textbf{7.2 } & \textbf{7.4 } & \textbf{9.4 } & \textbf{7.7 } & \textbf{13.0 } & \textcolor{blue}{\textbf{5.1 }} & \textcolor{red}{\textbf{3.4 }} \\
    \bottomrule
    \end{tabular}%
  \label{tab:sel30_auc}%
  \end{adjustbox}
\end{table*}%

